The Space of Adversarial Strategies

Adversarial examples, inputs designed to induce worst-case behavior in machine learning models, have been extensively studied over the past decade. Yet, our understanding of this phenomenon stems from a rather fragmented pool of knowledge; at present, there are a handful of attacks, each with disparate assumptions in threat models and incomparable definitions of optimality. In this paper, we propose a systematic approach to characterize worst-case (i.e., optimal) adversaries. We first introduce an extensible decomposition of attacks in adversarial machine learning by atomizing attack components into surfaces and travelers. With our decomposition, we enumerate over components to create 576 attacks (568 of which were previously unexplored). Next, we propose the Pareto Ensemble Attack (PEA): a theoretical attack that upper-bounds attack performance. With our new attacks, we measure performance relative to the PEA on: both robust and non-robust models, seven datasets, and three extended lp-based threat models incorporating compute costs, formalizing the Space of Adversarial Strategies. From our evaluation we find that attack performance to be highly contextual: the domain, model robustness, and threat model can have a profound influence on attack efficacy. Our investigation suggests that future studies measuring the security of machine learning should: (1) be contextualized to the domain & threat models, and (2) go beyond the handful of known attacks used today.

==> 02.overview.tex <==
\section{Overview}\label{overview}

Analyses in adversarial machine learning have traditionally been disjoint and
ad hoc; claims are often incompatible with one another, leading to a fog of
narrow facts with vague notions of optimality. For any meaningful evaluation,
we require more than the handful of attacks that exist today as well as a
standardized approach for assessing their performance. To this end, we: (1)
propose a decomposition of attacks that yields an attack space that is
exponential in the number of attacks used today, and (2) define a standardized
approach to fairly measure attack performance. This paper is principally driven
by these two objectives.

\shortsection{Formalizing the Space of Adversarial Strategies} We find that
seminal attacks in adversarial machine learning rely on a common set of
techniques, seasoned with algorithmic choices to meet specific objectives
defined in their respective papers. We project these choices into a set of
mutually-compatible components, wherein we assemble \num{568} new attacks by
permuting these components. We describe our formulation for decomposing
adversarial machine learning attacks in \autoref{decomposition}.

\shortsection{Defining Optimality} At present, we find it challenging to answer
when one attack outperforms another (if they can even be fairly compared at
all). To investigate this hypothesis, we construct a theoretical attack, the
\oeafull{} (\oea{}), which we then use to fairly compare attack performance. We
disclose the formulation of the \oea{} and performance measurements in
\autoref{methodology}.


==> figures/attack_translation_full0.tex <==
0.0 & \sgd{} & \textit{False} & \textit{False} & \lp[0] & \identitysmap{} & \identityloss{}\\0.7D0 & \sgd{} & \textit{False} & \textit{False} & \lp[2] & \identitysmap{} & \identityloss{}\\0.BB8 & \sgd{} & \textit{False} & \textit{False} & \lp[\infty] & \identitysmap{} & \identityloss{}\\\texttt{JSMA} & \sgd{} & \textit{False} & \textit{False} & \lp[0] & \jsmasmap{} & \identityloss{}\\0.834 & \sgd{} & \textit{False} & \textit{False} & \lp[2] & \jsmasmap{} & \identityloss{}\\0.C1C & \sgd{} & \textit{False} & \textit{False} & \lp[\infty] & \jsmasmap{} & \identityloss{}\\0.C8 & \sgd{} & \textit{False} & \textit{False} & \lp[0] & \dfsmap{} & \identityloss{}\\\texttt{DF} & \sgd{} & \textit{False} & \textit{False} & \lp[2] & \dfsmap{} & \identityloss{}\\0.C80 & \sgd{} & \textit{False} & \textit{False} & \lp[\infty] & \dfsmap{} & \identityloss{}\\0.A & \sgd{} & \textit{False} & \textit{False} & \lp[0] & \identitysmap{} & \crossentropy{}\\0.7DA & \sgd{} & \textit{False} & \textit{False} & \lp[2] & \identitysmap{} & \crossentropy{}\\\texttt{BIM} & \sgd{} & \textit{False} & \textit{False} & \lp[\infty] & \identitysmap{} & \crossentropy{}\\0.6E & \sgd{} & \textit{False} & \textit{False} & \lp[0] & \jsmasmap{} & \crossentropy{}\\0.83E & \sgd{} & \textit{False} & \textit{False} & \lp[2] & \jsmasmap{} & \crossentropy{}\\0.C26 & \sgd{} & \textit{False} & \textit{False} & \lp[\infty] & \jsmasmap{} & \crossentropy{}\\0.D2 & \sgd{} & \textit{False} & \textit{False} & \lp[0] & \dfsmap{} & \crossentropy{}\\0.8A2 & \sgd{} & \textit{False} & \textit{False} & \lp[2] & \dfsmap{} & \crossentropy{}\\0.C8A & \sgd{} & \textit{False} & \textit{False} & \lp[\infty] & \dfsmap{} & \crossentropy{}\\0.14 & \sgd{} & \textit{False} & \textit{False} & \lp[0] & \identitysmap{} & \cwloss{}\\0.7E4 & \sgd{} & \textit{False} & \textit{False} & \lp[2] & \identitysmap{} & \cwloss{}\\0.BCC & \sgd{} & \textit{False} & \textit{False} & \lp[\infty] & \identitysmap{} & \cwloss{}\\0.78 & \sgd{} & \textit{False} & \textit{False} & \lp[0] & \jsmasmap{} & \cwloss{}\\0.848 & \sgd{} & \textit{False} & \textit{False} & \lp[2] & \jsmasmap{} & \cwloss{}\\0.C30 & \sgd{} & \textit{False} & \textit{False} & \lp[\infty] & \jsmasmap{} & \cwloss{}\\0.DC & \sgd{} & \textit{False} & \textit{False} & \lp[0] & \dfsmap{} & \cwloss{}\\0.8AC & \sgd{} & \textit{False} & \textit{False} & \lp[2] & \dfsmap{} & \cwloss{}\\0.C94 & \sgd{} & \textit{False} & \textit{False} & \lp[\infty] & \dfsmap{} & \cwloss{}\\A.0 & \sgd{} & \textit{True} & \textit{False} & \lp[0] & \identitysmap{} & \identityloss{}\\A.7D0 & \sgd{} & \textit{True} & \textit{False} & \lp[2] & \identitysmap{} & \identityloss{}\\A.BB8 & \sgd{} & \textit{True} & \textit{False} & \lp[\infty] & \identitysmap{} & \identityloss{}\\A.64 & \sgd{} & \textit{True} & \textit{False} & \lp[0] & \jsmasmap{} & \identityloss{}\\A.834 & \sgd{} & \textit{True} & \textit{False} & \lp[2] & \jsmasmap{} & \identityloss{}\\A.C1C & \sgd{} & \textit{True} & \textit{False} & \lp[\infty] & \jsmasmap{} & \identityloss{}\\A.C8 & \sgd{} & \textit{True} & \textit{False} & \lp[0] & \dfsmap{} & \identityloss{}\\A.898 & \sgd{} & \textit{True} & \textit{False} & \lp[2] & \dfsmap{} & \identityloss{}\\A.C80 & \sgd{} & \textit{True} & \textit{False} & \lp[\infty] & \dfsmap{} & \identityloss{}\\A.A & \sgd{} & \textit{True} & \textit{False} & \lp[0] & \identitysmap{} & \crossentropy{}\\A.7DA & \sgd{} & \textit{True} & \textit{False} & \lp[2] & \identitysmap{} & \crossentropy{}\\A.BC2 & \sgd{} & \textit{True} & \textit{False} & \lp[\infty] & \identitysmap{} & \crossentropy{}\\A.6E & \sgd{} & \textit{True} & \textit{False} & \lp[0] & \jsmasmap{} & \crossentropy{}\\A.83E & \sgd{} & \textit{True} & \textit{False} & \lp[2] & \jsmasmap{} & \crossentropy{}\\A.C26 & \sgd{} & \textit{True} & \textit{False} & \lp[\infty] & \jsmasmap{} & \crossentropy{}\\A.D2 & \sgd{} & \textit{True} & \textit{False} & \lp[0] & \dfsmap{} & \crossentropy{}\\A.8A2 & \sgd{} & \textit{True} & \textit{False} & \lp[2] & \dfsmap{} & \crossentropy{}\\A.C8A & \sgd{} & \textit{True} & \textit{False} & \lp[\infty] & \dfsmap{} & \crossentropy{}\\A.14 & \sgd{} & \textit{True} & \textit{False} & \lp[0] & \identitysmap{} & \cwloss{}\\A.7E4 & \sgd{} & \textit{True} & \textit{False} & \lp[2] & \identitysmap{} & \cwloss{}\\A.BCC & \sgd{} & \textit{True} & \textit{False} & \lp[\infty] & \identitysmap{} & \cwloss{}\\A.78 & \sgd{} & \textit{True} & \textit{False} & \lp[0] & \jsmasmap{} & \cwloss{}\\A.848 & \sgd{} & \textit{True} & \textit{False} & \lp[2] & \jsmasmap{} & \cwloss{}\\A.C30 & \sgd{} & \textit{True} & \textit{False} & \lp[\infty] & \jsmasmap{} & \cwloss{}\\A.DC & \sgd{} & \textit{True} & \textit{False} & \lp[0] & \dfsmap{} & \cwloss{}\\A.8AC & \sgd{} & \textit{True} & \textit{False} & \lp[2] & \dfsmap{} & \cwloss{}\\A.C94 & \sgd{} & \textit{True} & \textit{False} & \lp[\infty] & \dfsmap{} & \cwloss{}\\64.0 & \sgd{} & \textit{False} & \textit{True} & \lp[0] & \identitysmap{} & \identityloss{}\\64.7D0 & \sgd{} & \textit{False} & \textit{True} & \lp[2] & \identitysmap{} & \identityloss{}\\64.BB8 & \sgd{} & \textit{False} & \textit{True} & \lp[\infty] & \identitysmap{} & \identityloss{}\\64.64 & \sgd{} & \textit{False} & \textit{True} & \lp[0] & \jsmasmap{} & \identityloss{}\\64.834 & \sgd{} & \textit{False} & \textit{True} & \lp[2] & \jsmasmap{} & \identityloss{}\\64.C1C & \sgd{} & \textit{False} & \textit{True} & \lp[\infty] & \jsmasmap{} & \identityloss{}\\64.C8 & \sgd{} & \textit{False} & \textit{True} & \lp[0] & \dfsmap{} & \identityloss{}\\64.898 & \sgd{} & \textit{False} & \textit{True} & \lp[2] & \dfsmap{} & \identityloss{}\\64.C80 & \sgd{} & \textit{False} & \textit{True} & \lp[\infty] & \dfsmap{} & \identityloss{}\\64.A & \sgd{} & \textit{False} & \textit{True} & \lp[0] & \identitysmap{} & \crossentropy{}\\64.7DA & \sgd{} & \textit{False} & \textit{True} & \lp[2] & \identitysmap{} & \crossentropy{}\\\texttt{PGD} & \sgd{} & \textit{False} & \textit{True} & \lp[\infty] & \identitysmap{} & \crossentropy{}\\64.6E & \sgd{} & \textit{False} & \textit{True} & \lp[0] & \jsmasmap{} & \crossentropy{}\\64.83E & \sgd{} & \textit{False} & \textit{True} & \lp[2] & \jsmasmap{} & \crossentropy{}\\64.C26 & \sgd{} & \textit{False} & \textit{True} & \lp[\infty] & \jsmasmap{} & \crossentropy{}\\64.D2 & \sgd{} & \textit{False} & \textit{True} & \lp[0] & \dfsmap{} & \crossentropy{}\\64.8A2 & \sgd{} & \textit{False} & \textit{True} & \lp[2] & \dfsmap{} & \crossentropy{}\\64.C8A & \sgd{} & \textit{False} & \textit{True} & \lp[\infty] & \dfsmap{} & \crossentropy{}\\

==> figures/attack_translation_full1.tex <==
64.14 & \sgd{} & \textit{False} & \textit{True} & \lp[0] & \identitysmap{} & \cwloss{}\\64.7E4 & \sgd{} & \textit{False} & \textit{True} & \lp[2] & \identitysmap{} & \cwloss{}\\64.BCC & \sgd{} & \textit{False} & \textit{True} & \lp[\infty] & \identitysmap{} & \cwloss{}\\64.78 & \sgd{} & \textit{False} & \textit{True} & \lp[0] & \jsmasmap{} & \cwloss{}\\64.848 & \sgd{} & \textit{False} & \textit{True} & \lp[2] & \jsmasmap{} & \cwloss{}\\64.C30 & \sgd{} & \textit{False} & \textit{True} & \lp[\infty] & \jsmasmap{} & \cwloss{}\\64.DC & \sgd{} & \textit{False} & \textit{True} & \lp[0] & \dfsmap{} & \cwloss{}\\64.8AC & \sgd{} & \textit{False} & \textit{True} & \lp[2] & \dfsmap{} & \cwloss{}\\64.C94 & \sgd{} & \textit{False} & \textit{True} & \lp[\infty] & \dfsmap{} & \cwloss{}\\6E.0 & \sgd{} & \textit{True} & \textit{True} & \lp[0] & \identitysmap{} & \identityloss{}\\6E.7D0 & \sgd{} & \textit{True} & \textit{True} & \lp[2] & \identitysmap{} & \identityloss{}\\6E.BB8 & \sgd{} & \textit{True} & \textit{True} & \lp[\infty] & \identitysmap{} & \identityloss{}\\6E.64 & \sgd{} & \textit{True} & \textit{True} & \lp[0] & \jsmasmap{} & \identityloss{}\\6E.834 & \sgd{} & \textit{True} & \textit{True} & \lp[2] & \jsmasmap{} & \identityloss{}\\6E.C1C & \sgd{} & \textit{True} & \textit{True} & \lp[\infty] & \jsmasmap{} & \identityloss{}\\6E.C8 & \sgd{} & \textit{True} & \textit{True} & \lp[0] & \dfsmap{} & \identityloss{}\\6E.898 & \sgd{} & \textit{True} & \textit{True} & \lp[2] & \dfsmap{} & \identityloss{}\\6E.C80 & \sgd{} & \textit{True} & \textit{True} & \lp[\infty] & \dfsmap{} & \identityloss{}\\6E.A & \sgd{} & \textit{True} & \textit{True} & \lp[0] & \identitysmap{} & \crossentropy{}\\6E.7DA & \sgd{} & \textit{True} & \textit{True} & \lp[2] & \identitysmap{} & \crossentropy{}\\6E.BC2 & \sgd{} & \textit{True} & \textit{True} & \lp[\infty] & \identitysmap{} & \crossentropy{}\\6E.6E & \sgd{} & \textit{True} & \textit{True} & \lp[0] & \jsmasmap{} & \crossentropy{}\\6E.83E & \sgd{} & \textit{True} & \textit{True} & \lp[2] & \jsmasmap{} & \crossentropy{}\\6E.C26 & \sgd{} & \textit{True} & \textit{True} & \lp[\infty] & \jsmasmap{} & \crossentropy{}\\6E.D2 & \sgd{} & \textit{True} & \textit{True} & \lp[0] & \dfsmap{} & \crossentropy{}\\6E.8A2 & \sgd{} & \textit{True} & \textit{True} & \lp[2] & \dfsmap{} & \crossentropy{}\\6E.C8A & \sgd{} & \textit{True} & \textit{True} & \lp[\infty] & \dfsmap{} & \crossentropy{}\\6E.14 & \sgd{} & \textit{True} & \textit{True} & \lp[0] & \identitysmap{} & \cwloss{}\\6E.7E4 & \sgd{} & \textit{True} & \textit{True} & \lp[2] & \identitysmap{} & \cwloss{}\\6E.BCC & \sgd{} & \textit{True} & \textit{True} & \lp[\infty] & \identitysmap{} & \cwloss{}\\6E.78 & \sgd{} & \textit{True} & \textit{True} & \lp[0] & \jsmasmap{} & \cwloss{}\\6E.848 & \sgd{} & \textit{True} & \textit{True} & \lp[2] & \jsmasmap{} & \cwloss{}\\6E.C30 & \sgd{} & \textit{True} & \textit{True} & \lp[\infty] & \jsmasmap{} & \cwloss{}\\6E.DC & \sgd{} & \textit{True} & \textit{True} & \lp[0] & \dfsmap{} & \cwloss{}\\6E.8AC & \sgd{} & \textit{True} & \textit{True} & \lp[2] & \dfsmap{} & \cwloss{}\\6E.C94 & \sgd{} & \textit{True} & \textit{True} & \lp[\infty] & \dfsmap{} & \cwloss{}\\1.0 & \adam{} & \textit{False} & \textit{False} & \lp[0] & \identitysmap{} & \identityloss{}\\1.7D0 & \adam{} & \textit{False} & \textit{False} & \lp[2] & \identitysmap{} & \identityloss{}\\1.BB8 & \adam{} & \textit{False} & \textit{False} & \lp[\infty] & \identitysmap{} & \identityloss{}\\1.64 & \adam{} & \textit{False} & \textit{False} & \lp[0] & \jsmasmap{} & \identityloss{}\\1.834 & \adam{} & \textit{False} & \textit{False} & \lp[2] & \jsmasmap{} & \identityloss{}\\1.C1C & \adam{} & \textit{False} & \textit{False} & \lp[\infty] & \jsmasmap{} & \identityloss{}\\1.C8 & \adam{} & \textit{False} & \textit{False} & \lp[0] & \dfsmap{} & \identityloss{}\\1.898 & \adam{} & \textit{False} & \textit{False} & \lp[2] & \dfsmap{} & \identityloss{}\\1.C80 & \adam{} & \textit{False} & \textit{False} & \lp[\infty] & \dfsmap{} & \identityloss{}\\1.A & \adam{} & \textit{False} & \textit{False} & \lp[0] & \identitysmap{} & \crossentropy{}\\1.7DA & \adam{} & \textit{False} & \textit{False} & \lp[2] & \identitysmap{} & \crossentropy{}\\1.BC2 & \adam{} & \textit{False} & \textit{False} & \lp[\infty] & \identitysmap{} & \crossentropy{}\\1.6E & \adam{} & \textit{False} & \textit{False} & \lp[0] & \jsmasmap{} & \crossentropy{}\\1.83E & \adam{} & \textit{False} & \textit{False} & \lp[2] & \jsmasmap{} & \crossentropy{}\\1.C26 & \adam{} & \textit{False} & \textit{False} & \lp[\infty] & \jsmasmap{} & \crossentropy{}\\1.D2 & \adam{} & \textit{False} & \textit{False} & \lp[0] & \dfsmap{} & \crossentropy{}\\1.8A2 & \adam{} & \textit{False} & \textit{False} & \lp[2] & \dfsmap{} & \crossentropy{}\\1.C8A & \adam{} & \textit{False} & \textit{False} & \lp[\infty] & \dfsmap{} & \crossentropy{}\\1.14 & \adam{} & \textit{False} & \textit{False} & \lp[0] & \identitysmap{} & \cwloss{}\\1.7E4 & \adam{} & \textit{False} & \textit{False} & \lp[2] & \identitysmap{} & \cwloss{}\\1.BCC & \adam{} & \textit{False} & \textit{False} & \lp[\infty] & \identitysmap{} & \cwloss{}\\1.78 & \adam{} & \textit{False} & \textit{False} & \lp[0] & \jsmasmap{} & \cwloss{}\\1.848 & \adam{} & \textit{False} & \textit{False} & \lp[2] & \jsmasmap{} & \cwloss{}\\1.C30 & \adam{} & \textit{False} & \textit{False} & \lp[\infty] & \jsmasmap{} & \cwloss{}\\1.DC & \adam{} & \textit{False} & \textit{False} & \lp[0] & \dfsmap{} & \cwloss{}\\1.8AC & \adam{} & \textit{False} & \textit{False} & \lp[2] & \dfsmap{} & \cwloss{}\\1.C94 & \adam{} & \textit{False} & \textit{False} & \lp[\infty] & \dfsmap{} & \cwloss{}\\B.0 & \adam{} & \textit{True} & \textit{False} & \lp[0] & \identitysmap{} & \identityloss{}\\B.7D0 & \adam{} & \textit{True} & \textit{False} & \lp[2] & \identitysmap{} & \identityloss{}\\B.BB8 & \adam{} & \textit{True} & \textit{False} & \lp[\infty] & \identitysmap{} & \identityloss{}\\B.64 & \adam{} & \textit{True} & \textit{False} & \lp[0] & \jsmasmap{} & \identityloss{}\\B.834 & \adam{} & \textit{True} & \textit{False} & \lp[2] & \jsmasmap{} & \identityloss{}\\B.C1C & \adam{} & \textit{True} & \textit{False} & \lp[\infty] & \jsmasmap{} & \identityloss{}\\B.C8 & \adam{} & \textit{True} & \textit{False} & \lp[0] & \dfsmap{} & \identityloss{}\\B.898 & \adam{} & \textit{True} & \textit{False} & \lp[2] & \dfsmap{} & \identityloss{}\\B.C80 & \adam{} & \textit{True} & \textit{False} & \lp[\infty] & \dfsmap{} & \identityloss{}\\

==> figures/attack_translation_full2.tex <==
B.A & \adam{} & \textit{True} & \textit{False} & \lp[0] & \identitysmap{} & \crossentropy{}\\B.7DA & \adam{} & \textit{True} & \textit{False} & \lp[2] & \identitysmap{} & \crossentropy{}\\B.BC2 & \adam{} & \textit{True} & \textit{False} & \lp[\infty] & \identitysmap{} & \crossentropy{}\\B.6E & \adam{} & \textit{True} & \textit{False} & \lp[0] & \jsmasmap{} & \crossentropy{}\\B.83E & \adam{} & \textit{True} & \textit{False} & \lp[2] & \jsmasmap{} & \crossentropy{}\\B.C26 & \adam{} & \textit{True} & \textit{False} & \lp[\infty] & \jsmasmap{} & \crossentropy{}\\B.D2 & \adam{} & \textit{True} & \textit{False} & \lp[0] & \dfsmap{} & \crossentropy{}\\B.8A2 & \adam{} & \textit{True} & \textit{False} & \lp[2] & \dfsmap{} & \crossentropy{}\\B.C8A & \adam{} & \textit{True} & \textit{False} & \lp[\infty] & \dfsmap{} & \crossentropy{}\\B.14 & \adam{} & \textit{True} & \textit{False} & \lp[0] & \identitysmap{} & \cwloss{}\\\texttt{CW} & \adam{} & \textit{True} & \textit{False} & \lp[2] & \identitysmap{} & \cwloss{}\\B.BCC & \adam{} & \textit{True} & \textit{False} & \lp[\infty] & \identitysmap{} & \cwloss{}\\B.78 & \adam{} & \textit{True} & \textit{False} & \lp[0] & \jsmasmap{} & \cwloss{}\\B.848 & \adam{} & \textit{True} & \textit{False} & \lp[2] & \jsmasmap{} & \cwloss{}\\B.C30 & \adam{} & \textit{True} & \textit{False} & \lp[\infty] & \jsmasmap{} & \cwloss{}\\B.DC & \adam{} & \textit{True} & \textit{False} & \lp[0] & \dfsmap{} & \cwloss{}\\B.8AC & \adam{} & \textit{True} & \textit{False} & \lp[2] & \dfsmap{} & \cwloss{}\\B.C94 & \adam{} & \textit{True} & \textit{False} & \lp[\infty] & \dfsmap{} & \cwloss{}\\65.0 & \adam{} & \textit{False} & \textit{True} & \lp[0] & \identitysmap{} & \identityloss{}\\65.7D0 & \adam{} & \textit{False} & \textit{True} & \lp[2] & \identitysmap{} & \identityloss{}\\65.BB8 & \adam{} & \textit{False} & \textit{True} & \lp[\infty] & \identitysmap{} & \identityloss{}\\65.64 & \adam{} & \textit{False} & \textit{True} & \lp[0] & \jsmasmap{} & \identityloss{}\\65.834 & \adam{} & \textit{False} & \textit{True} & \lp[2] & \jsmasmap{} & \identityloss{}\\65.C1C & \adam{} & \textit{False} & \textit{True} & \lp[\infty] & \jsmasmap{} & \identityloss{}\\65.C8 & \adam{} & \textit{False} & \textit{True} & \lp[0] & \dfsmap{} & \identityloss{}\\65.898 & \adam{} & \textit{False} & \textit{True} & \lp[2] & \dfsmap{} & \identityloss{}\\65.C80 & \adam{} & \textit{False} & \textit{True} & \lp[\infty] & \dfsmap{} & \identityloss{}\\65.A & \adam{} & \textit{False} & \textit{True} & \lp[0] & \identitysmap{} & \crossentropy{}\\65.7DA & \adam{} & \textit{False} & \textit{True} & \lp[2] & \identitysmap{} & \crossentropy{}\\65.BC2 & \adam{} & \textit{False} & \textit{True} & \lp[\infty] & \identitysmap{} & \crossentropy{}\\65.6E & \adam{} & \textit{False} & \textit{True} & \lp[0] & \jsmasmap{} & \crossentropy{}\\65.83E & \adam{} & \textit{False} & \textit{True} & \lp[2] & \jsmasmap{} & \crossentropy{}\\65.C26 & \adam{} & \textit{False} & \textit{True} & \lp[\infty] & \jsmasmap{} & \crossentropy{}\\65.D2 & \adam{} & \textit{False} & \textit{True} & \lp[0] & \dfsmap{} & \crossentropy{}\\65.8A2 & \adam{} & \textit{False} & \textit{True} & \lp[2] & \dfsmap{} & \crossentropy{}\\65.C8A & \adam{} & \textit{False} & \textit{True} & \lp[\infty] & \dfsmap{} & \crossentropy{}\\65.14 & \adam{} & \textit{False} & \textit{True} & \lp[0] & \identitysmap{} & \cwloss{}\\65.7E4 & \adam{} & \textit{False} & \textit{True} & \lp[2] & \identitysmap{} & \cwloss{}\\65.BCC & \adam{} & \textit{False} & \textit{True} & \lp[\infty] & \identitysmap{} & \cwloss{}\\65.78 & \adam{} & \textit{False} & \textit{True} & \lp[0] & \jsmasmap{} & \cwloss{}\\65.848 & \adam{} & \textit{False} & \textit{True} & \lp[2] & \jsmasmap{} & \cwloss{}\\65.C30 & \adam{} & \textit{False} & \textit{True} & \lp[\infty] & \jsmasmap{} & \cwloss{}\\65.DC & \adam{} & \textit{False} & \textit{True} & \lp[0] & \dfsmap{} & \cwloss{}\\65.8AC & \adam{} & \textit{False} & \textit{True} & \lp[2] & \dfsmap{} & \cwloss{}\\65.C94 & \adam{} & \textit{False} & \textit{True} & \lp[\infty] & \dfsmap{} & \cwloss{}\\6F.0 & \adam{} & \textit{True} & \textit{True} & \lp[0] & \identitysmap{} & \identityloss{}\\6F.7D0 & \adam{} & \textit{True} & \textit{True} & \lp[2] & \identitysmap{} & \identityloss{}\\6F.BB8 & \adam{} & \textit{True} & \textit{True} & \lp[\infty] & \identitysmap{} & \identityloss{}\\6F.64 & \adam{} & \textit{True} & \textit{True} & \lp[0] & \jsmasmap{} & \identityloss{}\\6F.834 & \adam{} & \textit{True} & \textit{True} & \lp[2] & \jsmasmap{} & \identityloss{}\\6F.C1C & \adam{} & \textit{True} & \textit{True} & \lp[\infty] & \jsmasmap{} & \identityloss{}\\6F.C8 & \adam{} & \textit{True} & \textit{True} & \lp[0] & \dfsmap{} & \identityloss{}\\6F.898 & \adam{} & \textit{True} & \textit{True} & \lp[2] & \dfsmap{} & \identityloss{}\\6F.C80 & \adam{} & \textit{True} & \textit{True} & \lp[\infty] & \dfsmap{} & \identityloss{}\\6F.A & \adam{} & \textit{True} & \textit{True} & \lp[0] & \identitysmap{} & \crossentropy{}\\6F.7DA & \adam{} & \textit{True} & \textit{True} & \lp[2] & \identitysmap{} & \crossentropy{}\\6F.BC2 & \adam{} & \textit{True} & \textit{True} & \lp[\infty] & \identitysmap{} & \crossentropy{}\\6F.6E & \adam{} & \textit{True} & \textit{True} & \lp[0] & \jsmasmap{} & \crossentropy{}\\6F.83E & \adam{} & \textit{True} & \textit{True} & \lp[2] & \jsmasmap{} & \crossentropy{}\\6F.C26 & \adam{} & \textit{True} & \textit{True} & \lp[\infty] & \jsmasmap{} & \crossentropy{}\\6F.D2 & \adam{} & \textit{True} & \textit{True} & \lp[0] & \dfsmap{} & \crossentropy{}\\6F.8A2 & \adam{} & \textit{True} & \textit{True} & \lp[2] & \dfsmap{} & \crossentropy{}\\6F.C8A & \adam{} & \textit{True} & \textit{True} & \lp[\infty] & \dfsmap{} & \crossentropy{}\\6F.14 & \adam{} & \textit{True} & \textit{True} & \lp[0] & \identitysmap{} & \cwloss{}\\6F.7E4 & \adam{} & \textit{True} & \textit{True} & \lp[2] & \identitysmap{} & \cwloss{}\\6F.BCC & \adam{} & \textit{True} & \textit{True} & \lp[\infty] & \identitysmap{} & \cwloss{}\\6F.78 & \adam{} & \textit{True} & \textit{True} & \lp[0] & \jsmasmap{} & \cwloss{}\\6F.848 & \adam{} & \textit{True} & \textit{True} & \lp[2] & \jsmasmap{} & \cwloss{}\\6F.C30 & \adam{} & \textit{True} & \textit{True} & \lp[\infty] & \jsmasmap{} & \cwloss{}\\6F.DC & \adam{} & \textit{True} & \textit{True} & \lp[0] & \dfsmap{} & \cwloss{}\\6F.8AC & \adam{} & \textit{True} & \textit{True} & \lp[2] & \dfsmap{} & \cwloss{}\\6F.C94 & \adam{} & \textit{True} & \textit{True} & \lp[\infty] & \dfsmap{} & \cwloss{}\\

==> figures/attack_translation_full_numbering0.tex <==
0 & \sgd{} & \textit{False} & \textit{False} & \lp[0] & \identitysmap{} & \identityloss{}\\1 & \sgd{} & \textit{False} & \textit{False} & \lp[2] & \identitysmap{} & \identityloss{}\\2 & \sgd{} & \textit{False} & \textit{False} & \lp[\infty] & \identitysmap{} & \identityloss{}\\\texttt{JSMA} & \sgd{} & \textit{False} & \textit{False} & \lp[0] & \jsmasmap{} & \identityloss{}\\4 & \sgd{} & \textit{False} & \textit{False} & \lp[2] & \jsmasmap{} & \identityloss{}\\5 & \sgd{} & \textit{False} & \textit{False} & \lp[\infty] & \jsmasmap{} & \identityloss{}\\6 & \sgd{} & \textit{False} & \textit{False} & \lp[0] & \dfsmap{} & \identityloss{}\\\texttt{DF} & \sgd{} & \textit{False} & \textit{False} & \lp[2] & \dfsmap{} & \identityloss{}\\8 & \sgd{} & \textit{False} & \textit{False} & \lp[\infty] & \dfsmap{} & \identityloss{}\\9 & \sgd{} & \textit{False} & \textit{False} & \lp[0] & \identitysmap{} & \crossentropy{}\\10 & \sgd{} & \textit{False} & \textit{False} & \lp[2] & \identitysmap{} & \crossentropy{}\\\texttt{BIM} & \sgd{} & \textit{False} & \textit{False} & \lp[\infty] & \identitysmap{} & \crossentropy{}\\12 & \sgd{} & \textit{False} & \textit{False} & \lp[0] & \jsmasmap{} & \crossentropy{}\\13 & \sgd{} & \textit{False} & \textit{False} & \lp[2] & \jsmasmap{} & \crossentropy{}\\14 & \sgd{} & \textit{False} & \textit{False} & \lp[\infty] & \jsmasmap{} & \crossentropy{}\\15 & \sgd{} & \textit{False} & \textit{False} & \lp[0] & \dfsmap{} & \crossentropy{}\\16 & \sgd{} & \textit{False} & \textit{False} & \lp[2] & \dfsmap{} & \crossentropy{}\\17 & \sgd{} & \textit{False} & \textit{False} & \lp[\infty] & \dfsmap{} & \crossentropy{}\\18 & \sgd{} & \textit{False} & \textit{False} & \lp[0] & \identitysmap{} & \cwloss{}\\19 & \sgd{} & \textit{False} & \textit{False} & \lp[2] & \identitysmap{} & \cwloss{}\\20 & \sgd{} & \textit{False} & \textit{False} & \lp[\infty] & \identitysmap{} & \cwloss{}\\21 & \sgd{} & \textit{False} & \textit{False} & \lp[0] & \jsmasmap{} & \cwloss{}\\22 & \sgd{} & \textit{False} & \textit{False} & \lp[2] & \jsmasmap{} & \cwloss{}\\23 & \sgd{} & \textit{False} & \textit{False} & \lp[\infty] & \jsmasmap{} & \cwloss{}\\24 & \sgd{} & \textit{False} & \textit{False} & \lp[0] & \dfsmap{} & \cwloss{}\\25 & \sgd{} & \textit{False} & \textit{False} & \lp[2] & \dfsmap{} & \cwloss{}\\26 & \sgd{} & \textit{False} & \textit{False} & \lp[\infty] & \dfsmap{} & \cwloss{}\\27 & \sgd{} & \textit{True} & \textit{False} & \lp[0] & \identitysmap{} & \identityloss{}\\28 & \sgd{} & \textit{True} & \textit{False} & \lp[2] & \identitysmap{} & \identityloss{}\\29 & \sgd{} & \textit{True} & \textit{False} & \lp[\infty] & \identitysmap{} & \identityloss{}\\30 & \sgd{} & \textit{True} & \textit{False} & \lp[0] & \jsmasmap{} & \identityloss{}\\31 & \sgd{} & \textit{True} & \textit{False} & \lp[2] & \jsmasmap{} & \identityloss{}\\32 & \sgd{} & \textit{True} & \textit{False} & \lp[\infty] & \jsmasmap{} & \identityloss{}\\33 & \sgd{} & \textit{True} & \textit{False} & \lp[0] & \dfsmap{} & \identityloss{}\\34 & \sgd{} & \textit{True} & \textit{False} & \lp[2] & \dfsmap{} & \identityloss{}\\35 & \sgd{} & \textit{True} & \textit{False} & \lp[\infty] & \dfsmap{} & \identityloss{}\\36 & \sgd{} & \textit{True} & \textit{False} & \lp[0] & \identitysmap{} & \crossentropy{}\\37 & \sgd{} & \textit{True} & \textit{False} & \lp[2] & \identitysmap{} & \crossentropy{}\\38 & \sgd{} & \textit{True} & \textit{False} & \lp[\infty] & \identitysmap{} & \crossentropy{}\\39 & \sgd{} & \textit{True} & \textit{False} & \lp[0] & \jsmasmap{} & \crossentropy{}\\40 & \sgd{} & \textit{True} & \textit{False} & \lp[2] & \jsmasmap{} & \crossentropy{}\\41 & \sgd{} & \textit{True} & \textit{False} & \lp[\infty] & \jsmasmap{} & \crossentropy{}\\42 & \sgd{} & \textit{True} & \textit{False} & \lp[0] & \dfsmap{} & \crossentropy{}\\43 & \sgd{} & \textit{True} & \textit{False} & \lp[2] & \dfsmap{} & \crossentropy{}\\44 & \sgd{} & \textit{True} & \textit{False} & \lp[\infty] & \dfsmap{} & \crossentropy{}\\45 & \sgd{} & \textit{True} & \textit{False} & \lp[0] & \identitysmap{} & \cwloss{}\\46 & \sgd{} & \textit{True} & \textit{False} & \lp[2] & \identitysmap{} & \cwloss{}\\47 & \sgd{} & \textit{True} & \textit{False} & \lp[\infty] & \identitysmap{} & \cwloss{}\\48 & \sgd{} & \textit{True} & \textit{False} & \lp[0] & \jsmasmap{} & \cwloss{}\\49 & \sgd{} & \textit{True} & \textit{False} & \lp[2] & \jsmasmap{} & \cwloss{}\\50 & \sgd{} & \textit{True} & \textit{False} & \lp[\infty] & \jsmasmap{} & \cwloss{}\\51 & \sgd{} & \textit{True} & \textit{False} & \lp[0] & \dfsmap{} & \cwloss{}\\52 & \sgd{} & \textit{True} & \textit{False} & \lp[2] & \dfsmap{} & \cwloss{}\\53 & \sgd{} & \textit{True} & \textit{False} & \lp[\infty] & \dfsmap{} & \cwloss{}\\54 & \sgd{} & \textit{False} & \textit{True} & \lp[0] & \identitysmap{} & \identityloss{}\\55 & \sgd{} & \textit{False} & \textit{True} & \lp[2] & \identitysmap{} & \identityloss{}\\56 & \sgd{} & \textit{False} & \textit{True} & \lp[\infty] & \identitysmap{} & \identityloss{}\\57 & \sgd{} & \textit{False} & \textit{True} & \lp[0] & \jsmasmap{} & \identityloss{}\\58 & \sgd{} & \textit{False} & \textit{True} & \lp[2] & \jsmasmap{} & \identityloss{}\\59 & \sgd{} & \textit{False} & \textit{True} & \lp[\infty] & \jsmasmap{} & \identityloss{}\\60 & \sgd{} & \textit{False} & \textit{True} & \lp[0] & \dfsmap{} & \identityloss{}\\61 & \sgd{} & \textit{False} & \textit{True} & \lp[2] & \dfsmap{} & \identityloss{}\\62 & \sgd{} & \textit{False} & \textit{True} & \lp[\infty] & \dfsmap{} & \identityloss{}\\63 & \sgd{} & \textit{False} & \textit{True} & \lp[0] & \identitysmap{} & \crossentropy{}\\64 & \sgd{} & \textit{False} & \textit{True} & \lp[2] & \identitysmap{} & \crossentropy{}\\\texttt{PGD} & \sgd{} & \textit{False} & \textit{True} & \lp[\infty] & \identitysmap{} & \crossentropy{}\\66 & \sgd{} & \textit{False} & \textit{True} & \lp[0] & \jsmasmap{} & \crossentropy{}\\67 & \sgd{} & \textit{False} & \textit{True} & \lp[2] & \jsmasmap{} & \crossentropy{}\\68 & \sgd{} & \textit{False} & \textit{True} & \lp[\infty] & \jsmasmap{} & \crossentropy{}\\69 & \sgd{} & \textit{False} & \textit{True} & \lp[0] & \dfsmap{} & \crossentropy{}\\70 & \sgd{} & \textit{False} & \textit{True} & \lp[2] & \dfsmap{} & \crossentropy{}\\71 & \sgd{} & \textit{False} & \textit{True} & \lp[\infty] & \dfsmap{} & \crossentropy{}\\

==> figures/attack_translation_full_numbering1.tex <==
72 & \sgd{} & \textit{False} & \textit{True} & \lp[0] & \identitysmap{} & \cwloss{}\\73 & \sgd{} & \textit{False} & \textit{True} & \lp[2] & \identitysmap{} & \cwloss{}\\74 & \sgd{} & \textit{False} & \textit{True} & \lp[\infty] & \identitysmap{} & \cwloss{}\\75 & \sgd{} & \textit{False} & \textit{True} & \lp[0] & \jsmasmap{} & \cwloss{}\\76 & \sgd{} & \textit{False} & \textit{True} & \lp[2] & \jsmasmap{} & \cwloss{}\\77 & \sgd{} & \textit{False} & \textit{True} & \lp[\infty] & \jsmasmap{} & \cwloss{}\\78 & \sgd{} & \textit{False} & \textit{True} & \lp[0] & \dfsmap{} & \cwloss{}\\79 & \sgd{} & \textit{False} & \textit{True} & \lp[2] & \dfsmap{} & \cwloss{}\\80 & \sgd{} & \textit{False} & \textit{True} & \lp[\infty] & \dfsmap{} & \cwloss{}\\81 & \sgd{} & \textit{True} & \textit{True} & \lp[0] & \identitysmap{} & \identityloss{}\\82 & \sgd{} & \textit{True} & \textit{True} & \lp[2] & \identitysmap{} & \identityloss{}\\83 & \sgd{} & \textit{True} & \textit{True} & \lp[\infty] & \identitysmap{} & \identityloss{}\\84 & \sgd{} & \textit{True} & \textit{True} & \lp[0] & \jsmasmap{} & \identityloss{}\\85 & \sgd{} & \textit{True} & \textit{True} & \lp[2] & \jsmasmap{} & \identityloss{}\\86 & \sgd{} & \textit{True} & \textit{True} & \lp[\infty] & \jsmasmap{} & \identityloss{}\\87 & \sgd{} & \textit{True} & \textit{True} & \lp[0] & \dfsmap{} & \identityloss{}\\88 & \sgd{} & \textit{True} & \textit{True} & \lp[2] & \dfsmap{} & \identityloss{}\\89 & \sgd{} & \textit{True} & \textit{True} & \lp[\infty] & \dfsmap{} & \identityloss{}\\90 & \sgd{} & \textit{True} & \textit{True} & \lp[0] & \identitysmap{} & \crossentropy{}\\91 & \sgd{} & \textit{True} & \textit{True} & \lp[2] & \identitysmap{} & \crossentropy{}\\92 & \sgd{} & \textit{True} & \textit{True} & \lp[\infty] & \identitysmap{} & \crossentropy{}\\93 & \sgd{} & \textit{True} & \textit{True} & \lp[0] & \jsmasmap{} & \crossentropy{}\\94 & \sgd{} & \textit{True} & \textit{True} & \lp[2] & \jsmasmap{} & \crossentropy{}\\95 & \sgd{} & \textit{True} & \textit{True} & \lp[\infty] & \jsmasmap{} & \crossentropy{}\\96 & \sgd{} & \textit{True} & \textit{True} & \lp[0] & \dfsmap{} & \crossentropy{}\\97 & \sgd{} & \textit{True} & \textit{True} & \lp[2] & \dfsmap{} & \crossentropy{}\\98 & \sgd{} & \textit{True} & \textit{True} & \lp[\infty] & \dfsmap{} & \crossentropy{}\\99 & \sgd{} & \textit{True} & \textit{True} & \lp[0] & \identitysmap{} & \cwloss{}\\100 & \sgd{} & \textit{True} & \textit{True} & \lp[2] & \identitysmap{} & \cwloss{}\\101 & \sgd{} & \textit{True} & \textit{True} & \lp[\infty] & \identitysmap{} & \cwloss{}\\102 & \sgd{} & \textit{True} & \textit{True} & \lp[0] & \jsmasmap{} & \cwloss{}\\103 & \sgd{} & \textit{True} & \textit{True} & \lp[2] & \jsmasmap{} & \cwloss{}\\104 & \sgd{} & \textit{True} & \textit{True} & \lp[\infty] & \jsmasmap{} & \cwloss{}\\105 & \sgd{} & \textit{True} & \textit{True} & \lp[0] & \dfsmap{} & \cwloss{}\\106 & \sgd{} & \textit{True} & \textit{True} & \lp[2] & \dfsmap{} & \cwloss{}\\107 & \sgd{} & \textit{True} & \textit{True} & \lp[\infty] & \dfsmap{} & \cwloss{}\\108 & \adam{} & \textit{False} & \textit{False} & \lp[0] & \identitysmap{} & \identityloss{}\\109 & \adam{} & \textit{False} & \textit{False} & \lp[2] & \identitysmap{} & \identityloss{}\\110 & \adam{} & \textit{False} & \textit{False} & \lp[\infty] & \identitysmap{} & \identityloss{}\\111 & \adam{} & \textit{False} & \textit{False} & \lp[0] & \jsmasmap{} & \identityloss{}\\112 & \adam{} & \textit{False} & \textit{False} & \lp[2] & \jsmasmap{} & \identityloss{}\\113 & \adam{} & \textit{False} & \textit{False} & \lp[\infty] & \jsmasmap{} & \identityloss{}\\114 & \adam{} & \textit{False} & \textit{False} & \lp[0] & \dfsmap{} & \identityloss{}\\115 & \adam{} & \textit{False} & \textit{False} & \lp[2] & \dfsmap{} & \identityloss{}\\116 & \adam{} & \textit{False} & \textit{False} & \lp[\infty] & \dfsmap{} & \identityloss{}\\117 & \adam{} & \textit{False} & \textit{False} & \lp[0] & \identitysmap{} & \crossentropy{}\\118 & \adam{} & \textit{False} & \textit{False} & \lp[2] & \identitysmap{} & \crossentropy{}\\119 & \adam{} & \textit{False} & \textit{False} & \lp[\infty] & \identitysmap{} & \crossentropy{}\\120 & \adam{} & \textit{False} & \textit{False} & \lp[0] & \jsmasmap{} & \crossentropy{}\\121 & \adam{} & \textit{False} & \textit{False} & \lp[2] & \jsmasmap{} & \crossentropy{}\\122 & \adam{} & \textit{False} & \textit{False} & \lp[\infty] & \jsmasmap{} & \crossentropy{}\\123 & \adam{} & \textit{False} & \textit{False} & \lp[0] & \dfsmap{} & \crossentropy{}\\124 & \adam{} & \textit{False} & \textit{False} & \lp[2] & \dfsmap{} & \crossentropy{}\\125 & \adam{} & \textit{False} & \textit{False} & \lp[\infty] & \dfsmap{} & \crossentropy{}\\126 & \adam{} & \textit{False} & \textit{False} & \lp[0] & \identitysmap{} & \cwloss{}\\127 & \adam{} & \textit{False} & \textit{False} & \lp[2] & \identitysmap{} & \cwloss{}\\128 & \adam{} & \textit{False} & \textit{False} & \lp[\infty] & \identitysmap{} & \cwloss{}\\129 & \adam{} & \textit{False} & \textit{False} & \lp[0] & \jsmasmap{} & \cwloss{}\\130 & \adam{} & \textit{False} & \textit{False} & \lp[2] & \jsmasmap{} & \cwloss{}\\131 & \adam{} & \textit{False} & \textit{False} & \lp[\infty] & \jsmasmap{} & \cwloss{}\\132 & \adam{} & \textit{False} & \textit{False} & \lp[0] & \dfsmap{} & \cwloss{}\\133 & \adam{} & \textit{False} & \textit{False} & \lp[2] & \dfsmap{} & \cwloss{}\\134 & \adam{} & \textit{False} & \textit{False} & \lp[\infty] & \dfsmap{} & \cwloss{}\\135 & \adam{} & \textit{True} & \textit{False} & \lp[0] & \identitysmap{} & \identityloss{}\\136 & \adam{} & \textit{True} & \textit{False} & \lp[2] & \identitysmap{} & \identityloss{}\\137 & \adam{} & \textit{True} & \textit{False} & \lp[\infty] & \identitysmap{} & \identityloss{}\\138 & \adam{} & \textit{True} & \textit{False} & \lp[0] & \jsmasmap{} & \identityloss{}\\139 & \adam{} & \textit{True} & \textit{False} & \lp[2] & \jsmasmap{} & \identityloss{}\\140 & \adam{} & \textit{True} & \textit{False} & \lp[\infty] & \jsmasmap{} & \identityloss{}\\141 & \adam{} & \textit{True} & \textit{False} & \lp[0] & \dfsmap{} & \identityloss{}\\142 & \adam{} & \textit{True} & \textit{False} & \lp[2] & \dfsmap{} & \identityloss{}\\143 & \adam{} & \textit{True} & \textit{False} & \lp[\infty] & \dfsmap{} & \identityloss{}\\

==> figures/attack_translation_full_numbering2.tex <==
144 & \adam{} & \textit{True} & \textit{False} & \lp[0] & \identitysmap{} & \crossentropy{}\\145 & \adam{} & \textit{True} & \textit{False} & \lp[2] & \identitysmap{} & \crossentropy{}\\146 & \adam{} & \textit{True} & \textit{False} & \lp[\infty] & \identitysmap{} & \crossentropy{}\\147 & \adam{} & \textit{True} & \textit{False} & \lp[0] & \jsmasmap{} & \crossentropy{}\\148 & \adam{} & \textit{True} & \textit{False} & \lp[2] & \jsmasmap{} & \crossentropy{}\\149 & \adam{} & \textit{True} & \textit{False} & \lp[\infty] & \jsmasmap{} & \crossentropy{}\\150 & \adam{} & \textit{True} & \textit{False} & \lp[0] & \dfsmap{} & \crossentropy{}\\151 & \adam{} & \textit{True} & \textit{False} & \lp[2] & \dfsmap{} & \crossentropy{}\\152 & \adam{} & \textit{True} & \textit{False} & \lp[\infty] & \dfsmap{} & \crossentropy{}\\153 & \adam{} & \textit{True} & \textit{False} & \lp[0] & \identitysmap{} & \cwloss{}\\\texttt{CW} & \adam{} & \textit{True} & \textit{False} & \lp[2] & \identitysmap{} & \cwloss{}\\155 & \adam{} & \textit{True} & \textit{False} & \lp[\infty] & \identitysmap{} & \cwloss{}\\156 & \adam{} & \textit{True} & \textit{False} & \lp[0] & \jsmasmap{} & \cwloss{}\\157 & \adam{} & \textit{True} & \textit{False} & \lp[2] & \jsmasmap{} & \cwloss{}\\158 & \adam{} & \textit{True} & \textit{False} & \lp[\infty] & \jsmasmap{} & \cwloss{}\\159 & \adam{} & \textit{True} & \textit{False} & \lp[0] & \dfsmap{} & \cwloss{}\\160 & \adam{} & \textit{True} & \textit{False} & \lp[2] & \dfsmap{} & \cwloss{}\\161 & \adam{} & \textit{True} & \textit{False} & \lp[\infty] & \dfsmap{} & \cwloss{}\\162 & \adam{} & \textit{False} & \textit{True} & \lp[0] & \identitysmap{} & \identityloss{}\\163 & \adam{} & \textit{False} & \textit{True} & \lp[2] & \identitysmap{} & \identityloss{}\\164 & \adam{} & \textit{False} & \textit{True} & \lp[\infty] & \identitysmap{} & \identityloss{}\\165 & \adam{} & \textit{False} & \textit{True} & \lp[0] & \jsmasmap{} & \identityloss{}\\166 & \adam{} & \textit{False} & \textit{True} & \lp[2] & \jsmasmap{} & \identityloss{}\\167 & \adam{} & \textit{False} & \textit{True} & \lp[\infty] & \jsmasmap{} & \identityloss{}\\168 & \adam{} & \textit{False} & \textit{True} & \lp[0] & \dfsmap{} & \identityloss{}\\169 & \adam{} & \textit{False} & \textit{True} & \lp[2] & \dfsmap{} & \identityloss{}\\170 & \adam{} & \textit{False} & \textit{True} & \lp[\infty] & \dfsmap{} & \identityloss{}\\171 & \adam{} & \textit{False} & \textit{True} & \lp[0] & \identitysmap{} & \crossentropy{}\\172 & \adam{} & \textit{False} & \textit{True} & \lp[2] & \identitysmap{} & \crossentropy{}\\173 & \adam{} & \textit{False} & \textit{True} & \lp[\infty] & \identitysmap{} & \crossentropy{}\\174 & \adam{} & \textit{False} & \textit{True} & \lp[0] & \jsmasmap{} & \crossentropy{}\\175 & \adam{} & \textit{False} & \textit{True} & \lp[2] & \jsmasmap{} & \crossentropy{}\\176 & \adam{} & \textit{False} & \textit{True} & \lp[\infty] & \jsmasmap{} & \crossentropy{}\\177 & \adam{} & \textit{False} & \textit{True} & \lp[0] & \dfsmap{} & \crossentropy{}\\178 & \adam{} & \textit{False} & \textit{True} & \lp[2] & \dfsmap{} & \crossentropy{}\\179 & \adam{} & \textit{False} & \textit{True} & \lp[\infty] & \dfsmap{} & \crossentropy{}\\180 & \adam{} & \textit{False} & \textit{True} & \lp[0] & \identitysmap{} & \cwloss{}\\181 & \adam{} & \textit{False} & \textit{True} & \lp[2] & \identitysmap{} & \cwloss{}\\182 & \adam{} & \textit{False} & \textit{True} & \lp[\infty] & \identitysmap{} & \cwloss{}\\183 & \adam{} & \textit{False} & \textit{True} & \lp[0] & \jsmasmap{} & \cwloss{}\\184 & \adam{} & \textit{False} & \textit{True} & \lp[2] & \jsmasmap{} & \cwloss{}\\185 & \adam{} & \textit{False} & \textit{True} & \lp[\infty] & \jsmasmap{} & \cwloss{}\\186 & \adam{} & \textit{False} & \textit{True} & \lp[0] & \dfsmap{} & \cwloss{}\\187 & \adam{} & \textit{False} & \textit{True} & \lp[2] & \dfsmap{} & \cwloss{}\\188 & \adam{} & \textit{False} & \textit{True} & \lp[\infty] & \dfsmap{} & \cwloss{}\\189 & \adam{} & \textit{True} & \textit{True} & \lp[0] & \identitysmap{} & \identityloss{}\\190 & \adam{} & \textit{True} & \textit{True} & \lp[2] & \identitysmap{} & \identityloss{}\\191 & \adam{} & \textit{True} & \textit{True} & \lp[\infty] & \identitysmap{} & \identityloss{}\\192 & \adam{} & \textit{True} & \textit{True} & \lp[0] & \jsmasmap{} & \identityloss{}\\193 & \adam{} & \textit{True} & \textit{True} & \lp[2] & \jsmasmap{} & \identityloss{}\\194 & \adam{} & \textit{True} & \textit{True} & \lp[\infty] & \jsmasmap{} & \identityloss{}\\195 & \adam{} & \textit{True} & \textit{True} & \lp[0] & \dfsmap{} & \identityloss{}\\196 & \adam{} & \textit{True} & \textit{True} & \lp[2] & \dfsmap{} & \identityloss{}\\197 & \adam{} & \textit{True} & \textit{True} & \lp[\infty] & \dfsmap{} & \identityloss{}\\198 & \adam{} & \textit{True} & \textit{True} & \lp[0] & \identitysmap{} & \crossentropy{}\\199 & \adam{} & \textit{True} & \textit{True} & \lp[2] & \identitysmap{} & \crossentropy{}\\200 & \adam{} & \textit{True} & \textit{True} & \lp[\infty] & \identitysmap{} & \crossentropy{}\\201 & \adam{} & \textit{True} & \textit{True} & \lp[0] & \jsmasmap{} & \crossentropy{}\\202 & \adam{} & \textit{True} & \textit{True} & \lp[2] & \jsmasmap{} & \crossentropy{}\\203 & \adam{} & \textit{True} & \textit{True} & \lp[\infty] & \jsmasmap{} & \crossentropy{}\\204 & \adam{} & \textit{True} & \textit{True} & \lp[0] & \dfsmap{} & \crossentropy{}\\205 & \adam{} & \textit{True} & \textit{True} & \lp[2] & \dfsmap{} & \crossentropy{}\\206 & \adam{} & \textit{True} & \textit{True} & \lp[\infty] & \dfsmap{} & \crossentropy{}\\207 & \adam{} & \textit{True} & \textit{True} & \lp[0] & \identitysmap{} & \cwloss{}\\208 & \adam{} & \textit{True} & \textit{True} & \lp[2] & \identitysmap{} & \cwloss{}\\209 & \adam{} & \textit{True} & \textit{True} & \lp[\infty] & \identitysmap{} & \cwloss{}\\210 & \adam{} & \textit{True} & \textit{True} & \lp[0] & \jsmasmap{} & \cwloss{}\\211 & \adam{} & \textit{True} & \textit{True} & \lp[2] & \jsmasmap{} & \cwloss{}\\212 & \adam{} & \textit{True} & \textit{True} & \lp[\infty] & \jsmasmap{} & \cwloss{}\\213 & \adam{} & \textit{True} & \textit{True} & \lp[0] & \dfsmap{} & \cwloss{}\\214 & \adam{} & \textit{True} & \textit{True} & \lp[2] & \dfsmap{} & \cwloss{}\\215 & \adam{} & \textit{True} & \textit{True} & \lp[\infty] & \dfsmap{} & \cwloss{}\\

==> figures/hypotheses.tex <==
1. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\lp{}-\mathtt{target}=\lp[0]\) & \num{< 2.2e-308} & \qty{100}{\percent} \\
2. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Dataset}=\mnist{}\) & \num{< 2.2e-308} & \qty{99}{\percent} \\
3. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Solver}=\adam{}\) & \num{< 2.2e-308} & \qty{99}{\percent} \\
4. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\lp{}-\mathtt{target}=\lp[\infty]\) & \num{< 2.2e-308} & \qty{99}{\percent} \\
5. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Dataset}=\fmnist{}\) & \num{< 2.2e-308} & \qty{97}{\percent} \\
6. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Saliency Map}=\dfsmapfull{}\) & \num{< 2.2e-308} & \qty{96}{\percent} \\
7. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Dataset}=\nslkdd{}\) & \num{< 2.2e-308} & \qty{96}{\percent} \\
8. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\rr{}=\textit{Disabled}\) & \num{< 2.2e-308} & \qty{95}{\percent} \\
9. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Loss}=\crossentropyfull{}\) & \num{< 2.2e-308} & \qty{95}{\percent} \\
10. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Loss}=\identitylossfull{}\) & \num{< 2.2e-308} & \qty{95}{\percent} \\
11. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Loss}=\cwlossfull{}\) & \num{< 2.2e-308} & \qty{94}{\percent} \\
12. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\rr{}=\textit{Enabled}\) & \num{< 2.2e-308} & \qty{94}{\percent} \\
13. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Saliency Map}=\jsmasmapfull{}\) & \num{< 2.2e-308} & \qty{94}{\percent} \\
14. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Saliency Map}=\identitysmapfull{}\) & \num{< 2.2e-308} & \qty{93}{\percent} \\
15. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Dataset}=\phishing{}\) & \num{< 2.2e-308} & \qty{92}{\percent} \\
16. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Dataset}=\phishing{}\) & \num{< 2.2e-308} & \qty{91}{\percent} \\
17. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Dataset}=\phishing{}\) & \num{< 2.2e-308} & \qty{90}{\percent} \\
18. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Solver}=\sgd{}\) & \num{< 2.2e-308} & \qty{90}{\percent} \\
19. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Dataset}=\unswnb{}\) & \num{< 2.2e-308} & \qty{90}{\percent} \\
20. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Dataset}=\nslkdd{}\) & \num{< 2.2e-308} & \qty{89}{\percent} \\
21. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Dataset}=\mnist{}\) & \num{< 2.2e-308} & \qty{89}{\percent} \\
22. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Loss}=\identitylossfull{}\) & \num{< 2.2e-308} & \qty{86}{\percent} \\
23. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\lp{}-\mathtt{target}=\lp[2]\) & \num{< 2.2e-308} & \qty{85}{\percent} \\
24. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Dataset}=\phishing{}\) & \num{< 2.2e-308} & \qty{84}{\percent} \\
25. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Dataset}=\nslkdd{}\) & \num{< 2.2e-308} & \qty{81}{\percent} \\
26. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\cov{}=\textit{Disabled}\) & \num{< 2.2e-308} & \qty{79}{\percent} \\
27. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\lp{}-\mathtt{target}=\lp[\infty]\) & \num{< 2.2e-308} & \qty{78}{\percent} \\
28. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Saliency Map}=\dfsmapfull{}\) & \num{< 2.2e-308} & \qty{78}{\percent} \\
29. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Saliency Map}=\identitysmapfull{}\) & \num{< 2.2e-308} & \qty{78}{\percent} \\
30. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Saliency Map}=\dfsmapfull{}\) & \num{< 2.2e-308} & \qty{77}{\percent} \\
31. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Solver}=\adam{}\) & \num{< 2.2e-308} & \qty{74}{\percent} \\
32. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Dataset}=\mnist{}\) & \num{< 2.2e-308} & \qty{74}{\percent} \\
33. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\lp{}-\mathtt{target}=\lp[\infty]\) & \num{< 2.2e-308} & \qty{73}{\percent} \\
34. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\cov{}=\textit{Enabled}\) & \num{< 2.2e-308} & \qty{73}{\percent} \\
35. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Loss}=\identitylossfull{}\) & \num{< 2.2e-308} & \qty{71}{\percent} \\
36. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\cov{}=\textit{Enabled}\) & \num{< 2.2e-308} & \qty{71}{\percent} \\
37. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Saliency Map}=\identitysmapfull{}\) & \num{< 2.2e-308} & \qty{71}{\percent} \\
38. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\lp{}-\mathtt{target}=\lp[0]\) & \num{< 2.2e-308} & \qty{70}{\percent} \\
39. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\cov{}=\textit{Enabled}\) & \num{< 2.2e-308} & \qty{70}{\percent} \\
40. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Solver}=\adam{}\) & \num{< 2.2e-308} & \qty{70}{\percent} \\
41. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\cov{}=\textit{Enabled}\) & \num{< 2.2e-308} & \qty{69}{\percent} \\
42. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\rr{}=\textit{Disabled}\) & \num{< 2.2e-308} & \qty{69}{\percent} \\
43. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\lp{}-\mathtt{target}=\lp[0]\) & \num{< 2.2e-308} & \qty{67}{\percent} \\
44. & \sgd{} & is better than &  \adam{} & when & \(\cov{}=\textit{Enabled}\) & \num{< 2.2e-308} & \qty{39}{\percent} \\
45. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Saliency Map}=\identitysmapfull{}\) & \num{< 2.2e-308} & \qty{37}{\percent} \\
46. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Loss}=\cwlossfull{}\) & \num{< 2.2e-308} & \qty{36}{\percent} \\
47. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Dataset}=\fmnist{}\) & \num{< 2.2e-308} & \qty{36}{\percent} \\
48. & \sgd{} & is better than &  \adam{} & when & \(\rr{}=\textit{Disabled}\) & \num{< 2.2e-308} & \qty{35}{\percent} \\
49. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Saliency Map}=\dfsmapfull{}\) & \num{< 2.2e-308} & \qty{35}{\percent} \\
50. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Loss}=\crossentropyfull{}\) & \num{< 2.2e-308} & \qty{34}{\percent} \\
51. & \lp[2] & is better than &  \lp[\infty] & when & \(\cov{}=\textit{Disabled}\) & \num{< 2.2e-308} & \qty{34}{\percent} \\
52. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Loss}=\identitylossfull{}\) & \num{< 2.2e-308} & \qty{32}{\percent} \\
53. & \lp[0] & is better than &  \lp[2] & when & \(\rr{}=\textit{Enabled}\) & \num{< 2.2e-308} & \qty{32}{\percent} \\
54. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Saliency Map}=\dfsmapfull{}\) & \num{< 2.2e-308} & \qty{31}{\percent} \\
55. & \sgd{} & is better than &  \adam{} & when & \(\rr{}=\textit{Enabled}\) & \num{< 2.2e-308} & \qty{30}{\percent} \\
56. & \sgd{} & is better than &  \adam{} & when & \(\lp{}-\mathtt{target}=\lp[2]\) & \num{< 2.2e-308} & \qty{30}{\percent} \\
57. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Loss}=\crossentropyfull{}\) & \num{< 2.2e-308} & \qty{29}{\percent} \\
58. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Dataset}=\mnist{}\) & \num{< 2.2e-308} & \qty{29}{\percent} \\
59. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Solver}=\sgd{}\) & \num{< 2.2e-308} & \qty{28}{\percent} \\
60. & \sgd{} & is better than &  \adam{} & when & \(\cov{}=\textit{Disabled}\) & \num{< 2.2e-308} & \qty{26}{\percent} \\
61. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Dataset}=\unswnb{}\) & \num{< 2.2e-308} & \qty{26}{\percent} \\
62. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Saliency Map}=\jsmasmapfull{}\) & \num{< 2.2e-308} & \qty{26}{\percent} \\
63. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Saliency Map}=\identitysmapfull{}\) & \num{< 2.2e-308} & \qty{25}{\percent} \\
64. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Solver}=\adam{}\) & \num{< 2.2e-308} & \qty{24}{\percent} \\
65. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Dataset}=\nslkdd{}\) & \num{< 2.2e-308} & \qty{23}{\percent} \\
66. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Solver}=\adam{}\) & \num{< 2.2e-308} & \qty{22}{\percent} \\
67. & \lp[0] & is better than &  \lp[\infty] & when & \(\rr{}=\textit{Disabled}\) & \num{< 2.2e-308} & \qty{22}{\percent} \\
68. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Loss}=\cwlossfull{}\) & \num{< 2.2e-308} & \qty{21}{\percent} \\
69. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Loss}=\crossentropyfull{}\) & \num{< 2.2e-308} & \qty{21}{\percent} \\
70. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Dataset}=\mnist{}\) & \num{< 2.2e-308} & \qty{20}{\percent} \\
71. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Loss}=\identitylossfull{}\) & \num{< 2.2e-308} & \qty{19}{\percent} \\
72. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Dataset}=\mnist{}\) & \num{< 2.2e-308} & \qty{19}{\percent} \\
73. & \lp[0] & is better than &  \lp[\infty] & when & \(\rr{}=\textit{Enabled}\) & \num{< 2.2e-308} & \qty{19}{\percent} \\
74. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Solver}=\sgd{}\) & \num{< 2.2e-308} & \qty{18}{\percent} \\
75. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Saliency Map}=\jsmasmapfull{}\) & \num{< 2.2e-308} & \qty{18}{\percent} \\
76. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Saliency Map}=\dfsmapfull{}\) & \num{< 2.2e-308} & \qty{18}{\percent} \\
77. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Dataset}=\phishing{}\) & \num{< 2.2e-308} & \qty{16}{\percent} \\
78. & \lp[0] & is better than &  \lp[2] & when & \(\cov{}=\textit{Enabled}\) & \num{< 2.2e-308} & \qty{10}{\percent} \\
79. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\cov{}=\textit{Enabled}\) & \num{< 2.2e-308} & \qty{6}{\percent} \\
80. & \lp[0] & is better than &  \lp[\infty] & when & \(\cov{}=\textit{Enabled}\) & \num{< 2.2e-308} & \qty{1}{\percent} \\
81. & \sgd{} & is better than &  \adam{} & when & \(\lp{}-\mathtt{target}=\lp[0]\) & \num{< 2.2e-308} & \qty{1}{\percent} \\
82. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Dataset}=\mnist{}\) & \num{< 0.01} & \qty{35}{\percent} \\
83. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\rr{}=\textit{Enabled}\) & \num{< 0.01} & \qty{67}{\percent} \\
84. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Dataset}=\mnist{}\) & \num{< 0.01} & \qty{37}{\percent} \\
85. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Dataset}=\fmnist{}\) & \num{< 0.01} & \qty{17}{\percent} \\
86. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Solver}=\sgd{}\) & \num{< 0.01} & \qty{66}{\percent} \\
87. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Dataset}=\phishing{}\) & \num{< 0.01} & \qty{80}{\percent} \\
88. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\rr{}=\textit{Disabled}\) & \num{< 0.01} & \qty{68}{\percent} \\
89. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Dataset}=\nslkdd{}\) & \num{< 0.01} & \qty{18}{\percent} \\
90. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\rr{}=\textit{Enabled}\) & \num{< 0.01} & \qty{67}{\percent} \\
91. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\lp{}-\mathtt{target}=\lp[0]\) & \num{< 0.01} & \qty{67}{\percent} \\
92. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\cov{}=\textit{Disabled}\) & \num{< 0.01} & \qty{66}{\percent} \\
93. & \lp[2] & is better than &  \lp[\infty] & when & \(\rr{}=\textit{Enabled}\) & \num{< 0.01} & \qty{42}{\percent} \\
94. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Dataset}=\phishing{}\) & \num{< 0.01} & \qty{27}{\percent} \\
95. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Dataset}=\phishing{}\) & \num{< 0.01} & \qty{75}{\percent} \\
96. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\rr{}=\textit{Enabled}\) & \num{< 0.01} & \qty{67}{\percent} \\
97. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Dataset}=\phishing{}\) & \num{< 0.01} & \qty{40}{\percent} \\
98. & \lp[2] & is better than &  \lp[\infty] & when & \(\rr{}=\textit{Disabled}\) & \num{< 0.01} & \qty{42}{\percent} \\
99. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Dataset}=\phishing{}\) & \num{< 0.01} & \qty{40}{\percent} \\
100. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\lp{}-\mathtt{target}=\lp[2]\) & \num{< 0.01} & \qty{68}{\percent} \\
101. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Dataset}=\mnist{}\) & \num{< 0.01} & \qty{26}{\percent} \\
102. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Solver}=\sgd{}\) & \num{< 0.01} & \qty{66}{\percent} \\
103. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Saliency Map}=\jsmasmapfull{}\) & \num{< 0.01} & \qty{67}{\percent} \\
104. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Solver}=\adam{}\) & \num{< 0.01} & \qty{45}{\percent} \\
105. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\lp{}-\mathtt{target}=\lp[2]\) & \num{< 0.01} & \qty{41}{\percent} \\
106. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Dataset}=\unswnb{}\) & \num{< 0.01} & \qty{73}{\percent} \\
107. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Saliency Map}=\dfsmapfull{}\) & \num{< 0.01} & \qty{40}{\percent} \\
108. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Dataset}=\unswnb{}\) & \num{< 0.01} & \qty{70}{\percent} \\
109. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Dataset}=\fmnist{}\) & \num{< 0.01} & \qty{26}{\percent} \\
110. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Loss}=\identitylossfull{}\) & \num{< 0.01} & \qty{31}{\percent} \\
111. & \lp[0] & is better than &  \lp[2] & when & \(\cov{}=\textit{Disabled}\) & \num{< 0.01} & \qty{57}{\percent} \\
112. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Dataset}=\fmnist{}\) & \num{< 0.01} & \qty{39}{\percent} \\
113. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Saliency Map}=\jsmasmapfull{}\) & \num{< 0.01} & \qty{30}{\percent} \\
114. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Dataset}=\nslkdd{}\) & \num{< 0.01} & \qty{41}{\percent} \\
115. & \sgd{} & is better than &  \adam{} & when & \(\lp{}-\mathtt{target}=\lp[\infty]\) & \num{< 0.01} & \qty{67}{\percent} \\
116. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Saliency Map}=\dfsmapfull{}\) & \num{< 0.01} & \qty{33}{\percent} \\
117. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Solver}=\sgd{}\) & \num{< 0.01} & \qty{41}{\percent} \\
118. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Saliency Map}=\identitysmapfull{}\) & \num{< 0.01} & \qty{43}{\percent} \\
119. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Loss}=\cwlossfull{}\) & \num{< 0.01} & \qty{33}{\percent} \\
120. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Loss}=\crossentropyfull{}\) & \num{< 0.01} & \qty{40}{\percent} \\
121. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Dataset}=\fmnist{}\) & \num{< 0.01} & \qty{30}{\percent} \\
122. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\lp{}-\mathtt{target}=\lp[\infty]\) & \num{< 0.01} & \qty{47}{\percent} \\
123. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Loss}=\cwlossfull{}\) & \num{< 0.01} & \qty{43}{\percent} \\
124. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Dataset}=\unswnb{}\) & \num{< 0.01} & \qty{70}{\percent} \\
125. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Loss}=\identitylossfull{}\) & \num{< 0.01} & \qty{45}{\percent} \\
126. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Dataset}=\fmnist{}\) & \num{< 0.01} & \qty{28}{\percent} \\
127. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\cov{}=\textit{Disabled}\) & \num{< 0.01} & \qty{64}{\percent} \\
128. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Dataset}=\nslkdd{}\) & \num{< 0.01} & \qty{65}{\percent} \\
129. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Saliency Map}=\jsmasmapfull{}\) & \num{< 0.01} & \qty{39}{\percent} \\
130. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\lp{}-\mathtt{target}=\lp[2]\) & \num{< 0.01} & \qty{58}{\percent} \\
131. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Dataset}=\nslkdd{}\) & \num{< 0.01} & \qty{65}{\percent} \\
132. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Solver}=\adam{}\) & \num{< 0.01} & \qty{58}{\percent} \\
133. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Saliency Map}=\dfsmapfull{}\) & \num{< 0.01} & \qty{61}{\percent} \\
134. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\lp{}-\mathtt{target}=\lp[\infty]\) & \num{< 0.01} & \qty{40}{\percent} \\
135. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Dataset}=\unswnb{}\) & \num{< 0.01} & \qty{45}{\percent} \\
136. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\lp{}-\mathtt{target}=\lp[0]\) & \num{< 0.01} & \qty{62}{\percent} \\
137. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\rr{}=\textit{Disabled}\) & \num{< 0.01} & \qty{61}{\percent} \\
138. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Saliency Map}=\identitysmapfull{}\) & \num{< 0.01} & \qty{46}{\percent} \\
139. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\rr{}=\textit{Disabled}\) & \num{< 0.01} & \qty{60}{\percent} \\
140. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Loss}=\cwlossfull{}\) & \num{< 0.01} & \qty{46}{\percent} \\
141. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.7\) & \num{< 0.01} & \qty{98}{\percent} \\
142. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.5\) & \num{< 0.01} & \qty{98}{\percent} \\
143. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.6\) & \num{< 0.01} & \qty{98}{\percent} \\
144. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.8\) & \num{< 0.01} & \qty{98}{\percent} \\
145. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.4\) & \num{< 0.01} & \qty{98}{\percent} \\
146. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.3\) & \num{< 0.01} & \qty{98}{\percent} \\
147. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.2\) & \num{< 0.01} & \qty{98}{\percent} \\
148. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.9\) & \num{< 0.01} & \qty{98}{\percent} \\
149. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.0\) & \num{< 0.01} & \qty{98}{\percent} \\
150. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.1\) & \num{< 0.01} & \qty{98}{\percent} \\
151. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.1\) & \num{< 0.01} & \qty{98}{\percent} \\
152. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.2\) & \num{< 0.01} & \qty{98}{\percent} \\
153. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.0\) & \num{< 0.01} & \qty{97}{\percent} \\
154. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.3\) & \num{< 0.01} & \qty{98}{\percent} \\
155. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.4\) & \num{< 0.01} & \qty{98}{\percent} \\
156. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.5\) & \num{< 0.01} & \qty{98}{\percent} \\
157. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.6\) & \num{< 0.01} & \qty{98}{\percent} \\
158. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.7\) & \num{< 0.01} & \qty{98}{\percent} \\
159. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.8\) & \num{< 0.01} & \qty{98}{\percent} \\
160. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.9\) & \num{< 0.01} & \qty{98}{\percent} \\
161. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+2.0\) & \num{< 0.01} & \qty{98}{\percent} \\
162. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Dataset}=\nslkdd{}\) & \num{< 0.01} & \qty{31}{\percent} \\
163. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Loss}=\crossentropyfull{}\) & \num{< 0.01} & \qty{37}{\percent} \\
164. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Solver}=\sgd{}\) & \num{< 0.01} & \qty{43}{\percent} \\
165. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Loss}=\identitylossfull{}\) & \num{< 0.01} & \qty{45}{\percent} \\
166. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Solver}=\adam{}\) & \num{< 0.01} & \qty{62}{\percent} \\
167. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Loss}=\identitylossfull{}\) & \num{< 0.01} & \qty{40}{\percent} \\
168. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Saliency Map}=\identitysmapfull{}\) & \num{< 0.01} & \qty{37}{\percent} \\
169. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.7\) & \num{< 0.01} & \qty{92}{\percent} \\
170. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.6\) & \num{< 0.01} & \qty{92}{\percent} \\
171. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.8\) & \num{< 0.01} & \qty{92}{\percent} \\
172. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.9\) & \num{< 0.01} & \qty{92}{\percent} \\
173. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.5\) & \num{< 0.01} & \qty{92}{\percent} \\
174. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+2.0\) & \num{< 0.01} & \qty{92}{\percent} \\
175. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Dataset}=\unswnb{}\) & \num{< 0.01} & \qty{31}{\percent} \\
176. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.4\) & \num{< 0.01} & \qty{92}{\percent} \\
177. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.3\) & \num{< 0.01} & \qty{92}{\percent} \\
178. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.2\) & \num{< 0.01} & \qty{92}{\percent} \\
179. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+2.0\) & \num{< 0.01} & \qty{94}{\percent} \\
180. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.1\) & \num{< 0.01} & \qty{92}{\percent} \\
181. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.0\) & \num{< 0.01} & \qty{92}{\percent} \\
182. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.9\) & \num{< 0.01} & \qty{94}{\percent} \\
183. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.9\) & \num{< 0.01} & \qty{93}{\percent} \\
184. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.8\) & \num{< 0.01} & \qty{94}{\percent} \\
185. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.8\) & \num{< 0.01} & \qty{93}{\percent} \\
186. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.7\) & \num{< 0.01} & \qty{94}{\percent} \\
187. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.6\) & \num{< 0.01} & \qty{94}{\percent} \\
188. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.7\) & \num{< 0.01} & \qty{93}{\percent} \\
189. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\cov{}=\textit{Disabled}\) & \num{< 0.01} & \qty{56}{\percent} \\
190. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.5\) & \num{< 0.01} & \qty{93}{\percent} \\
191. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.6\) & \num{< 0.01} & \qty{93}{\percent} \\
192. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.4\) & \num{< 0.01} & \qty{93}{\percent} \\
193. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\rr{}=\textit{Disabled}\) & \num{< 0.01} & \qty{56}{\percent} \\
194. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.3\) & \num{< 0.01} & \qty{93}{\percent} \\
195. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.2\) & \num{< 0.01} & \qty{93}{\percent} \\
196. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.5\) & \num{< 0.01} & \qty{93}{\percent} \\
197. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.1\) & \num{< 0.01} & \qty{93}{\percent} \\
198. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.0\) & \num{< 0.01} & \qty{92}{\percent} \\
199. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.4\) & \num{< 0.01} & \qty{93}{\percent} \\
200. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.9\) & \num{< 0.01} & \qty{92}{\percent} \\
201. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.8\) & \num{< 0.01} & \qty{92}{\percent} \\
202. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.3\) & \num{< 0.01} & \qty{93}{\percent} \\
203. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.7\) & \num{< 0.01} & \qty{92}{\percent} \\
204. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Dataset}=\unswnb{}\) & \num{< 0.01} & \qty{38}{\percent} \\
205. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.6\) & \num{< 0.01} & \qty{92}{\percent} \\
206. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Solver}=\sgd{}\) & \num{< 0.01} & \qty{58}{\percent} \\
207. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Dataset}=\mnist{}\) & \num{< 0.01} & \qty{45}{\percent} \\
208. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.2\) & \num{< 0.01} & \qty{93}{\percent} \\
209. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.5\) & \num{< 0.01} & \qty{92}{\percent} \\
210. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Dataset}=\unswnb{}\) & \num{< 0.01} & \qty{64}{\percent} \\
211. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.4\) & \num{< 0.01} & \qty{92}{\percent} \\
212. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.0\) & \num{< 0.01} & \qty{85}{\percent} \\
213. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.1\) & \num{< 0.01} & \qty{93}{\percent} \\
214. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.3\) & \num{< 0.01} & \qty{92}{\percent} \\
215. & \lp[2] & is better than &  \lp[\infty] & when & \(\cov{}=\textit{Enabled}\) & \num{< 0.01} & \qty{50}{\percent} \\
216. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.0\) & \num{< 0.01} & \qty{93}{\percent} \\
217. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.2\) & \num{< 0.01} & \qty{92}{\percent} \\
218. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.1\) & \num{< 0.01} & \qty{92}{\percent} \\
219. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\lp{}-\mathtt{target}=\lp[2]\) & \num{< 0.01} & \qty{63}{\percent} \\
220. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.0\) & \num{< 0.01} & \qty{92}{\percent} \\
221. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Solver}=\sgd{}\) & \num{< 0.01} & \qty{61}{\percent} \\
222. & \lp[0] & is better than &  \lp[2] & when & \(\rr{}=\textit{Disabled}\) & \num{< 0.01} & \qty{35}{\percent} \\
223. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\rr{}=\textit{Enabled}\) & \num{< 0.01} & \qty{56}{\percent} \\
224. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.0\) & \num{< 0.01} & \qty{0}{\percent} \\
225. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.1\) & \num{< 0.01} & \qty{0}{\percent} \\
226. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.2\) & \num{< 0.01} & \qty{0}{\percent} \\
227. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.3\) & \num{< 0.01} & \qty{0}{\percent} \\
228. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.4\) & \num{< 0.01} & \qty{0}{\percent} \\
229. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.5\) & \num{< 0.01} & \qty{1}{\percent} \\
230. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.6\) & \num{< 0.01} & \qty{1}{\percent} \\
231. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.7\) & \num{< 0.01} & \qty{1}{\percent} \\
232. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.8\) & \num{< 0.01} & \qty{1}{\percent} \\
233. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.9\) & \num{< 0.01} & \qty{1}{\percent} \\
234. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.0\) & \num{< 0.01} & \qty{1}{\percent} \\
235. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.1\) & \num{< 0.01} & \qty{1}{\percent} \\
236. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.2\) & \num{< 0.01} & \qty{1}{\percent} \\
237. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.3\) & \num{< 0.01} & \qty{1}{\percent} \\
238. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.4\) & \num{< 0.01} & \qty{1}{\percent} \\
239. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.5\) & \num{< 0.01} & \qty{1}{\percent} \\
240. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.6\) & \num{< 0.01} & \qty{1}{\percent} \\
241. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.7\) & \num{< 0.01} & \qty{1}{\percent} \\
242. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.8\) & \num{< 0.01} & \qty{1}{\percent} \\
243. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.9\) & \num{< 0.01} & \qty{1}{\percent} \\
244. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[inf]+2.0\) & \num{< 0.01} & \qty{1}{\percent} \\
245. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.4\) & \num{< 0.01} & \qty{23}{\percent} \\
246. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.5\) & \num{< 0.01} & \qty{23}{\percent} \\
247. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.7\) & \num{< 0.01} & \qty{24}{\percent} \\
248. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.8\) & \num{< 0.01} & \qty{24}{\percent} \\
249. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.6\) & \num{< 0.01} & \qty{23}{\percent} \\
250. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.9\) & \num{< 0.01} & \qty{24}{\percent} \\
251. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.3\) & \num{< 0.01} & \qty{24}{\percent} \\
252. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.0\) & \num{< 0.01} & \qty{24}{\percent} \\
253. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.2\) & \num{< 0.01} & \qty{24}{\percent} \\
254. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.1\) & \num{< 0.01} & \qty{24}{\percent} \\
255. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.3\) & \num{< 0.01} & \qty{24}{\percent} \\
256. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.4\) & \num{< 0.01} & \qty{24}{\percent} \\
257. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.5\) & \num{< 0.01} & \qty{24}{\percent} \\
258. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.2\) & \num{< 0.01} & \qty{24}{\percent} \\
259. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.0\) & \num{< 0.01} & \qty{94}{\percent} \\
260. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.6\) & \num{< 0.01} & \qty{24}{\percent} \\
261. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.7\) & \num{< 0.01} & \qty{25}{\percent} \\
262. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.8\) & \num{< 0.01} & \qty{24}{\percent} \\
263. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.1\) & \num{< 0.01} & \qty{25}{\percent} \\
264. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.9\) & \num{< 0.01} & \qty{24}{\percent} \\
265. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+2.0\) & \num{< 0.01} & \qty{25}{\percent} \\
266. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\cov{}=\textit{Disabled}\) & \num{< 0.01} & \qty{43}{\percent} \\
267. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.0\) & \num{< 0.01} & \qty{26}{\percent} \\
268. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[2]+2.0\) & \num{< 0.01} & \qty{8}{\percent} \\
269. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.9\) & \num{< 0.01} & \qty{8}{\percent} \\
270. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.8\) & \num{< 0.01} & \qty{9}{\percent} \\
271. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.7\) & \num{< 0.01} & \qty{9}{\percent} \\
272. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.6\) & \num{< 0.01} & \qty{9}{\percent} \\
273. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.5\) & \num{< 0.01} & \qty{9}{\percent} \\
274. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.4\) & \num{< 0.01} & \qty{9}{\percent} \\
275. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.3\) & \num{< 0.01} & \qty{9}{\percent} \\
276. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.2\) & \num{< 0.01} & \qty{10}{\percent} \\
277. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Saliency Map}=\jsmasmapfull{}\) & \num{< 0.01} & \qty{48}{\percent} \\
278. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.1\) & \num{< 0.01} & \qty{10}{\percent} \\
279. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Dataset}=\unswnb{}\) & \num{< 0.01} & \qty{30}{\percent} \\
280. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.0\) & \num{< 0.01} & \qty{11}{\percent} \\
281. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\lp{}-\mathtt{target}=\lp[0]\) & \num{< 0.01} & \qty{41}{\percent} \\
282. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.9\) & \num{< 0.01} & \qty{11}{\percent} \\
283. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.8\) & \num{< 0.01} & \qty{11}{\percent} \\
284. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.7\) & \num{< 0.01} & \qty{11}{\percent} \\
285. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Dataset}=\unswnb{}\) & \num{< 0.01} & \qty{51}{\percent} \\
286. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.6\) & \num{< 0.01} & \qty{11}{\percent} \\
287. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.5\) & \num{< 0.01} & \qty{13}{\percent} \\
288. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Saliency Map}=\jsmasmapfull{}\) & \num{< 0.01} & \qty{45}{\percent} \\
289. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.4\) & \num{< 0.01} & \qty{15}{\percent} \\
290. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Dataset}=\fmnist{}\) & \num{< 0.01} & \qty{54}{\percent} \\
291. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Solver}=\adam{}\) & \num{< 0.01} & \qty{56}{\percent} \\
292. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.3\) & \num{< 0.01} & \qty{16}{\percent} \\
293. & \lp[0] & is better than &  \lp[\infty] & when & \(\cov{}=\textit{Disabled}\) & \num{< 0.01} & \qty{39}{\percent} \\
294. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.2\) & \num{< 0.01} & \qty{17}{\percent} \\
295. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\rr{}=\textit{Enabled}\) & \num{< 0.01} & \qty{46}{\percent} \\
296. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\cov{}=\textit{Enabled}\) & \num{< 0.01} & \qty{58}{\percent} \\
297. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Solver}=\sgd{}\) & \num{< 0.01} & \qty{54}{\percent} \\
298. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+2.0\) & \num{< 0.01} & \qty{32}{\percent} \\
299. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Solver}=\sgd{}\) & \num{< 0.01} & \qty{43}{\percent} \\
300. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.1\) & \num{< 0.01} & \qty{21}{\percent} \\
301. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.9\) & \num{< 0.01} & \qty{33}{\percent} \\
302. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.1\) & \num{< 0.01} & \qty{20}{\percent} \\
303. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Dataset}=\nslkdd{}\) & \num{< 0.01} & \qty{46}{\percent} \\
304. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.2\) & \num{< 0.01} & \qty{21}{\percent} \\
305. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.0\) & \num{< 0.01} & \qty{84}{\percent} \\
306. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.1\) & \num{< 0.01} & \qty{31}{\percent} \\
307. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.0\) & \num{< 0.01} & \qty{22}{\percent} \\
308. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.3\) & \num{< 0.01} & \qty{22}{\percent} \\
309. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\lp{}-\mathtt{target}=\lp[\infty]\) & \num{< 0.01} & \qty{56}{\percent} \\
310. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.8\) & \num{< 0.01} & \qty{33}{\percent} \\
311. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.4\) & \num{< 0.01} & \qty{22}{\percent} \\
312. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.5\) & \num{< 0.01} & \qty{22}{\percent} \\
313. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.6\) & \num{< 0.01} & \qty{23}{\percent} \\
314. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.7\) & \num{< 0.01} & \qty{22}{\percent} \\
315. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.7\) & \num{< 0.01} & \qty{33}{\percent} \\
316. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.2\) & \num{< 0.01} & \qty{31}{\percent} \\
317. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.8\) & \num{< 0.01} & \qty{22}{\percent} \\
318. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.9\) & \num{< 0.01} & \qty{23}{\percent} \\
319. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.0\) & \num{< 0.01} & \qty{23}{\percent} \\
320. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.1\) & \num{< 0.01} & \qty{23}{\percent} \\
321. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.6\) & \num{< 0.01} & \qty{34}{\percent} \\
322. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.2\) & \num{< 0.01} & \qty{23}{\percent} \\
323. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.0\) & \num{< 0.01} & \qty{32}{\percent} \\
324. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.3\) & \num{< 0.01} & \qty{24}{\percent} \\
325. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\rr{}=\textit{Enabled}\) & \num{< 0.01} & \qty{54}{\percent} \\
326. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Dataset}=\phishing{}\) & \num{< 0.01} & \qty{40}{\percent} \\
327. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.5\) & \num{< 0.01} & \qty{35}{\percent} \\
328. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.4\) & \num{< 0.01} & \qty{24}{\percent} \\
329. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.3\) & \num{< 0.01} & \qty{32}{\percent} \\
330. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.5\) & \num{< 0.01} & \qty{24}{\percent} \\
331. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.4\) & \num{< 0.01} & \qty{35}{\percent} \\
332. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.6\) & \num{< 0.01} & \qty{25}{\percent} \\
333. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.7\) & \num{< 0.01} & \qty{25}{\percent} \\
334. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.3\) & \num{< 0.01} & \qty{36}{\percent} \\
335. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.8\) & \num{< 0.01} & \qty{25}{\percent} \\
336. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.2\) & \num{< 0.01} & \qty{35}{\percent} \\
337. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.9\) & \num{< 0.01} & \qty{25}{\percent} \\
338. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.4\) & \num{< 0.01} & \qty{34}{\percent} \\
339. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[inf]+2.0\) & \num{< 0.01} & \qty{24}{\percent} \\
340. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.1\) & \num{< 0.01} & \qty{36}{\percent} \\
341. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.0\) & \num{< 0.01} & \qty{37}{\percent} \\
342. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.5\) & \num{< 0.01} & \qty{34}{\percent} \\
343. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.9\) & \num{< 0.01} & \qty{37}{\percent} \\
344. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.8\) & \num{< 0.01} & \qty{37}{\percent} \\
345. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.6\) & \num{< 0.01} & \qty{34}{\percent} \\
346. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.0\) & \num{< 0.01} & \qty{25}{\percent} \\
347. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.7\) & \num{< 0.01} & \qty{38}{\percent} \\
348. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.7\) & \num{< 0.01} & \qty{34}{\percent} \\
349. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+2.0\) & \num{< 0.01} & \qty{34}{\percent} \\
350. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.6\) & \num{< 0.01} & \qty{37}{\percent} \\
351. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.9\) & \num{< 0.01} & \qty{34}{\percent} \\
352. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\lp{}-\mathtt{target}=\lp[\infty]\) & \num{< 0.01} & \qty{59}{\percent} \\
353. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.8\) & \num{< 0.01} & \qty{35}{\percent} \\
354. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Saliency Map}=\identitysmapfull{}\) & \num{< 0.01} & \qty{57}{\percent} \\
355. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[2]+2.0\) & \num{< 0.01} & \qty{20}{\percent} \\
356. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.8\) & \num{< 0.01} & \qty{34}{\percent} \\
357. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.9\) & \num{< 0.01} & \qty{21}{\percent} \\
358. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.7\) & \num{< 0.01} & \qty{34}{\percent} \\
359. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.9\) & \num{< 0.01} & \qty{34}{\percent} \\
360. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.5\) & \num{< 0.01} & \qty{38}{\percent} \\
361. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.6\) & \num{< 0.01} & \qty{34}{\percent} \\
362. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[inf]+2.0\) & \num{< 0.01} & \qty{20}{\percent} \\
363. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.8\) & \num{< 0.01} & \qty{21}{\percent} \\
364. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.0\) & \num{< 0.01} & \qty{35}{\percent} \\
365. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.5\) & \num{< 0.01} & \qty{34}{\percent} \\
366. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.9\) & \num{< 0.01} & \qty{20}{\percent} \\
367. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.1\) & \num{< 0.01} & \qty{35}{\percent} \\
368. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.7\) & \num{< 0.01} & \qty{23}{\percent} \\
369. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.4\) & \num{< 0.01} & \qty{34}{\percent} \\
370. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.2\) & \num{< 0.01} & \qty{35}{\percent} \\
371. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.8\) & \num{< 0.01} & \qty{20}{\percent} \\
372. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.3\) & \num{< 0.01} & \qty{35}{\percent} \\
373. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.3\) & \num{< 0.01} & \qty{35}{\percent} \\
374. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.4\) & \num{< 0.01} & \qty{39}{\percent} \\
375. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.7\) & \num{< 0.01} & \qty{20}{\percent} \\
376. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.6\) & \num{< 0.01} & \qty{23}{\percent} \\
377. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.4\) & \num{< 0.01} & \qty{35}{\percent} \\
378. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+2.0\) & \num{< 0.01} & \qty{77}{\percent} \\
379. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.2\) & \num{< 0.01} & \qty{35}{\percent} \\
380. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.9\) & \num{< 0.01} & \qty{77}{\percent} \\
381. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.6\) & \num{< 0.01} & \qty{19}{\percent} \\
382. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.5\) & \num{< 0.01} & \qty{35}{\percent} \\
383. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.8\) & \num{< 0.01} & \qty{77}{\percent} \\
384. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.5\) & \num{< 0.01} & \qty{24}{\percent} \\
385. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.7\) & \num{< 0.01} & \qty{77}{\percent} \\
386. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.1\) & \num{< 0.01} & \qty{35}{\percent} \\
387. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.6\) & \num{< 0.01} & \qty{35}{\percent} \\
388. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.6\) & \num{< 0.01} & \qty{77}{\percent} \\
389. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.5\) & \num{< 0.01} & \qty{19}{\percent} \\
390. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.5\) & \num{< 0.01} & \qty{76}{\percent} \\
391. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.3\) & \num{< 0.01} & \qty{40}{\percent} \\
392. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.7\) & \num{< 0.01} & \qty{35}{\percent} \\
393. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.4\) & \num{< 0.01} & \qty{77}{\percent} \\
394. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Dataset}=\fmnist{}\) & \num{< 0.01} & \qty{51}{\percent} \\
395. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.0\) & \num{< 0.01} & \qty{35}{\percent} \\
396. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.4\) & \num{< 0.01} & \qty{19}{\percent} \\
397. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.4\) & \num{< 0.01} & \qty{25}{\percent} \\
398. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.3\) & \num{< 0.01} & \qty{77}{\percent} \\
399. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.8\) & \num{< 0.01} & \qty{35}{\percent} \\
400. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.2\) & \num{< 0.01} & \qty{77}{\percent} \\
401. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.9\) & \num{< 0.01} & \qty{35}{\percent} \\
402. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.1\) & \num{< 0.01} & \qty{77}{\percent} \\
403. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.9\) & \num{< 0.01} & \qty{35}{\percent} \\
404. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.3\) & \num{< 0.01} & \qty{25}{\percent} \\
405. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.3\) & \num{< 0.01} & \qty{21}{\percent} \\
406. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.0\) & \num{< 0.01} & \qty{76}{\percent} \\
407. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Threat\ Model}=\lp[2]+2.0\) & \num{< 0.01} & \qty{35}{\percent} \\
408. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.8\) & \num{< 0.01} & \qty{36}{\percent} \\
409. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.2\) & \num{< 0.01} & \qty{21}{\percent} \\
410. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.2\) & \num{< 0.01} & \qty{42}{\percent} \\
411. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.9\) & \num{< 0.01} & \qty{76}{\percent} \\
412. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.2\) & \num{< 0.01} & \qty{25}{\percent} \\
413. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.0\) & \num{< 0.01} & \qty{26}{\percent} \\
414. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.1\) & \num{< 0.01} & \qty{21}{\percent} \\
415. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.8\) & \num{< 0.01} & \qty{76}{\percent} \\
416. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Dataset}=\fmnist{}\) & \num{< 0.01} & \qty{51}{\percent} \\
417. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.7\) & \num{< 0.01} & \qty{37}{\percent} \\
418. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.0\) & \num{< 0.01} & \qty{35}{\percent} \\
419. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.1\) & \num{< 0.01} & \qty{25}{\percent} \\
420. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.0\) & \num{< 0.01} & \qty{21}{\percent} \\
421. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.7\) & \num{< 0.01} & \qty{76}{\percent} \\
422. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.1\) & \num{< 0.01} & \qty{43}{\percent} \\
423. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.6\) & \num{< 0.01} & \qty{36}{\percent} \\
424. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.1\) & \num{< 0.01} & \qty{58}{\percent} \\
425. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.9\) & \num{< 0.01} & \qty{21}{\percent} \\
426. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.1\) & \num{< 0.01} & \qty{36}{\percent} \\
427. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.0\) & \num{< 0.01} & \qty{26}{\percent} \\
428. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.6\) & \num{< 0.01} & \qty{75}{\percent} \\
429. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.5\) & \num{< 0.01} & \qty{37}{\percent} \\
430. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.8\) & \num{< 0.01} & \qty{22}{\percent} \\
431. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.5\) & \num{< 0.01} & \qty{75}{\percent} \\
432. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.9\) & \num{< 0.01} & \qty{27}{\percent} \\
433. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.4\) & \num{< 0.01} & \qty{37}{\percent} \\
434. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.0\) & \num{< 0.01} & \qty{44}{\percent} \\
435. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.7\) & \num{< 0.01} & \qty{22}{\percent} \\
436. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.4\) & \num{< 0.01} & \qty{74}{\percent} \\
437. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.3\) & \num{< 0.01} & \qty{37}{\percent} \\
438. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+2.0\) & \num{< 0.01} & \qty{75}{\percent} \\
439. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.8\) & \num{< 0.01} & \qty{27}{\percent} \\
440. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.6\) & \num{< 0.01} & \qty{21}{\percent} \\
441. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.9\) & \num{< 0.01} & \qty{74}{\percent} \\
442. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.8\) & \num{< 0.01} & \qty{74}{\percent} \\
443. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.2\) & \num{< 0.01} & \qty{37}{\percent} \\
444. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.7\) & \num{< 0.01} & \qty{73}{\percent} \\
445. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.6\) & \num{< 0.01} & \qty{73}{\percent} \\
446. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+2.0\) & \num{< 0.01} & \qty{70}{\percent} \\
447. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.2\) & \num{< 0.01} & \qty{37}{\percent} \\
448. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+2.0\) & \num{< 0.01} & \qty{77}{\percent} \\
449. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.9\) & \num{< 0.01} & \qty{77}{\percent} \\
450. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.5\) & \num{< 0.01} & \qty{22}{\percent} \\
451. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.8\) & \num{< 0.01} & \qty{77}{\percent} \\
452. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.5\) & \num{< 0.01} & \qty{72}{\percent} \\
453. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.9\) & \num{< 0.01} & \qty{70}{\percent} \\
454. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.7\) & \num{< 0.01} & \qty{28}{\percent} \\
455. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.7\) & \num{< 0.01} & \qty{76}{\percent} \\
456. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.6\) & \num{< 0.01} & \qty{77}{\percent} \\
457. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.3\) & \num{< 0.01} & \qty{73}{\percent} \\
458. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.5\) & \num{< 0.01} & \qty{76}{\percent} \\
459. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.8\) & \num{< 0.01} & \qty{70}{\percent} \\
460. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.4\) & \num{< 0.01} & \qty{72}{\percent} \\
461. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.2\) & \num{< 0.01} & \qty{56}{\percent} \\
462. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.4\) & \num{< 0.01} & \qty{76}{\percent} \\
463. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.3\) & \num{< 0.01} & \qty{76}{\percent} \\
464. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.2\) & \num{< 0.01} & \qty{76}{\percent} \\
465. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\cov{}=\textit{Enabled}\) & \num{< 0.01} & \qty{46}{\percent} \\
466. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.7\) & \num{< 0.01} & \qty{70}{\percent} \\
467. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.1\) & \num{< 0.01} & \qty{76}{\percent} \\
468. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+2.0\) & \num{< 0.01} & \qty{69}{\percent} \\
469. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.3\) & \num{< 0.01} & \qty{72}{\percent} \\
470. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.9\) & \num{< 0.01} & \qty{69}{\percent} \\
471. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.1\) & \num{< 0.01} & \qty{37}{\percent} \\
472. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.8\) & \num{< 0.01} & \qty{69}{\percent} \\
473. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.0\) & \num{< 0.01} & \qty{76}{\percent} \\
474. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.7\) & \num{< 0.01} & \qty{68}{\percent} \\
475. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.6\) & \num{< 0.01} & \qty{70}{\percent} \\
476. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.6\) & \num{< 0.01} & \qty{68}{\percent} \\
477. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.9\) & \num{< 0.01} & \qty{76}{\percent} \\
478. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.5\) & \num{< 0.01} & \qty{68}{\percent} \\
479. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.2\) & \num{< 0.01} & \qty{72}{\percent} \\
480. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.4\) & \num{< 0.01} & \qty{68}{\percent} \\
481. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.8\) & \num{< 0.01} & \qty{75}{\percent} \\
482. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.3\) & \num{< 0.01} & \qty{38}{\percent} \\
483. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.3\) & \num{< 0.01} & \qty{68}{\percent} \\
484. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.5\) & \num{< 0.01} & \qty{70}{\percent} \\
485. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.2\) & \num{< 0.01} & \qty{68}{\percent} \\
486. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.4\) & \num{< 0.01} & \qty{24}{\percent} \\
487. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.1\) & \num{< 0.01} & \qty{68}{\percent} \\
488. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.0\) & \num{< 0.01} & \qty{67}{\percent} \\
489. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.7\) & \num{< 0.01} & \qty{69}{\percent} \\
490. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.2\) & \num{< 0.01} & \qty{73}{\percent} \\
491. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.5\) & \num{< 0.01} & \qty{69}{\percent} \\
492. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.9\) & \num{< 0.01} & \qty{68}{\percent} \\
493. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.6\) & \num{< 0.01} & \qty{69}{\percent} \\
494. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.8\) & \num{< 0.01} & \qty{68}{\percent} \\
495. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.6\) & \num{< 0.01} & \qty{28}{\percent} \\
496. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.1\) & \num{< 0.01} & \qty{71}{\percent} \\
497. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.4\) & \num{< 0.01} & \qty{69}{\percent} \\
498. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.7\) & \num{< 0.01} & \qty{75}{\percent} \\
499. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.4\) & \num{< 0.01} & \qty{70}{\percent} \\
500. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Dataset}=\mnist{}\) & \num{< 0.01} & \qty{52}{\percent} \\
501. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.0\) & \num{< 0.01} & \qty{38}{\percent} \\
502. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.3\) & \num{< 0.01} & \qty{70}{\percent} \\
503. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.3\) & \num{< 0.01} & \qty{69}{\percent} \\
504. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.0\) & \num{< 0.01} & \qty{71}{\percent} \\
505. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.6\) & \num{< 0.01} & \qty{74}{\percent} \\
506. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.2\) & \num{< 0.01} & \qty{69}{\percent} \\
507. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.2\) & \num{< 0.01} & \qty{71}{\percent} \\
508. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.1\) & \num{< 0.01} & \qty{33}{\percent} \\
509. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.3\) & \num{< 0.01} & \qty{26}{\percent} \\
510. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.1\) & \num{< 0.01} & \qty{69}{\percent} \\
511. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.9\) & \num{< 0.01} & \qty{71}{\percent} \\
512. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.4\) & \num{< 0.01} & \qty{39}{\percent} \\
513. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.5\) & \num{< 0.01} & \qty{73}{\percent} \\
514. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.1\) & \num{< 0.01} & \qty{73}{\percent} \\
515. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.5\) & \num{< 0.01} & \qty{29}{\percent} \\
516. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.0\) & \num{< 0.01} & \qty{68}{\percent} \\
517. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.0\) & \num{< 0.01} & \qty{28}{\percent} \\
518. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.3\) & \num{< 0.01} & \qty{55}{\percent} \\
519. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.8\) & \num{< 0.01} & \qty{70}{\percent} \\
520. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+2.0\) & \num{< 0.01} & \qty{70}{\percent} \\
521. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.9\) & \num{< 0.01} & \qty{68}{\percent} \\
522. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Dataset}=\nslkdd{}\) & \num{< 0.01} & \qty{45}{\percent} \\
523. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.9\) & \num{< 0.01} & \qty{70}{\percent} \\
524. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.8\) & \num{< 0.01} & \qty{70}{\percent} \\
525. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.7\) & \num{< 0.01} & \qty{70}{\percent} \\
526. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.1\) & \num{< 0.01} & \qty{53}{\percent} \\
527. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.0\) & \num{< 0.01} & \qty{71}{\percent} \\
528. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.1\) & \num{< 0.01} & \qty{72}{\percent} \\
529. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.6\) & \num{< 0.01} & \qty{69}{\percent} \\
530. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.9\) & \num{< 0.01} & \qty{71}{\percent} \\
531. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.1\) & \num{< 0.01} & \qty{70}{\percent} \\
532. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.5\) & \num{< 0.01} & \qty{69}{\percent} \\
533. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.4\) & \num{< 0.01} & \qty{72}{\percent} \\
534. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.5\) & \num{< 0.01} & \qty{40}{\percent} \\
535. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.8\) & \num{< 0.01} & \qty{67}{\percent} \\
536. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.2\) & \num{< 0.01} & \qty{69}{\percent} \\
537. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.4\) & \num{< 0.01} & \qty{69}{\percent} \\
538. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.3\) & \num{< 0.01} & \qty{72}{\percent} \\
539. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+2.0\) & \num{< 0.01} & \qty{71}{\percent} \\
540. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.3\) & \num{< 0.01} & \qty{69}{\percent} \\
541. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.2\) & \num{< 0.01} & \qty{27}{\percent} \\
542. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.8\) & \num{< 0.01} & \qty{69}{\percent} \\
543. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.9\) & \num{< 0.01} & \qty{70}{\percent} \\
544. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.7\) & \num{< 0.01} & \qty{68}{\percent} \\
545. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.8\) & \num{< 0.01} & \qty{70}{\percent} \\
546. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.7\) & \num{< 0.01} & \qty{66}{\percent} \\
547. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Threat\ Model}=\lp[0]+2.0\) & \num{< 0.01} & \qty{38}{\percent} \\
548. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+2.0\) & \num{< 0.01} & \qty{65}{\percent} \\
549. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.7\) & \num{< 0.01} & \qty{70}{\percent} \\
550. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.4\) & \num{< 0.01} & \qty{30}{\percent} \\
551. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.1\) & \num{< 0.01} & \qty{53}{\percent} \\
552. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.9\) & \num{< 0.01} & \qty{38}{\percent} \\
553. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.2\) & \num{< 0.01} & \qty{72}{\percent} \\
554. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.8\) & \num{< 0.01} & \qty{38}{\percent} \\
555. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.9\) & \num{< 0.01} & \qty{66}{\percent} \\
556. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.7\) & \num{< 0.01} & \qty{69}{\percent} \\
557. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.7\) & \num{< 0.01} & \qty{38}{\percent} \\
558. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.6\) & \num{< 0.01} & \qty{39}{\percent} \\
559. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.6\) & \num{< 0.01} & \qty{69}{\percent} \\
560. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.8\) & \num{< 0.01} & \qty{66}{\percent} \\
561. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.4\) & \num{< 0.01} & \qty{55}{\percent} \\
562. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.5\) & \num{< 0.01} & \qty{39}{\percent} \\
563. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.6\) & \num{< 0.01} & \qty{41}{\percent} \\
564. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.4\) & \num{< 0.01} & \qty{39}{\percent} \\
565. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.7\) & \num{< 0.01} & \qty{65}{\percent} \\
566. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.6\) & \num{< 0.01} & \qty{66}{\percent} \\
567. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.6\) & \num{< 0.01} & \qty{67}{\percent} \\
568. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.5\) & \num{< 0.01} & \qty{69}{\percent} \\
569. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.3\) & \num{< 0.01} & \qty{39}{\percent} \\
570. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.0\) & \num{< 0.01} & \qty{36}{\percent} \\
571. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.1\) & \num{< 0.01} & \qty{38}{\percent} \\
572. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Dataset}=\fmnist{}\) & \num{< 0.01} & \qty{41}{\percent} \\
573. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.2\) & \num{< 0.01} & \qty{40}{\percent} \\
574. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.6\) & \num{< 0.01} & \qty{67}{\percent} \\
575. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.4\) & \num{< 0.01} & \qty{69}{\percent} \\
576. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.6\) & \num{< 0.01} & \qty{65}{\percent} \\
577. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.2\) & \num{< 0.01} & \qty{38}{\percent} \\
578. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.1\) & \num{< 0.01} & \qty{39}{\percent} \\
579. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.1\) & \num{< 0.01} & \qty{29}{\percent} \\
580. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.1\) & \num{< 0.01} & \qty{38}{\percent} \\
581. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\cov{}=\textit{Disabled}\) & \num{< 0.01} & \qty{48}{\percent} \\
582. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.3\) & \num{< 0.01} & \qty{38}{\percent} \\
583. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.0\) & \num{< 0.01} & \qty{39}{\percent} \\
584. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.2\) & \num{< 0.01} & \qty{38}{\percent} \\
585. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.4\) & \num{< 0.01} & \qty{38}{\percent} \\
586. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.9\) & \num{< 0.01} & \qty{39}{\percent} \\
587. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.3\) & \num{< 0.01} & \qty{69}{\percent} \\
588. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.3\) & \num{< 0.01} & \qty{38}{\percent} \\
589. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.5\) & \num{< 0.01} & \qty{39}{\percent} \\
590. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.8\) & \num{< 0.01} & \qty{40}{\percent} \\
591. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.5\) & \num{< 0.01} & \qty{65}{\percent} \\
592. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+2.0\) & \num{< 0.01} & \qty{67}{\percent} \\
593. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.5\) & \num{< 0.01} & \qty{66}{\percent} \\
594. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.5\) & \num{< 0.01} & \qty{67}{\percent} \\
595. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.7\) & \num{< 0.01} & \qty{40}{\percent} \\
596. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.6\) & \num{< 0.01} & \qty{39}{\percent} \\
597. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.4\) & \num{< 0.01} & \qty{39}{\percent} \\
598. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.2\) & \num{< 0.01} & \qty{68}{\percent} \\
599. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.5\) & \num{< 0.01} & \qty{39}{\percent} \\
600. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.7\) & \num{< 0.01} & \qty{41}{\percent} \\
601. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.5\) & \num{< 0.01} & \qty{66}{\percent} \\
602. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.9\) & \num{< 0.01} & \qty{67}{\percent} \\
603. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.6\) & \num{< 0.01} & \qty{39}{\percent} \\
604. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.4\) & \num{< 0.01} & \qty{65}{\percent} \\
605. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.5\) & \num{< 0.01} & \qty{55}{\percent} \\
606. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.1\) & \num{< 0.01} & \qty{68}{\percent} \\
607. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.1\) & \num{< 0.01} & \qty{71}{\percent} \\
608. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.1\) & \num{< 0.01} & \qty{38}{\percent} \\
609. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.7\) & \num{< 0.01} & \qty{39}{\percent} \\
610. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.2\) & \num{< 0.01} & \qty{38}{\percent} \\
611. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.4\) & \num{< 0.01} & \qty{66}{\percent} \\
612. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.0\) & \num{< 0.01} & \qty{38}{\percent} \\
613. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.3\) & \num{< 0.01} & \qty{38}{\percent} \\
614. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.8\) & \num{< 0.01} & \qty{39}{\percent} \\
615. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.4\) & \num{< 0.01} & \qty{38}{\percent} \\
616. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.9\) & \num{< 0.01} & \qty{38}{\percent} \\
617. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.5\) & \num{< 0.01} & \qty{38}{\percent} \\
618. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.8\) & \num{< 0.01} & \qty{67}{\percent} \\
619. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.6\) & \num{< 0.01} & \qty{38}{\percent} \\
620. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.7\) & \num{< 0.01} & \qty{38}{\percent} \\
621. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.3\) & \num{< 0.01} & \qty{65}{\percent} \\
622. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.3\) & \num{< 0.01} & \qty{33}{\percent} \\
623. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.0\) & \num{< 0.01} & \qty{67}{\percent} \\
624. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.4\) & \num{< 0.01} & \qty{66}{\percent} \\
625. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.3\) & \num{< 0.01} & \qty{66}{\percent} \\
626. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.8\) & \num{< 0.01} & \qty{38}{\percent} \\
627. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.9\) & \num{< 0.01} & \qty{38}{\percent} \\
628. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+2.0\) & \num{< 0.01} & \qty{65}{\percent} \\
629. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.2\) & \num{< 0.01} & \qty{67}{\percent} \\
630. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+2.0\) & \num{< 0.01} & \qty{37}{\percent} \\
631. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.2\) & \num{< 0.01} & \qty{65}{\percent} \\
632. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.7\) & \num{< 0.01} & \qty{66}{\percent} \\
633. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.9\) & \num{< 0.01} & \qty{67}{\percent} \\
634. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.9\) & \num{< 0.01} & \qty{65}{\percent} \\
635. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+2.0\) & \num{< 0.01} & \qty{66}{\percent} \\
636. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.4\) & \num{< 0.01} & \qty{65}{\percent} \\
637. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.2\) & \num{< 0.01} & \qty{38}{\percent} \\
638. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.8\) & \num{< 0.01} & \qty{41}{\percent} \\
639. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.8\) & \num{< 0.01} & \qty{65}{\percent} \\
640. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.6\) & \num{< 0.01} & \qty{54}{\percent} \\
641. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.8\) & \num{< 0.01} & \qty{66}{\percent} \\
642. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.9\) & \num{< 0.01} & \qty{66}{\percent} \\
643. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.6\) & \num{< 0.01} & \qty{66}{\percent} \\
644. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.1\) & \num{< 0.01} & \qty{63}{\percent} \\
645. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Loss}=\cwlossfull{}\) & \num{< 0.01} & \qty{54}{\percent} \\
646. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.7\) & \num{< 0.01} & \qty{65}{\percent} \\
647. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Solver}=\adam{}\) & \num{< 0.01} & \qty{56}{\percent} \\
648. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.0\) & \num{< 0.01} & \qty{31}{\percent} \\
649. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.0\) & \num{< 0.01} & \qty{27}{\percent} \\
650. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.8\) & \num{< 0.01} & \qty{66}{\percent} \\
651. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.1\) & \num{< 0.01} & \qty{66}{\percent} \\
652. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+2.0\) & \num{< 0.01} & \qty{63}{\percent} \\
653. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.3\) & \num{< 0.01} & \qty{65}{\percent} \\
654. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.7\) & \num{< 0.01} & \qty{66}{\percent} \\
655. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Solver}=\adam{}\) & \num{< 0.01} & \qty{51}{\percent} \\
656. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.2\) & \num{< 0.01} & \qty{53}{\percent} \\
657. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.6\) & \num{< 0.01} & \qty{65}{\percent} \\
658. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.5\) & \num{< 0.01} & \qty{65}{\percent} \\
659. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.7\) & \num{< 0.01} & \qty{66}{\percent} \\
660. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.0\) & \num{< 0.01} & \qty{63}{\percent} \\
661. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.2\) & \num{< 0.01} & \qty{51}{\percent} \\
662. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.9\) & \num{< 0.01} & \qty{62}{\percent} \\
663. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.7\) & \num{< 0.01} & \qty{54}{\percent} \\
664. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.1\) & \num{< 0.01} & \qty{36}{\percent} \\
665. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.5\) & \num{< 0.01} & \qty{65}{\percent} \\
666. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.6\) & \num{< 0.01} & \qty{66}{\percent} \\
667. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.0\) & \num{< 0.01} & \qty{39}{\percent} \\
668. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.3\) & \num{< 0.01} & \qty{64}{\percent} \\
669. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.6\) & \num{< 0.01} & \qty{65}{\percent} \\
670. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.9\) & \num{< 0.01} & \qty{44}{\percent} \\
671. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.4\) & \num{< 0.01} & \qty{65}{\percent} \\
672. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.8\) & \num{< 0.01} & \qty{62}{\percent} \\
673. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.9\) & \num{< 0.01} & \qty{62}{\percent} \\
674. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.4\) & \num{< 0.01} & \qty{65}{\percent} \\
675. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.5\) & \num{< 0.01} & \qty{66}{\percent} \\
676. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.7\) & \num{< 0.01} & \qty{61}{\percent} \\
677. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.8\) & \num{< 0.01} & \qty{54}{\percent} \\
678. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.3\) & \num{< 0.01} & \qty{64}{\percent} \\
679. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.3\) & \num{< 0.01} & \qty{65}{\percent} \\
680. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.4\) & \num{< 0.01} & \qty{65}{\percent} \\
681. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Dataset}=\fmnist{}\) & \num{< 0.01} & \qty{57}{\percent} \\
682. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Saliency Map}=\jsmasmapfull{}\) & \num{< 0.01} & \qty{48}{\percent} \\
683. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.2\) & \num{< 0.01} & \qty{35}{\percent} \\
684. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.8\) & \num{< 0.01} & \qty{62}{\percent} \\
685. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.2\) & \num{< 0.01} & \qty{63}{\percent} \\
686. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.5\) & \num{< 0.01} & \qty{64}{\percent} \\
687. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.0\) & \num{< 0.01} & \qty{43}{\percent} \\
688. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.6\) & \num{< 0.01} & \qty{61}{\percent} \\
689. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.2\) & \num{< 0.01} & \qty{64}{\percent} \\
690. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.3\) & \num{< 0.01} & \qty{65}{\percent} \\
691. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.9\) & \num{< 0.01} & \qty{54}{\percent} \\
692. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.2\) & \num{< 0.01} & \qty{65}{\percent} \\
693. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.5\) & \num{< 0.01} & \qty{60}{\percent} \\
694. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.5\) & \num{< 0.01} & \qty{59}{\percent} \\
695. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.1\) & \num{< 0.01} & \qty{64}{\percent} \\
696. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.6\) & \num{< 0.01} & \qty{59}{\percent} \\
697. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.4\) & \num{< 0.01} & \qty{58}{\percent} \\
698. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.7\) & \num{< 0.01} & \qty{60}{\percent} \\
699. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.1\) & \num{< 0.01} & \qty{43}{\percent} \\
700. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.2\) & \num{< 0.01} & \qty{65}{\percent} \\
701. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.2\) & \num{< 0.01} & \qty{63}{\percent} \\
702. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.2\) & \num{< 0.01} & \qty{57}{\percent} \\
703. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.3\) & \num{< 0.01} & \qty{57}{\percent} \\
704. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.4\) & \num{< 0.01} & \qty{63}{\percent} \\
705. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.7\) & \num{< 0.01} & \qty{58}{\percent} \\
706. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.0\) & \num{< 0.01} & \qty{54}{\percent} \\
707. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.3\) & \num{< 0.01} & \qty{53}{\percent} \\
708. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.4\) & \num{< 0.01} & \qty{59}{\percent} \\
709. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.1\) & \num{< 0.01} & \qty{65}{\percent} \\
710. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.8\) & \num{< 0.01} & \qty{59}{\percent} \\
711. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.0\) & \num{< 0.01} & \qty{64}{\percent} \\
712. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.1\) & \num{< 0.01} & \qty{57}{\percent} \\
713. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.1\) & \num{< 0.01} & \qty{65}{\percent} \\
714. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.0\) & \num{< 0.01} & \qty{62}{\percent} \\
715. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.6\) & \num{< 0.01} & \qty{60}{\percent} \\
716. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.9\) & \num{< 0.01} & \qty{60}{\percent} \\
717. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.3\) & \num{< 0.01} & \qty{41}{\percent} \\
718. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.1\) & \num{< 0.01} & \qty{54}{\percent} \\
719. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.2\) & \num{< 0.01} & \qty{44}{\percent} \\
720. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\lp{}-\mathtt{target}=\lp[2]\) & \num{< 0.01} & \qty{52}{\percent} \\
721. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.9\) & \num{< 0.01} & \qty{63}{\percent} \\
722. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.0\) & \num{< 0.01} & \qty{60}{\percent} \\
723. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Dataset}=\nslkdd{}\) & \num{< 0.01} & \qty{53}{\percent} \\
724. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.3\) & \num{< 0.01} & \qty{58}{\percent} \\
725. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.3\) & \num{< 0.01} & \qty{62}{\percent} \\
726. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.0\) & \num{< 0.01} & \qty{65}{\percent} \\
727. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.0\) & \num{< 0.01} & \qty{64}{\percent} \\
728. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.1\) & \num{< 0.01} & \qty{60}{\percent} \\
729. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.2\) & \num{< 0.01} & \qty{54}{\percent} \\
730. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.5\) & \num{< 0.01} & \qty{60}{\percent} \\
731. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.3\) & \num{< 0.01} & \qty{51}{\percent} \\
732. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.0\) & \num{< 0.01} & \qty{57}{\percent} \\
733. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.1\) & \num{< 0.01} & \qty{63}{\percent} \\
734. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.2\) & \num{< 0.01} & \qty{60}{\percent} \\
735. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.8\) & \num{< 0.01} & \qty{64}{\percent} \\
736. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.3\) & \num{< 0.01} & \qty{44}{\percent} \\
737. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.2\) & \num{< 0.01} & \qty{58}{\percent} \\
738. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.3\) & \num{< 0.01} & \qty{59}{\percent} \\
739. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.3\) & \num{< 0.01} & \qty{54}{\percent} \\
740. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.0\) & \num{< 0.01} & \qty{40}{\percent} \\
741. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.9\) & \num{< 0.01} & \qty{65}{\percent} \\
742. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.9\) & \num{< 0.01} & \qty{63}{\percent} \\
743. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.4\) & \num{< 0.01} & \qty{59}{\percent} \\
744. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Loss}=\crossentropyfull{}\) & \num{< 0.01} & \qty{47}{\percent} \\
745. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.4\) & \num{< 0.01} & \qty{44}{\percent} \\
746. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.7\) & \num{< 0.01} & \qty{63}{\percent} \\
747. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.5\) & \num{< 0.01} & \qty{59}{\percent} \\
748. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.4\) & \num{< 0.01} & \qty{52}{\percent} \\
749. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.4\) & \num{< 0.01} & \qty{60}{\percent} \\
750. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.4\) & \num{< 0.01} & \qty{54}{\percent} \\
751. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.1\) & \num{< 0.01} & \qty{57}{\percent} \\
752. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\lp{}-\mathtt{target}=\lp[0]\) & \num{< 0.01} & \qty{56}{\percent} \\
753. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.6\) & \num{< 0.01} & \qty{60}{\percent} \\
754. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.2\) & \num{< 0.01} & \qty{61}{\percent} \\
755. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.7\) & \num{< 0.01} & \qty{59}{\percent} \\
756. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.5\) & \num{< 0.01} & \qty{44}{\percent} \\
757. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.5\) & \num{< 0.01} & \qty{54}{\percent} \\
758. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+2.0\) & \num{< 0.01} & \qty{55}{\percent} \\
759. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.8\) & \num{< 0.01} & \qty{59}{\percent} \\
760. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.8\) & \num{< 0.01} & \qty{62}{\percent} \\
761. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.1\) & \num{< 0.01} & \qty{57}{\percent} \\
762. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.6\) & \num{< 0.01} & \qty{64}{\percent} \\
763. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.8\) & \num{< 0.01} & \qty{64}{\percent} \\
764. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.1\) & \num{< 0.01} & \qty{40}{\percent} \\
765. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.9\) & \num{< 0.01} & \qty{59}{\percent} \\
766. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.9\) & \num{< 0.01} & \qty{55}{\percent} \\
767. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.0\) & \num{< 0.01} & \qty{55}{\percent} \\
768. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+2.0\) & \num{< 0.01} & \qty{59}{\percent} \\
769. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.6\) & \num{< 0.01} & \qty{54}{\percent} \\
770. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.8\) & \num{< 0.01} & \qty{55}{\percent} \\
771. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.6\) & \num{< 0.01} & \qty{45}{\percent} \\
772. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.4\) & \num{< 0.01} & \qty{50}{\percent} \\
773. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.7\) & \num{< 0.01} & \qty{55}{\percent} \\
774. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.3\) & \num{< 0.01} & \qty{59}{\percent} \\
775. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.7\) & \num{< 0.01} & \qty{54}{\percent} \\
776. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.6\) & \num{< 0.01} & \qty{55}{\percent} \\
777. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+2.0\) & \num{< 0.01} & \qty{58}{\percent} \\
778. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.5\) & \num{< 0.01} & \qty{64}{\percent} \\
779. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\lp{}-\mathtt{target}=\lp[2]\) & \num{< 0.01} & \qty{57}{\percent} \\
780. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.4\) & \num{< 0.01} & \qty{43}{\percent} \\
781. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.5\) & \num{< 0.01} & \qty{51}{\percent} \\
782. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.1\) & \num{< 0.01} & \qty{44}{\percent} \\
783. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.7\) & \num{< 0.01} & \qty{61}{\percent} \\
784. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.2\) & \num{< 0.01} & \qty{42}{\percent} \\
785. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.5\) & \num{< 0.01} & \qty{55}{\percent} \\
786. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.4\) & \num{< 0.01} & \qty{56}{\percent} \\
787. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.9\) & \num{< 0.01} & \qty{55}{\percent} \\
788. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.8\) & \num{< 0.01} & \qty{54}{\percent} \\
789. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.7\) & \num{< 0.01} & \qty{63}{\percent} \\
790. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.9\) & \num{< 0.01} & \qty{57}{\percent} \\
791. & \sgd{} & is better than &  \adam{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.0\) & \num{< 0.01} & \qty{44}{\percent} \\
792. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.7\) & \num{< 0.01} & \qty{46}{\percent} \\
793. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.3\) & \num{< 0.01} & \qty{56}{\percent} \\
794. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.0\) & \num{< 0.01} & \qty{46}{\percent} \\
795. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.9\) & \num{< 0.01} & \qty{53}{\percent} \\
796. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.4\) & \num{< 0.01} & \qty{63}{\percent} \\
797. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.2\) & \num{< 0.01} & \qty{55}{\percent} \\
798. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.8\) & \num{< 0.01} & \qty{57}{\percent} \\
799. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.8\) & \num{< 0.01} & \qty{46}{\percent} \\
800. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+2.0\) & \num{< 0.01} & \qty{53}{\percent} \\
801. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.1\) & \num{< 0.01} & \qty{56}{\percent} \\
802. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.1\) & \num{< 0.01} & \qty{61}{\percent} \\
803. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.6\) & \num{< 0.01} & \qty{61}{\percent} \\
804. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\lp{}-\mathtt{target}=\lp[\infty]\) & \num{< 0.01} & \qty{49}{\percent} \\
805. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.1\) & \num{< 0.01} & \qty{48}{\percent} \\
806. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.6\) & \num{< 0.01} & \qty{51}{\percent} \\
807. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.0\) & \num{< 0.01} & \qty{55}{\percent} \\
808. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.2\) & \num{< 0.01} & \qty{58}{\percent} \\
809. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.7\) & \num{< 0.01} & \qty{56}{\percent} \\
810. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.0\) & \num{< 0.01} & \qty{55}{\percent} \\
811. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.5\) & \num{< 0.01} & \qty{49}{\percent} \\
812. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.1\) & \num{< 0.01} & \qty{62}{\percent} \\
813. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.9\) & \num{< 0.01} & \qty{47}{\percent} \\
814. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.9\) & \num{< 0.01} & \qty{54}{\percent} \\
815. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.8\) & \num{< 0.01} & \qty{53}{\percent} \\
816. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.6\) & \num{< 0.01} & \qty{61}{\percent} \\
817. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.0\) & \num{0.01} & \qty{43}{\percent} \\
818. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.3\) & \num{0.01} & \qty{63}{\percent} \\
819. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.8\) & \num{0.01} & \qty{54}{\percent} \\
820. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.2\) & \num{0.01} & \qty{47}{\percent} \\
821. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.3\) & \num{0.01} & \qty{43}{\percent} \\
822. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Dataset}=\phishing{}\) & \num{0.01} & \qty{51}{\percent} \\
823. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.1\) & \num{0.01} & \qty{45}{\percent} \\
824. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.2\) & \num{0.01} & \qty{44}{\percent} \\
825. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[2]+2.0\) & \num{0.01} & \qty{47}{\percent} \\
826. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.6\) & \num{0.01} & \qty{55}{\percent} \\
827. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.4\) & \num{0.01} & \qty{43}{\percent} \\
828. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.7\) & \num{0.01} & \qty{54}{\percent} \\
829. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.5\) & \num{0.01} & \qty{43}{\percent} \\
830. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.5\) & \num{0.01} & \qty{45}{\percent} \\
831. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.6\) & \num{0.01} & \qty{43}{\percent} \\
832. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.6\) & \num{0.01} & \qty{54}{\percent} \\
833. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.7\) & \num{0.01} & \qty{51}{\percent} \\
834. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.2\) & \num{0.01} & \qty{63}{\percent} \\
835. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.3\) & \num{0.02} & \qty{47}{\percent} \\
836. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.5\) & \num{0.02} & \qty{54}{\percent} \\
837. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.7\) & \num{0.02} & \qty{42}{\percent} \\
838. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.0\) & \num{0.02} & \qty{53}{\percent} \\
839. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.5\) & \num{0.02} & \qty{60}{\percent} \\
840. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.5\) & \num{0.02} & \qty{53}{\percent} \\
841. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.2\) & \num{0.02} & \qty{63}{\percent} \\
842. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\lp{}-\mathtt{target}=\lp[0]\) & \num{0.02} & \qty{51}{\percent} \\
843. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.6\) & \num{0.02} & \qty{48}{\percent} \\
844. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.7\) & \num{0.03} & \qty{51}{\percent} \\
845. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.3\) & \num{0.03} & \qty{62}{\percent} \\
846. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Dataset}=\mnist{}\) & \num{0.03} & \qty{59}{\percent} \\
847. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.5\) & \num{0.03} & \qty{60}{\percent} \\
848. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\rr{}=\textit{Disabled}\) & \num{0.03} & \qty{49}{\percent} \\
849. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.8\) & \num{0.03} & \qty{43}{\percent} \\
850. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.4\) & \num{0.03} & \qty{52}{\percent} \\
851. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.4\) & \num{0.04} & \qty{62}{\percent} \\
852. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.4\) & \num{0.04} & \qty{53}{\percent} \\
853. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Dataset}=\unswnb{}\) & \num{0.04} & \qty{46}{\percent} \\
854. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.3\) & \num{0.04} & \qty{53}{\percent} \\
855. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.8\) & \num{0.05} & \qty{51}{\percent} \\
856. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.5\) & \num{0.05} & \qty{62}{\percent} \\
857. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.0\) & \num{0.05} & \qty{45}{\percent} \\
858. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Loss}=\crossentropyfull{}\) & \num{0.05} & \qty{49}{\percent} \\
859. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.9\) & \num{0.05} & \qty{45}{\percent} \\
860. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.4\) & \num{0.06} & \qty{48}{\percent} \\
861. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+2.0\) & \num{0.06} & \qty{41}{\percent} \\
862. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.6\) & \num{0.06} & \qty{61}{\percent} \\
863. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Loss}=\cwlossfull{}\) & \num{0.06} & \qty{48}{\percent} \\
864. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+2.0\) & \num{0.06} & \qty{57}{\percent} \\
865. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.9\) & \num{0.07} & \qty{57}{\percent} \\
866. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.7\) & \num{0.07} & \qty{47}{\percent} \\
867. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.8\) & \num{0.07} & \qty{57}{\percent} \\
868. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.7\) & \num{0.07} & \qty{61}{\percent} \\
869. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.0\) & \num{0.08} & \qty{46}{\percent} \\
870. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.7\) & \num{0.08} & \qty{57}{\percent} \\
871. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.3\) & \num{0.08} & \qty{46}{\percent} \\
872. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.2\) & \num{0.08} & \qty{53}{\percent} \\
873. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.6\) & \num{0.08} & \qty{57}{\percent} \\
874. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.3\) & \num{0.08} & \qty{52}{\percent} \\
875. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.8\) & \num{0.09} & \qty{60}{\percent} \\
876. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.5\) & \num{0.09} & \qty{58}{\percent} \\
877. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.1\) & \num{0.09} & \qty{63}{\percent} \\
878. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.1\) & \num{0.09} & \qty{45}{\percent} \\
879. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.1\) & \num{0.09} & \qty{58}{\percent} \\
880. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.4\) & \num{0.09} & \qty{58}{\percent} \\
881. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.3\) & \num{0.10} & \qty{59}{\percent} \\
882. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.9\) & \num{0.10} & \qty{60}{\percent} \\
883. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.2\) & \num{0.10} & \qty{59}{\percent} \\
884. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.6\) & \num{0.11} & \qty{47}{\percent} \\
885. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Loss}=\cwlossfull{}\) & \num{0.11} & \qty{51}{\percent} \\
886. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.9\) & \num{0.11} & \qty{41}{\percent} \\
887. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.0\) & \num{0.11} & \qty{60}{\percent} \\
888. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.2\) & \num{0.11} & \qty{45}{\percent} \\
889. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.9\) & \num{0.11} & \qty{51}{\percent} \\
890. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.1\) & \num{0.11} & \qty{60}{\percent} \\
891. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.1\) & \num{0.12} & \qty{52}{\percent} \\
892. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Loss}=\crossentropyfull{}\) & \num{0.12} & \qty{55}{\percent} \\
893. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.3\) & \num{0.13} & \qty{46}{\percent} \\
894. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.5\) & \num{0.13} & \qty{48}{\percent} \\
895. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.4\) & \num{0.13} & \qty{46}{\percent} \\
896. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.4\) & \num{0.13} & \qty{58}{\percent} \\
897. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.6\) & \num{0.14} & \qty{50}{\percent} \\
898. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.5\) & \num{0.14} & \qty{46}{\percent} \\
899. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.0\) & \num{0.14} & \qty{44}{\percent} \\
900. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.4\) & \num{0.14} & \qty{59}{\percent} \\
901. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.6\) & \num{0.15} & \qty{46}{\percent} \\
902. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.7\) & \num{0.15} & \qty{46}{\percent} \\
903. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.8\) & \num{0.16} & \qty{46}{\percent} \\
904. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.2\) & \num{0.16} & \qty{51}{\percent} \\
905. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.8\) & \num{0.16} & \qty{48}{\percent} \\
906. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.1\) & \num{0.16} & \qty{53}{\percent} \\
907. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.9\) & \num{0.17} & \qty{46}{\percent} \\
908. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+2.0\) & \num{0.17} & \qty{53}{\percent} \\
909. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+2.0\) & \num{0.17} & \qty{46}{\percent} \\
910. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.0\) & \num{0.17} & \qty{49}{\percent} \\
911. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[0]+2.0\) & \num{0.17} & \qty{44}{\percent} \\
912. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.8\) & \num{0.18} & \qty{41}{\percent} \\
913. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.6\) & \num{0.21} & \qty{49}{\percent} \\
914. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.9\) & \num{0.21} & \qty{52}{\percent} \\
915. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.0\) & \num{0.22} & \qty{51}{\percent} \\
916. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\lp{}-\mathtt{target}=\lp[2]\) & \num{0.22} & \qty{50}{\percent} \\
917. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.0\) & \num{0.23} & \qty{49}{\percent} \\
918. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.7\) & \num{0.27} & \qty{41}{\percent} \\
919. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.9\) & \num{0.28} & \qty{44}{\percent} \\
920. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.1\) & \num{0.29} & \qty{50}{\percent} \\
921. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.9\) & \num{0.30} & \qty{47}{\percent} \\
922. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.8\) & \num{0.31} & \qty{52}{\percent} \\
923. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.7\) & \num{0.31} & \qty{49}{\percent} \\
924. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.2\) & \num{0.32} & \qty{53}{\percent} \\
925. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.1\) & \num{0.34} & \qty{50}{\percent} \\
926. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.8\) & \num{0.36} & \qty{49}{\percent} \\
927. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.0\) & \num{0.37} & \qty{55}{\percent} \\
928. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.7\) & \num{0.40} & \qty{48}{\percent} \\
929. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\cov{}=\textit{Disabled}\) & \num{0.40} & \qty{55}{\percent} \\
930. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.0\) & \num{0.40} & \qty{50}{\percent} \\
931. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.6\) & \num{0.40} & \qty{42}{\percent} \\
932. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.7\) & \num{0.41} & \qty{52}{\percent} \\
933. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.8\) & \num{0.42} & \qty{45}{\percent} \\
934. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.9\) & \num{0.44} & \qty{49}{\percent} \\
935. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.0\) & \num{0.47} & \qty{50}{\percent} \\
936. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.6\) & \num{0.47} & \qty{52}{\percent} \\
937. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.2\) & \num{0.48} & \qty{49}{\percent} \\
938. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.5\) & \num{0.49} & \qty{50}{\percent} \\
939. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.0\) & \num{0.50} & \qty{39}{\percent} \\
940. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.3\) & \num{0.51} & \qty{55}{\percent} \\
941. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.0\) & \num{0.52} & \qty{46}{\percent} \\
942. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.5\) & \num{0.54} & \qty{43}{\percent} \\
943. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.5\) & \num{0.56} & \qty{51}{\percent} \\
944. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.7\) & \num{0.59} & \qty{46}{\percent} \\
945. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.3\) & \num{0.64} & \qty{48}{\percent} \\
946. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.4\) & \num{0.66} & \qty{48}{\percent} \\
947. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.4\) & \num{0.68} & \qty{51}{\percent} \\
948. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.3\) & \num{0.68} & \qty{57}{\percent} \\
949. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.4\) & \num{0.69} & \qty{43}{\percent} \\
950. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.0\) & \num{0.71} & \qty{50}{\percent} \\
951. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.1\) & \num{0.73} & \qty{46}{\percent} \\
952. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.9\) & \num{0.77} & \qty{50}{\percent} \\
953. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.6\) & \num{0.77} & \qty{46}{\percent} \\
954. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.2\) & \num{0.79} & \qty{54}{\percent} \\
955. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.3\) & \num{0.80} & \qty{50}{\percent} \\
956. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.8\) & \num{0.82} & \qty{49}{\percent} \\
957. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.4\) & \num{0.83} & \qty{48}{\percent} \\
958. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.0\) & \num{0.84} & \qty{37}{\percent} \\
959. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.3\) & \num{0.85} & \qty{45}{\percent} \\
960. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.2\) & \num{0.91} & \qty{51}{\percent} \\
961. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.1\) & \num{0.94} & \qty{50}{\percent} \\
962. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.2\) & \num{0.96} & \qty{45}{\percent} \\
963. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.5\) & \num{0.97} & \qty{47}{\percent} \\


==> figures/hypotheses_robust.tex <==
1. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Dataset}=\unswnb{}\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{41}{\percent} & False \\
2. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Dataset}=\unswnb{}\) & \num{< 1e-5} & \qty{72}{\percent} & \qty{41}{\percent} & True \\
3. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Dataset}=\mnist{}\) & \num{< 2.2e-308} & \qty{89}{\percent} & \qty{40}{\percent} & False \\
4. & \jsmasmapfull{} & is better than &  \identitysmapfull{} & when & \(\mathtt{Dataset}=\mnist{}\) & \num{< 1e-5} & \qty{51}{\percent} & \qty{40}{\percent} & True \\
5. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Dataset}=\nslkdd{}\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{33}{\percent} & False \\
6. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Dataset}=\nslkdd{}\) & \num{< 1e-5} & \qty{68}{\percent} & \qty{33}{\percent} & True \\
7. & \dfsmapfull{} & is better than &  \identitysmapfull{} & when & \(\mathtt{Loss}=\crossentropyfull{}\) & \num{5.1e-02} & \qty{50}{\percent} & \qty{31}{\percent} & False \\
8. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Loss}=\crossentropyfull{}\) & \num{< 2.2e-308} & \qty{81}{\percent} & \qty{31}{\percent} & True \\
9. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Dataset}=\nslkdd{}\) & \num{< 2.2e-308} & \qty{81}{\percent} & \qty{30}{\percent} & False \\
10. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Dataset}=\nslkdd{}\) & \num{< 1e-5} & \qty{49}{\percent} & \qty{30}{\percent} & True \\
11. & \jsmasmapfull{} & is better than &  \identitysmapfull{} & when & \(\mathtt{Dataset}=\nslkdd{}\) & \num{< 1e-5} & \qty{54}{\percent} & \qty{30}{\percent} & False \\
12. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Dataset}=\nslkdd{}\) & \num{< 2.2e-308} & \qty{76}{\percent} & \qty{30}{\percent} & True \\
13. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Dataset}=\unswnb{}\) & \num{4.3e-02} & \qty{46}{\percent} & \qty{30}{\percent} & False \\
14. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Dataset}=\unswnb{}\) & \num{< 2.2e-308} & \qty{77}{\percent} & \qty{30}{\percent} & True \\
15. & \dfsmapfull{} & is better than &  \identitysmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.0\) & \num{< 1e-5} & \qty{73}{\percent} & \qty{29}{\percent} & False \\
16. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.0\) & \num{4.6e-01} & \qty{55}{\percent} & \qty{29}{\percent} & True \\
17. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Dataset}=\nslkdd{}\) & \num{< 1e-5} & \qty{53}{\percent} & \qty{28}{\percent} & False \\
18. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Dataset}=\nslkdd{}\) & \num{< 1e-5} & \qty{75}{\percent} & \qty{28}{\percent} & True \\
19. & \dfsmapfull{} & is better than &  \identitysmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.1\) & \num{< 1e-5} & \qty{66}{\percent} & \qty{28}{\percent} & False \\
20. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.1\) & \num{5.3e-02} & \qty{62}{\percent} & \qty{28}{\percent} & True \\
21. & \dfsmapfull{} & is better than &  \identitysmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.2\) & \num{< 1e-5} & \qty{61}{\percent} & \qty{27}{\percent} & False \\
22. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.2\) & \num{1.4e-02} & \qty{65}{\percent} & \qty{27}{\percent} & True \\
23. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Saliency Map}=\identitysmapfull{}\) & \num{< 1e-5} & \qty{57}{\percent} & \qty{27}{\percent} & False \\
24. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Saliency Map}=\identitysmapfull{}\) & \num{< 2.2e-308} & \qty{84}{\percent} & \qty{27}{\percent} & True \\
25. & \dfsmapfull{} & is better than &  \identitysmapfull{} & when & \(\mathtt{Dataset}=\fmnist{}\) & \num{< 1e-5} & \qty{71}{\percent} & \qty{27}{\percent} & False \\
26. & \dfsmapfull{} & is better than &  \identitysmapfull{} & when & \(\mathtt{Dataset}=\fmnist{}\) & \num{< 1e-5} & \qty{44}{\percent} & \qty{27}{\percent} & True \\
27. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.0\) & \num{< 1e-5} & \qty{64}{\percent} & \qty{25}{\percent} & False \\
28. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.0\) & \num{2.2e-02} & \qty{61}{\percent} & \qty{25}{\percent} & True \\
29. & \dfsmapfull{} & is better than &  \identitysmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.3\) & \num{< 1e-5} & \qty{58}{\percent} & \qty{24}{\percent} & False \\
30. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.3\) & \num{6.7e-03} & \qty{66}{\percent} & \qty{24}{\percent} & True \\
31. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Dataset}=\nslkdd{}\) & \num{< 2.2e-308} & \qty{89}{\percent} & \qty{24}{\percent} & False \\
32. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Dataset}=\nslkdd{}\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{24}{\percent} & True \\
33. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.5\) & \num{< 1e-5} & \qty{60}{\percent} & \qty{24}{\percent} & False \\
34. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.5\) & \num{2.6e-03} & \qty{64}{\percent} & \qty{24}{\percent} & True \\
35. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.7\) & \num{< 1e-5} & \qty{58}{\percent} & \qty{23}{\percent} & False \\
36. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.7\) & \num{1.5e-03} & \qty{65}{\percent} & \qty{23}{\percent} & True \\
37. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.6\) & \num{< 1e-5} & \qty{58}{\percent} & \qty{23}{\percent} & False \\
38. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.6\) & \num{1.6e-03} & \qty{64}{\percent} & \qty{23}{\percent} & True \\
39. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.8\) & \num{< 1e-5} & \qty{58}{\percent} & \qty{23}{\percent} & False \\
40. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.8\) & \num{1.5e-03} & \qty{65}{\percent} & \qty{23}{\percent} & True \\
41. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Loss}=\crossentropyfull{}\) & \num{1.2e-01} & \qty{55}{\percent} & \qty{23}{\percent} & False \\
42. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Loss}=\crossentropyfull{}\) & \num{< 2.2e-308} & \qty{78}{\percent} & \qty{23}{\percent} & True \\
43. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.4\) & \num{< 1e-5} & \qty{60}{\percent} & \qty{23}{\percent} & False \\
44. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.4\) & \num{6.4e-03} & \qty{62}{\percent} & \qty{23}{\percent} & True \\
45. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Loss}=\cwlossfull{}\) & \num{1.1e-01} & \qty{51}{\percent} & \qty{23}{\percent} & False \\
46. & \jsmasmapfull{} & is better than &  \identitysmapfull{} & when & \(\mathtt{Loss}=\cwlossfull{}\) & \num{< 2.2e-308} & \qty{71}{\percent} & \qty{23}{\percent} & True \\
47. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Dataset}=\unswnb{}\) & \num{< 2.2e-308} & \qty{73}{\percent} & \qty{22}{\percent} & False \\
48. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Dataset}=\unswnb{}\) & \num{< 1e-5} & \qty{50}{\percent} & \qty{22}{\percent} & True \\
49. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.1\) & \num{< 1e-5} & \qty{63}{\percent} & \qty{22}{\percent} & False \\
50. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.1\) & \num{2.9e-02} & \qty{58}{\percent} & \qty{22}{\percent} & True \\
51. & \dfsmapfull{} & is better than &  \identitysmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.4\) & \num{4.1e-04} & \qty{56}{\percent} & \qty{22}{\percent} & False \\
52. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.4\) & \num{4.0e-03} & \qty{66}{\percent} & \qty{22}{\percent} & True \\
53. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.7\) & \num{5.9e-01} & \qty{53}{\percent} & \qty{22}{\percent} & False \\
54. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.7\) & \num{< 1e-5} & \qty{76}{\percent} & \qty{22}{\percent} & True \\
55. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.6\) & \num{7.7e-01} & \qty{53}{\percent} & \qty{22}{\percent} & False \\
56. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.6\) & \num{< 1e-5} & \qty{75}{\percent} & \qty{22}{\percent} & True \\
57. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.8\) & \num{4.2e-01} & \qty{54}{\percent} & \qty{22}{\percent} & False \\
58. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.8\) & \num{< 1e-5} & \qty{76}{\percent} & \qty{22}{\percent} & True \\
59. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.2\) & \num{< 1e-5} & \qty{62}{\percent} & \qty{22}{\percent} & False \\
60. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.2\) & \num{2.6e-02} & \qty{59}{\percent} & \qty{22}{\percent} & True \\
61. & \dfsmapfull{} & is better than &  \identitysmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.0\) & \num{< 1e-5} & \qty{71}{\percent} & \qty{21}{\percent} & False \\
62. & \dfsmapfull{} & is better than &  \identitysmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.0\) & \num{3.9e-01} & \qty{49}{\percent} & \qty{21}{\percent} & True \\
63. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.3\) & \num{< 1e-5} & \qty{61}{\percent} & \qty{21}{\percent} & False \\
64. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.3\) & \num{1.5e-02} & \qty{60}{\percent} & \qty{21}{\percent} & True \\
65. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Dataset}=\fmnist{}\) & \num{< 1e-5} & \qty{51}{\percent} & \qty{21}{\percent} & False \\
66. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Dataset}=\fmnist{}\) & \num{< 1e-5} & \qty{70}{\percent} & \qty{21}{\percent} & True \\
67. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.9\) & \num{2.8e-01} & \qty{55}{\percent} & \qty{21}{\percent} & False \\
68. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.9\) & \num{< 1e-5} & \qty{76}{\percent} & \qty{21}{\percent} & True \\
69. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.1\) & \num{< 1e-5} & \qty{56}{\percent} & \qty{21}{\percent} & False \\
70. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.1\) & \num{1.9e-03} & \qty{65}{\percent} & \qty{21}{\percent} & True \\
71. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.0\) & \num{< 1e-5} & \qty{56}{\percent} & \qty{21}{\percent} & False \\
72. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.0\) & \num{1.7e-03} & \qty{65}{\percent} & \qty{21}{\percent} & True \\
73. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.2\) & \num{< 1e-5} & \qty{55}{\percent} & \qty{21}{\percent} & False \\
74. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.2\) & \num{2.0e-03} & \qty{65}{\percent} & \qty{21}{\percent} & True \\
75. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[0]+2.0\) & \num{1.7e-01} & \qty{55}{\percent} & \qty{21}{\percent} & False \\
76. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[0]+2.0\) & \num{< 1e-5} & \qty{76}{\percent} & \qty{21}{\percent} & True \\
77. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[0]+2.0\) & \num{5.6e-02} & \qty{58}{\percent} & \qty{21}{\percent} & False \\
78. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[0]+2.0\) & \num{< 1e-5} & \qty{80}{\percent} & \qty{21}{\percent} & True \\
79. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.6\) & \num{4.0e-01} & \qty{57}{\percent} & \qty{21}{\percent} & False \\
80. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.6\) & \num{< 1e-5} & \qty{78}{\percent} & \qty{21}{\percent} & True \\
81. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.9\) & \num{< 1e-5} & \qty{55}{\percent} & \qty{21}{\percent} & False \\
82. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.9\) & \num{1.5e-03} & \qty{65}{\percent} & \qty{21}{\percent} & True \\
83. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.0\) & \num{2.2e-01} & \qty{51}{\percent} & \qty{21}{\percent} & False \\
84. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.0\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{21}{\percent} & True \\
85. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.7\) & \num{2.7e-01} & \qty{58}{\percent} & \qty{21}{\percent} & False \\
86. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.7\) & \num{< 1e-5} & \qty{79}{\percent} & \qty{21}{\percent} & True \\
87. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.8\) & \num{1.8e-01} & \qty{58}{\percent} & \qty{21}{\percent} & False \\
88. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.8\) & \num{< 1e-5} & \qty{79}{\percent} & \qty{21}{\percent} & True \\
89. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.9\) & \num{1.1e-01} & \qty{58}{\percent} & \qty{21}{\percent} & False \\
90. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.9\) & \num{< 1e-5} & \qty{79}{\percent} & \qty{21}{\percent} & True \\
91. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Dataset}=\unswnb{}\) & \num{< 1e-5} & \qty{61}{\percent} & \qty{20}{\percent} & False \\
92. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Dataset}=\unswnb{}\) & \num{< 1e-5} & \qty{59}{\percent} & \qty{20}{\percent} & True \\
93. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.1\) & \num{3.4e-01} & \qty{50}{\percent} & \qty{20}{\percent} & False \\
94. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.1\) & \num{< 1e-5} & \qty{70}{\percent} & \qty{20}{\percent} & True \\
95. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.5\) & \num{9.7e-01} & \qty{52}{\percent} & \qty{20}{\percent} & False \\
96. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.5\) & \num{< 1e-5} & \qty{73}{\percent} & \qty{20}{\percent} & True \\
97. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.3\) & \num{< 1e-5} & \qty{55}{\percent} & \qty{20}{\percent} & False \\
98. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.3\) & \num{2.2e-03} & \qty{65}{\percent} & \qty{20}{\percent} & True \\
99. & \dfsmapfull{} & is better than &  \identitysmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.5\) & \num{1.3e-02} & \qty{54}{\percent} & \qty{20}{\percent} & False \\
100. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.5\) & \num{2.4e-03} & \qty{66}{\percent} & \qty{20}{\percent} & True \\
101. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.9\) & \num{1.1e-01} & \qty{51}{\percent} & \qty{20}{\percent} & False \\
102. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.9\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{20}{\percent} & True \\
103. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.3\) & \num{6.4e-01} & \qty{48}{\percent} & \qty{20}{\percent} & False \\
104. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.3\) & \num{< 1e-5} & \qty{71}{\percent} & \qty{20}{\percent} & True \\
105. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.4\) & \num{8.3e-01} & \qty{48}{\percent} & \qty{20}{\percent} & False \\
106. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.4\) & \num{< 1e-5} & \qty{72}{\percent} & \qty{20}{\percent} & True \\
107. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.4\) & \num{2.8e-05} & \qty{55}{\percent} & \qty{20}{\percent} & False \\
108. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.4\) & \num{2.5e-03} & \qty{65}{\percent} & \qty{20}{\percent} & True \\
109. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.5\) & \num{5.4e-01} & \qty{56}{\percent} & \qty{20}{\percent} & False \\
110. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.5\) & \num{< 1e-5} & \qty{76}{\percent} & \qty{20}{\percent} & True \\
111. & \dfsmapfull{} & is better than &  \identitysmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.1\) & \num{< 1e-5} & \qty{63}{\percent} & \qty{20}{\percent} & False \\
112. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.1\) & \num{4.4e-01} & \qty{56}{\percent} & \qty{20}{\percent} & True \\
113. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.5\) & \num{7.8e-05} & \qty{55}{\percent} & \qty{20}{\percent} & False \\
114. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.5\) & \num{2.7e-03} & \qty{65}{\percent} & \qty{20}{\percent} & True \\
115. & \dfsmapfull{} & is better than &  \identitysmapfull{} & when & \(\lp{}-\mathtt{target}=\lp[\infty]\) & \num{2.9e-03} & \qty{50}{\percent} & \qty{20}{\percent} & False \\
116. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\lp{}-\mathtt{target}=\lp[\infty]\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{20}{\percent} & True \\
117. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.2\) & \num{4.8e-01} & \qty{49}{\percent} & \qty{20}{\percent} & False \\
118. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.2\) & \num{< 1e-5} & \qty{70}{\percent} & \qty{20}{\percent} & True \\
119. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.6\) & \num{2.6e-04} & \qty{55}{\percent} & \qty{19}{\percent} & False \\
120. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.6\) & \num{3.1e-03} & \qty{64}{\percent} & \qty{19}{\percent} & True \\
121. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.8\) & \num{4.5e-02} & \qty{51}{\percent} & \qty{19}{\percent} & False \\
122. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.8\) & \num{< 1e-5} & \qty{67}{\percent} & \qty{19}{\percent} & True \\
123. & \dfsmapfull{} & is better than &  \identitysmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.6\) & \num{1.1e-01} & \qty{52}{\percent} & \qty{19}{\percent} & False \\
124. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.6\) & \num{1.5e-03} & \qty{66}{\percent} & \qty{19}{\percent} & True \\
125. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.0\) & \num{< 1e-5} & \qty{93}{\percent} & \qty{19}{\percent} & False \\
126. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.0\) & \num{< 1e-5} & \qty{74}{\percent} & \qty{19}{\percent} & True \\
127. & \dfsmapfull{} & is better than &  \identitysmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.7\) & \num{4.0e-01} & \qty{51}{\percent} & \qty{18}{\percent} & False \\
128. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.7\) & \num{1.1e-03} & \qty{67}{\percent} & \qty{18}{\percent} & True \\
129. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.9\) & \num{< 1e-5} & \qty{71}{\percent} & \qty{18}{\percent} & False \\
130. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.9\) & \num{5.9e-01} & \qty{47}{\percent} & \qty{18}{\percent} & True \\
131. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Solver}=\sgd{}\) & \num{< 2.2e-308} & \qty{71}{\percent} & \qty{18}{\percent} & False \\
132. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Solver}=\sgd{}\) & \num{< 1e-5} & \qty{53}{\percent} & \qty{18}{\percent} & True \\
133. & \jsmasmapfull{} & is better than &  \identitysmapfull{} & when & \(\mathtt{Dataset}=\fmnist{}\) & \num{< 1e-5} & \qty{58}{\percent} & \qty{18}{\percent} & False \\
134. & \jsmasmapfull{} & is better than &  \identitysmapfull{} & when & \(\mathtt{Dataset}=\fmnist{}\) & \num{< 1e-5} & \qty{40}{\percent} & \qty{18}{\percent} & True \\
135. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Dataset}=\mnist{}\) & \num{< 2.2e-308} & \qty{74}{\percent} & \qty{18}{\percent} & False \\
136. & \dfsmapfull{} & is better than &  \identitysmapfull{} & when & \(\mathtt{Dataset}=\mnist{}\) & \num{< 1e-5} & \qty{44}{\percent} & \qty{18}{\percent} & True \\
137. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.6\) & \num{3.2e-03} & \qty{51}{\percent} & \qty{18}{\percent} & False \\
138. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.6\) & \num{< 1e-5} & \qty{66}{\percent} & \qty{18}{\percent} & True \\
139. & \dfsmapfull{} & is better than &  \identitysmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.2\) & \num{4.7e-04} & \qty{57}{\percent} & \qty{18}{\percent} & False \\
140. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.2\) & \num{5.4e-02} & \qty{60}{\percent} & \qty{18}{\percent} & True \\
141. & \dfsmapfull{} & is better than &  \identitysmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.8\) & \num{8.2e-01} & \qty{50}{\percent} & \qty{18}{\percent} & False \\
142. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.8\) & \num{8.2e-04} & \qty{67}{\percent} & \qty{18}{\percent} & True \\
143. & \lp[0] & is better than &  \lp[2] & when & \(\cov{}=\textit{Disabled}\) & \num{< 1e-5} & \qty{57}{\percent} & \qty{17}{\percent} & False \\
144. & \lp[2] & is better than &  \lp[0] & when & \(\cov{}=\textit{Disabled}\) & \num{< 1e-5} & \qty{60}{\percent} & \qty{17}{\percent} & True \\
145. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.7\) & \num{1.4e-02} & \qty{51}{\percent} & \qty{17}{\percent} & False \\
146. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.7\) & \num{< 1e-5} & \qty{66}{\percent} & \qty{17}{\percent} & True \\
147. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.0\) & \num{< 1e-5} & \qty{71}{\percent} & \qty{17}{\percent} & False \\
148. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.0\) & \num{6.2e-01} & \qty{46}{\percent} & \qty{17}{\percent} & True \\
149. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.0\) & \num{5.2e-01} & \qty{46}{\percent} & \qty{17}{\percent} & False \\
150. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.0\) & \num{< 1e-5} & \qty{70}{\percent} & \qty{17}{\percent} & True \\
151. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.1\) & \num{< 1e-5} & \qty{70}{\percent} & \qty{17}{\percent} & False \\
152. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.1\) & \num{6.1e-01} & \qty{46}{\percent} & \qty{17}{\percent} & True \\
153. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.1\) & \num{7.3e-01} & \qty{46}{\percent} & \qty{17}{\percent} & False \\
154. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.1\) & \num{< 1e-5} & \qty{71}{\percent} & \qty{17}{\percent} & True \\
155. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.7\) & \num{8.9e-04} & \qty{53}{\percent} & \qty{17}{\percent} & False \\
156. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.7\) & \num{3.5e-03} & \qty{63}{\percent} & \qty{17}{\percent} & True \\
157. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.3\) & \num{< 1e-5} & \qty{53}{\percent} & \qty{17}{\percent} & False \\
158. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.3\) & \num{3.5e-01} & \qty{63}{\percent} & \qty{17}{\percent} & True \\
159. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.4\) & \num{3.2e-05} & \qty{52}{\percent} & \qty{17}{\percent} & False \\
160. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.4\) & \num{3.4e-02} & \qty{65}{\percent} & \qty{17}{\percent} & True \\
161. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.5\) & \num{4.5e-04} & \qty{51}{\percent} & \qty{17}{\percent} & False \\
162. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.5\) & \num{8.7e-04} & \qty{65}{\percent} & \qty{17}{\percent} & True \\
163. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.9\) & \num{3.0e-01} & \qty{47}{\percent} & \qty{17}{\percent} & False \\
164. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.9\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{17}{\percent} & True \\
165. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.2\) & \num{9.6e-01} & \qty{45}{\percent} & \qty{17}{\percent} & False \\
166. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.2\) & \num{< 1e-5} & \qty{71}{\percent} & \qty{17}{\percent} & True \\
167. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.3\) & \num{8.5e-01} & \qty{55}{\percent} & \qty{17}{\percent} & False \\
168. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.3\) & \num{< 1e-5} & \qty{72}{\percent} & \qty{17}{\percent} & True \\
169. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.4\) & \num{6.9e-01} & \qty{56}{\percent} & \qty{17}{\percent} & False \\
170. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.4\) & \num{< 1e-5} & \qty{73}{\percent} & \qty{17}{\percent} & True \\
171. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.9\) & \num{< 1e-5} & \qty{70}{\percent} & \qty{16}{\percent} & False \\
172. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.9\) & \num{6.2e-01} & \qty{46}{\percent} & \qty{16}{\percent} & True \\
173. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.9\) & \num{7.7e-01} & \qty{50}{\percent} & \qty{16}{\percent} & False \\
174. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.9\) & \num{8.7e-04} & \qty{67}{\percent} & \qty{16}{\percent} & True \\
175. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.8\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{16}{\percent} & False \\
176. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.8\) & \num{5.8e-01} & \qty{47}{\percent} & \qty{16}{\percent} & True \\
177. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Loss}=\crossentropyfull{}\) & \num{< 2.2e-308} & \qty{65}{\percent} & \qty{16}{\percent} & False \\
178. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Loss}=\crossentropyfull{}\) & \num{< 1e-5} & \qty{48}{\percent} & \qty{16}{\percent} & True \\
179. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Loss}=\cwlossfull{}\) & \num{6.1e-02} & \qty{48}{\percent} & \qty{16}{\percent} & False \\
180. & \dfsmapfull{} & is better than &  \identitysmapfull{} & when & \(\mathtt{Loss}=\cwlossfull{}\) & \num{< 2.2e-308} & \qty{68}{\percent} & \qty{16}{\percent} & True \\
181. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.4\) & \num{2.6e-04} & \qty{50}{\percent} & \qty{16}{\percent} & False \\
182. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.4\) & \num{1.4e-02} & \qty{66}{\percent} & \qty{16}{\percent} & True \\
183. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.7\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{16}{\percent} & False \\
184. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.7\) & \num{5.9e-01} & \qty{47}{\percent} & \qty{16}{\percent} & True \\
185. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.8\) & \num{1.6e-01} & \qty{48}{\percent} & \qty{16}{\percent} & False \\
186. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.8\) & \num{< 1e-5} & \qty{68}{\percent} & \qty{16}{\percent} & True \\
187. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.8\) & \num{< 1e-5} & \qty{70}{\percent} & \qty{16}{\percent} & False \\
188. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.8\) & \num{6.2e-01} & \qty{46}{\percent} & \qty{16}{\percent} & True \\
189. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+2.0\) & \num{< 1e-5} & \qty{70}{\percent} & \qty{16}{\percent} & False \\
190. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+2.0\) & \num{6.3e-01} & \qty{46}{\percent} & \qty{16}{\percent} & True \\
191. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.0\) & \num{4.7e-01} & \qty{50}{\percent} & \qty{16}{\percent} & False \\
192. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.0\) & \num{9.5e-04} & \qty{66}{\percent} & \qty{16}{\percent} & True \\
193. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Saliency Map}=\dfsmapfull{}\) & \num{< 2.2e-308} & \qty{68}{\percent} & \qty{16}{\percent} & False \\
194. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Saliency Map}=\dfsmapfull{}\) & \num{< 1e-5} & \qty{51}{\percent} & \qty{16}{\percent} & True \\
195. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.3\) & \num{< 1e-5} & \qty{51}{\percent} & \qty{16}{\percent} & False \\
196. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.3\) & \num{1.7e-01} & \qty{65}{\percent} & \qty{16}{\percent} & True \\
197. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.6\) & \num{2.3e-02} & \qty{48}{\percent} & \qty{16}{\percent} & False \\
198. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.6\) & \num{< 1e-5} & \qty{67}{\percent} & \qty{16}{\percent} & True \\
199. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.2\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{16}{\percent} & False \\
200. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.2\) & \num{6.1e-01} & \qty{46}{\percent} & \qty{16}{\percent} & True \\
201. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.7\) & \num{< 1e-5} & \qty{70}{\percent} & \qty{16}{\percent} & False \\
202. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.7\) & \num{6.2e-01} & \qty{46}{\percent} & \qty{16}{\percent} & True \\
203. & \dfsmapfull{} & is better than &  \identitysmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.3\) & \num{7.7e-02} & \qty{53}{\percent} & \qty{16}{\percent} & False \\
204. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.3\) & \num{8.3e-03} & \qty{62}{\percent} & \qty{16}{\percent} & True \\
205. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Dataset}=\mnist{}\) & \num{< 1e-5} & \qty{73}{\percent} & \qty{16}{\percent} & False \\
206. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Dataset}=\mnist{}\) & \num{< 1e-5} & \qty{57}{\percent} & \qty{16}{\percent} & True \\
207. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\cov{}=\textit{Enabled}\) & \num{< 2.2e-308} & \qty{93}{\percent} & \qty{16}{\percent} & False \\
208. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\cov{}=\textit{Enabled}\) & \num{< 2.2e-308} & \qty{76}{\percent} & \qty{16}{\percent} & True \\
209. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.5\) & \num{3.8e-03} & \qty{49}{\percent} & \qty{16}{\percent} & False \\
210. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.5\) & \num{2.4e-04} & \qty{66}{\percent} & \qty{16}{\percent} & True \\
211. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.5\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{16}{\percent} & False \\
212. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.5\) & \num{6.2e-01} & \qty{46}{\percent} & \qty{16}{\percent} & True \\
213. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.6\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{16}{\percent} & False \\
214. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.6\) & \num{6.3e-01} & \qty{46}{\percent} & \qty{16}{\percent} & True \\
215. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Saliency Map}=\identitysmapfull{}\) & \num{< 1e-5} & \qty{53}{\percent} & \qty{15}{\percent} & False \\
216. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Saliency Map}=\identitysmapfull{}\) & \num{< 1e-5} & \qty{62}{\percent} & \qty{15}{\percent} & True \\
217. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.7\) & \num{7.1e-02} & \qty{47}{\percent} & \qty{15}{\percent} & False \\
218. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.7\) & \num{< 1e-5} & \qty{68}{\percent} & \qty{15}{\percent} & True \\
219. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.3\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{15}{\percent} & False \\
220. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.3\) & \num{6.2e-01} & \qty{46}{\percent} & \qty{15}{\percent} & True \\
221. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.4\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{15}{\percent} & False \\
222. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.4\) & \num{6.2e-01} & \qty{46}{\percent} & \qty{15}{\percent} & True \\
223. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.0\) & \num{< 1e-5} & \qty{68}{\percent} & \qty{15}{\percent} & False \\
224. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.0\) & \num{6.9e-01} & \qty{53}{\percent} & \qty{15}{\percent} & True \\
225. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.1\) & \num{2.9e-01} & \qty{50}{\percent} & \qty{15}{\percent} & False \\
226. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.1\) & \num{1.1e-03} & \qty{66}{\percent} & \qty{15}{\percent} & True \\
227. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Solver}=\sgd{}\) & \num{< 1e-5} & \qty{56}{\percent} & \qty{15}{\percent} & False \\
228. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Solver}=\sgd{}\) & \num{< 2.2e-308} & \qty{71}{\percent} & \qty{15}{\percent} & True \\
229. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.1\) & \num{< 1e-5} & \qty{53}{\percent} & \qty{15}{\percent} & False \\
230. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.1\) & \num{3.3e-01} & \qty{37}{\percent} & \qty{15}{\percent} & True \\
231. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.2\) & \num{< 1e-5} & \qty{53}{\percent} & \qty{15}{\percent} & False \\
232. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.2\) & \num{8.0e-01} & \qty{37}{\percent} & \qty{15}{\percent} & True \\
233. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.2\) & \num{< 1e-5} & \qty{51}{\percent} & \qty{15}{\percent} & False \\
234. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.2\) & \num{7.0e-01} & \qty{64}{\percent} & \qty{15}{\percent} & True \\
235. & \dfsmapfull{} & is better than &  \identitysmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.4\) & \num{6.6e-01} & \qty{51}{\percent} & \qty{15}{\percent} & False \\
236. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.4\) & \num{2.3e-03} & \qty{63}{\percent} & \qty{15}{\percent} & True \\
237. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.2\) & \num{1.6e-01} & \qty{51}{\percent} & \qty{15}{\percent} & False \\
238. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.2\) & \num{1.1e-03} & \qty{66}{\percent} & \qty{15}{\percent} & True \\
239. & \dfsmapfull{} & is better than &  \identitysmapfull{} & when & \(\cov{}=\textit{Disabled}\) & \num{< 1e-5} & \qty{56}{\percent} & \qty{15}{\percent} & False \\
240. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\cov{}=\textit{Disabled}\) & \num{5.8e-01} & \qty{59}{\percent} & \qty{15}{\percent} & True \\
241. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\lp{}-\mathtt{target}=\lp[0]\) & \num{2.3e-02} & \qty{48}{\percent} & \qty{15}{\percent} & False \\
242. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\lp{}-\mathtt{target}=\lp[0]\) & \num{< 1e-5} & \qty{66}{\percent} & \qty{15}{\percent} & True \\
243. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.5\) & \num{< 1e-5} & \qty{67}{\percent} & \qty{15}{\percent} & False \\
244. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.5\) & \num{6.6e-01} & \qty{47}{\percent} & \qty{15}{\percent} & True \\
245. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Dataset}=\phishing{}\) & \num{< 1e-5} & \qty{59}{\percent} & \qty{15}{\percent} & False \\
246. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Dataset}=\phishing{}\) & \num{< 2.2e-308} & \qty{74}{\percent} & \qty{15}{\percent} & True \\
247. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Dataset}=\fmnist{}\) & \num{< 1e-5} & \qty{73}{\percent} & \qty{15}{\percent} & False \\
248. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Dataset}=\fmnist{}\) & \num{< 2.2e-308} & \qty{88}{\percent} & \qty{15}{\percent} & True \\
249. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.6\) & \num{< 1e-5} & \qty{67}{\percent} & \qty{15}{\percent} & False \\
250. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.6\) & \num{5.9e-01} & \qty{47}{\percent} & \qty{15}{\percent} & True \\
251. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.8\) & \num{2.0e-03} & \qty{53}{\percent} & \qty{15}{\percent} & False \\
252. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.8\) & \num{3.9e-03} & \qty{61}{\percent} & \qty{15}{\percent} & True \\
253. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Dataset}=\mnist{}\) & \num{< 2.2e-308} & \qty{79}{\percent} & \qty{14}{\percent} & False \\
254. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Dataset}=\mnist{}\) & \num{< 2.2e-308} & \qty{94}{\percent} & \qty{14}{\percent} & True \\
255. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Saliency Map}=\identitysmapfull{}\) & \num{< 1e-5} & \qty{62}{\percent} & \qty{14}{\percent} & False \\
256. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Saliency Map}=\identitysmapfull{}\) & \num{< 2.2e-308} & \qty{77}{\percent} & \qty{14}{\percent} & True \\
257. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\lp{}-\mathtt{target}=\lp[0]\) & \num{4.1e-05} & \qty{56}{\percent} & \qty{14}{\percent} & False \\
258. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\lp{}-\mathtt{target}=\lp[0]\) & \num{< 1e-5} & \qty{58}{\percent} & \qty{14}{\percent} & True \\
259. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.2\) & \num{< 1e-5} & \qty{67}{\percent} & \qty{14}{\percent} & False \\
260. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.2\) & \num{9.2e-01} & \qty{53}{\percent} & \qty{14}{\percent} & True \\
261. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.9\) & \num{4.0e-03} & \qty{52}{\percent} & \qty{14}{\percent} & False \\
262. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.9\) & \num{4.2e-03} & \qty{61}{\percent} & \qty{14}{\percent} & True \\
263. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[2]+2.0\) & \num{7.9e-03} & \qty{52}{\percent} & \qty{14}{\percent} & False \\
264. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[2]+2.0\) & \num{4.7e-03} & \qty{62}{\percent} & \qty{14}{\percent} & True \\
265. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.0\) & \num{< 1e-5} & \qty{94}{\percent} & \qty{14}{\percent} & False \\
266. & \lp[0] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.0\) & \num{< 1e-5} & \qty{80}{\percent} & \qty{14}{\percent} & True \\
267. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Dataset}=\phishing{}\) & \num{< 2.2e-308} & \qty{91}{\percent} & \qty{14}{\percent} & False \\
268. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Dataset}=\phishing{}\) & \num{< 1e-5} & \qty{77}{\percent} & \qty{14}{\percent} & True \\
269. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Dataset}=\phishing{}\) & \num{< 1e-5} & \qty{59}{\percent} & \qty{14}{\percent} & False \\
270. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Dataset}=\phishing{}\) & \num{< 1e-5} & \qty{74}{\percent} & \qty{14}{\percent} & True \\
271. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.1\) & \num{< 1e-5} & \qty{93}{\percent} & \qty{14}{\percent} & False \\
272. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.1\) & \num{< 1e-5} & \qty{79}{\percent} & \qty{14}{\percent} & True \\
273. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Saliency Map}=\jsmasmapfull{}\) & \num{< 1e-5} & \qty{60}{\percent} & \qty{14}{\percent} & False \\
274. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Saliency Map}=\jsmasmapfull{}\) & \num{< 2.2e-308} & \qty{75}{\percent} & \qty{14}{\percent} & True \\
275. & \dfsmapfull{} & is better than &  \identitysmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.0\) & \num{8.4e-01} & \qty{62}{\percent} & \qty{14}{\percent} & False \\
276. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.0\) & \num{1.4e-01} & \qty{51}{\percent} & \qty{14}{\percent} & True \\
277. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.5\) & \num{4.9e-01} & \qty{50}{\percent} & \qty{14}{\percent} & False \\
278. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.5\) & \num{1.1e-03} & \qty{64}{\percent} & \qty{14}{\percent} & True \\
279. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[inf]+2.0\) & \num{< 1e-5} & \qty{75}{\percent} & \qty{14}{\percent} & False \\
280. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[inf]+2.0\) & \num{< 1e-5} & \qty{61}{\percent} & \qty{14}{\percent} & True \\
281. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.1\) & \num{< 1e-5} & \qty{66}{\percent} & \qty{14}{\percent} & False \\
282. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.1\) & \num{9.3e-01} & \qty{52}{\percent} & \qty{14}{\percent} & True \\
283. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.4\) & \num{< 1e-5} & \qty{66}{\percent} & \qty{14}{\percent} & False \\
284. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.4\) & \num{7.2e-01} & \qty{47}{\percent} & \qty{14}{\percent} & True \\
285. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.0\) & \num{5.0e-02} & \qty{55}{\percent} & \qty{14}{\percent} & False \\
286. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.0\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{14}{\percent} & True \\
287. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\lp{}-\mathtt{target}=\lp[2]\) & \num{< 1e-5} & \qty{58}{\percent} & \qty{14}{\percent} & False \\
288. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\lp{}-\mathtt{target}=\lp[2]\) & \num{< 1e-5} & \qty{55}{\percent} & \qty{14}{\percent} & True \\
289. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Dataset}=\mnist{}\) & \num{< 2.2e-308} & \qty{80}{\percent} & \qty{13}{\percent} & False \\
290. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Dataset}=\mnist{}\) & \num{< 2.2e-308} & \qty{94}{\percent} & \qty{13}{\percent} & True \\
291. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.6\) & \num{1.4e-01} & \qty{50}{\percent} & \qty{13}{\percent} & False \\
292. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.6\) & \num{6.2e-04} & \qty{64}{\percent} & \qty{13}{\percent} & True \\
293. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.3\) & \num{8.4e-02} & \qty{52}{\percent} & \qty{13}{\percent} & False \\
294. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.3\) & \num{1.1e-03} & \qty{66}{\percent} & \qty{13}{\percent} & True \\
295. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Saliency Map}=\dfsmapfull{}\) & \num{< 2.2e-308} & \qty{78}{\percent} & \qty{13}{\percent} & False \\
296. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Saliency Map}=\dfsmapfull{}\) & \num{< 1e-5} & \qty{64}{\percent} & \qty{13}{\percent} & True \\
297. & \cwlossfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Dataset}=\mnist{}\) & \num{< 1e-5} & \qty{64}{\percent} & \qty{13}{\percent} & False \\
298. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Dataset}=\mnist{}\) & \num{< 1e-5} & \qty{49}{\percent} & \qty{13}{\percent} & True \\
299. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Dataset}=\mnist{}\) & \num{2.7e-02} & \qty{59}{\percent} & \qty{13}{\percent} & False \\
300. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Dataset}=\mnist{}\) & \num{< 1e-5} & \qty{45}{\percent} & \qty{13}{\percent} & True \\
301. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.3\) & \num{< 1e-5} & \qty{66}{\percent} & \qty{13}{\percent} & False \\
302. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.3\) & \num{8.5e-01} & \qty{46}{\percent} & \qty{13}{\percent} & True \\
303. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.7\) & \num{2.6e-02} & \qty{51}{\percent} & \qty{13}{\percent} & False \\
304. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.7\) & \num{4.4e-04} & \qty{65}{\percent} & \qty{13}{\percent} & True \\
305. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.0\) & \num{< 1e-5} & \qty{61}{\percent} & \qty{13}{\percent} & False \\
306. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.0\) & \num{< 1e-5} & \qty{47}{\percent} & \qty{13}{\percent} & True \\
307. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Solver}=\sgd{}\) & \num{< 1e-5} & \qty{58}{\percent} & \qty{13}{\percent} & False \\
308. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Solver}=\sgd{}\) & \num{< 1e-5} & \qty{54}{\percent} & \qty{13}{\percent} & True \\
309. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.9\) & \num{< 1e-5} & \qty{75}{\percent} & \qty{13}{\percent} & False \\
310. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.9\) & \num{< 1e-5} & \qty{61}{\percent} & \qty{13}{\percent} & True \\
311. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Saliency Map}=\identitysmapfull{}\) & \num{< 2.2e-308} & \qty{71}{\percent} & \qty{12}{\percent} & False \\
312. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Saliency Map}=\identitysmapfull{}\) & \num{< 1e-5} & \qty{58}{\percent} & \qty{12}{\percent} & True \\
313. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.1\) & \num{1.1e-04} & \qty{59}{\percent} & \qty{12}{\percent} & False \\
314. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.1\) & \num{< 1e-5} & \qty{72}{\percent} & \qty{12}{\percent} & True \\
315. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.8\) & \num{< 1e-5} & \qty{75}{\percent} & \qty{12}{\percent} & False \\
316. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.8\) & \num{< 1e-5} & \qty{62}{\percent} & \qty{12}{\percent} & True \\
317. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Saliency Map}=\jsmasmapfull{}\) & \num{< 1e-5} & \qty{67}{\percent} & \qty{12}{\percent} & False \\
318. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Saliency Map}=\jsmasmapfull{}\) & \num{< 1e-5} & \qty{54}{\percent} & \qty{12}{\percent} & True \\
319. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.1\) & \num{< 1e-5} & \qty{53}{\percent} & \qty{12}{\percent} & False \\
320. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.1\) & \num{4.5e-02} & \qty{41}{\percent} & \qty{12}{\percent} & True \\
321. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.0\) & \num{2.1e-02} & \qty{53}{\percent} & \qty{12}{\percent} & False \\
322. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.0\) & \num{< 1e-5} & \qty{66}{\percent} & \qty{12}{\percent} & True \\
323. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.4\) & \num{3.8e-02} & \qty{53}{\percent} & \qty{12}{\percent} & False \\
324. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.4\) & \num{1.0e-03} & \qty{65}{\percent} & \qty{12}{\percent} & True \\
325. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\rr{}=\textit{Disabled}\) & \num{< 1e-5} & \qty{60}{\percent} & \qty{12}{\percent} & False \\
326. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\rr{}=\textit{Disabled}\) & \num{< 1e-5} & \qty{51}{\percent} & \qty{12}{\percent} & True \\
327. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.1\) & \num{< 1e-5} & \qty{62}{\percent} & \qty{12}{\percent} & False \\
328. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.1\) & \num{< 1e-5} & \qty{50}{\percent} & \qty{12}{\percent} & True \\
329. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\cov{}=\textit{Disabled}\) & \num{< 2.2e-308} & \qty{79}{\percent} & \qty{12}{\percent} & False \\
330. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\cov{}=\textit{Disabled}\) & \num{< 2.2e-308} & \qty{67}{\percent} & \qty{12}{\percent} & True \\
331. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\lp{}-\mathtt{target}=\lp[2]\) & \num{2.2e-01} & \qty{50}{\percent} & \qty{12}{\percent} & False \\
332. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\lp{}-\mathtt{target}=\lp[2]\) & \num{< 1e-5} & \qty{61}{\percent} & \qty{12}{\percent} & True \\
333. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.0\) & \num{1.7e-01} & \qty{49}{\percent} & \qty{11}{\percent} & False \\
334. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.0\) & \num{< 1e-5} & \qty{62}{\percent} & \qty{11}{\percent} & True \\
335. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.7\) & \num{< 1e-5} & \qty{75}{\percent} & \qty{11}{\percent} & False \\
336. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.7\) & \num{< 1e-5} & \qty{63}{\percent} & \qty{11}{\percent} & True \\
337. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Solver}=\adam{}\) & \num{< 1e-5} & \qty{58}{\percent} & \qty{11}{\percent} & False \\
338. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Solver}=\adam{}\) & \num{< 1e-5} & \qty{70}{\percent} & \qty{11}{\percent} & True \\
339. & \adam{} & is better than &  \sgd{} & when & \(\lp{}-\mathtt{target}=\lp[2]\) & \num{< 2.2e-308} & \qty{69}{\percent} & \qty{11}{\percent} & False \\
340. & \adam{} & is better than &  \sgd{} & when & \(\lp{}-\mathtt{target}=\lp[2]\) & \num{< 1e-5} & \qty{58}{\percent} & \qty{11}{\percent} & True \\
341. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.1\) & \num{< 1e-5} & \qty{68}{\percent} & \qty{11}{\percent} & False \\
342. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.1\) & \num{< 1e-5} & \qty{56}{\percent} & \qty{11}{\percent} & True \\
343. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Saliency Map}=\dfsmapfull{}\) & \num{< 2.2e-308} & \qty{77}{\percent} & \qty{11}{\percent} & False \\
344. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Saliency Map}=\dfsmapfull{}\) & \num{< 1e-5} & \qty{66}{\percent} & \qty{11}{\percent} & True \\
345. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Loss}=\identitylossfull{}\) & \num{< 2.2e-308} & \qty{71}{\percent} & \qty{11}{\percent} & False \\
346. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Loss}=\identitylossfull{}\) & \num{< 2.2e-308} & \qty{83}{\percent} & \qty{11}{\percent} & True \\
347. & \lp[\infty] & is better than &  \lp[2] & when & \(\rr{}=\textit{Disabled}\) & \num{< 1e-5} & \qty{57}{\percent} & \qty{11}{\percent} & False \\
348. & \lp[\infty] & is better than &  \lp[2] & when & \(\rr{}=\textit{Disabled}\) & \num{< 1e-5} & \qty{46}{\percent} & \qty{11}{\percent} & True \\
349. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.8\) & \num{4.4e-03} & \qty{53}{\percent} & \qty{11}{\percent} & False \\
350. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.8\) & \num{3.8e-04} & \qty{64}{\percent} & \qty{11}{\percent} & True \\
351. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.1\) & \num{1.1e-04} & \qty{57}{\percent} & \qty{11}{\percent} & False \\
352. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.1\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{11}{\percent} & True \\
353. & \jsmasmapfull{} & is better than &  \identitysmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.0\) & \num{< 1e-5} & \qty{60}{\percent} & \qty{11}{\percent} & False \\
354. & \jsmasmapfull{} & is better than &  \identitysmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.0\) & \num{2.8e-01} & \qty{48}{\percent} & \qty{11}{\percent} & True \\
355. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Saliency Map}=\identitysmapfull{}\) & \num{< 2.2e-308} & \qty{78}{\percent} & \qty{11}{\percent} & False \\
356. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Saliency Map}=\identitysmapfull{}\) & \num{< 2.2e-308} & \qty{89}{\percent} & \qty{11}{\percent} & True \\
357. & \cwlossfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Saliency Map}=\jsmasmapfull{}\) & \num{< 1e-5} & \qty{51}{\percent} & \qty{11}{\percent} & False \\
358. & \cwlossfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Saliency Map}=\jsmasmapfull{}\) & \num{< 1e-5} & \qty{62}{\percent} & \qty{11}{\percent} & True \\
359. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\cov{}=\textit{Enabled}\) & \num{< 1e-5} & \qty{58}{\percent} & \qty{11}{\percent} & False \\
360. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\cov{}=\textit{Enabled}\) & \num{< 1e-5} & \qty{53}{\percent} & \qty{11}{\percent} & True \\
361. & \sgd{} & is better than &  \adam{} & when & \(\lp{}-\mathtt{target}=\lp[\infty]\) & \num{< 1e-5} & \qty{67}{\percent} & \qty{11}{\percent} & False \\
362. & \adam{} & is better than &  \sgd{} & when & \(\lp{}-\mathtt{target}=\lp[\infty]\) & \num{< 1e-5} & \qty{44}{\percent} & \qty{11}{\percent} & True \\
363. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.8\) & \num{< 1e-5} & \qty{88}{\percent} & \qty{11}{\percent} & False \\
364. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.8\) & \num{< 1e-5} & \qty{77}{\percent} & \qty{11}{\percent} & True \\
365. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.1\) & \num{< 1e-5} & \qty{89}{\percent} & \qty{11}{\percent} & False \\
366. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.1\) & \num{< 1e-5} & \qty{78}{\percent} & \qty{11}{\percent} & True \\
367. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.3\) & \num{< 1e-5} & \qty{90}{\percent} & \qty{11}{\percent} & False \\
368. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.3\) & \num{< 1e-5} & \qty{79}{\percent} & \qty{11}{\percent} & True \\
369. & \cwlossfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.0\) & \num{1.1e-03} & \qty{53}{\percent} & \qty{11}{\percent} & False \\
370. & \cwlossfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.0\) & \num{1.9e-02} & \qty{64}{\percent} & \qty{11}{\percent} & True \\
371. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.5\) & \num{1.8e-02} & \qty{54}{\percent} & \qty{11}{\percent} & False \\
372. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.5\) & \num{1.1e-03} & \qty{65}{\percent} & \qty{11}{\percent} & True \\
373. & \lp[2] & is better than &  \lp[0] & when & \(\rr{}=\textit{Enabled}\) & \num{< 2.2e-308} & \qty{67}{\percent} & \qty{11}{\percent} & False \\
374. & \lp[2] & is better than &  \lp[0] & when & \(\rr{}=\textit{Enabled}\) & \num{< 2.2e-308} & \qty{78}{\percent} & \qty{11}{\percent} & True \\
375. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Dataset}=\unswnb{}\) & \num{< 1e-5} & \qty{54}{\percent} & \qty{10}{\percent} & False \\
376. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Dataset}=\unswnb{}\) & \num{2.3e-03} & \qty{44}{\percent} & \qty{10}{\percent} & True \\
377. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.0\) & \num{< 1e-5} & \qty{67}{\percent} & \qty{10}{\percent} & False \\
378. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.0\) & \num{< 1e-5} & \qty{56}{\percent} & \qty{10}{\percent} & True \\
379. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Loss}=\crossentropyfull{}\) & \num{< 1e-5} & \qty{62}{\percent} & \qty{10}{\percent} & False \\
380. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Loss}=\crossentropyfull{}\) & \num{< 2.2e-308} & \qty{73}{\percent} & \qty{10}{\percent} & True \\
381. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Dataset}=\mnist{}\) & \num{< 1e-5} & \qty{62}{\percent} & \qty{10}{\percent} & False \\
382. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Dataset}=\mnist{}\) & \num{< 2.2e-308} & \qty{73}{\percent} & \qty{10}{\percent} & True \\
383. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.2\) & \num{< 1e-5} & \qty{82}{\percent} & \qty{10}{\percent} & False \\
384. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.2\) & \num{< 1e-5} & \qty{71}{\percent} & \qty{10}{\percent} & True \\
385. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.6\) & \num{< 1e-5} & \qty{88}{\percent} & \qty{10}{\percent} & False \\
386. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.6\) & \num{< 1e-5} & \qty{77}{\percent} & \qty{10}{\percent} & True \\
387. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.7\) & \num{< 1e-5} & \qty{88}{\percent} & \qty{10}{\percent} & False \\
388. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.7\) & \num{< 1e-5} & \qty{77}{\percent} & \qty{10}{\percent} & True \\
389. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.9\) & \num{< 1e-5} & \qty{88}{\percent} & \qty{10}{\percent} & False \\
390. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.9\) & \num{< 1e-5} & \qty{77}{\percent} & \qty{10}{\percent} & True \\
391. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.0\) & \num{< 1e-5} & \qty{88}{\percent} & \qty{10}{\percent} & False \\
392. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.0\) & \num{< 1e-5} & \qty{78}{\percent} & \qty{10}{\percent} & True \\
393. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.2\) & \num{< 1e-5} & \qty{89}{\percent} & \qty{10}{\percent} & False \\
394. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.2\) & \num{< 1e-5} & \qty{78}{\percent} & \qty{10}{\percent} & True \\
395. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.6\) & \num{< 1e-5} & \qty{75}{\percent} & \qty{10}{\percent} & False \\
396. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.6\) & \num{< 1e-5} & \qty{64}{\percent} & \qty{10}{\percent} & True \\
397. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Dataset}=\phishing{}\) & \num{< 1e-5} & \qty{72}{\percent} & \qty{10}{\percent} & False \\
398. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Dataset}=\phishing{}\) & \num{< 1e-5} & \qty{62}{\percent} & \qty{10}{\percent} & True \\
399. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.1\) & \num{1.2e-01} & \qty{52}{\percent} & \qty{10}{\percent} & False \\
400. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.1\) & \num{< 1e-5} & \qty{58}{\percent} & \qty{10}{\percent} & True \\
401. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.2\) & \num{< 1e-5} & \qty{68}{\percent} & \qty{10}{\percent} & False \\
402. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.2\) & \num{< 1e-5} & \qty{57}{\percent} & \qty{10}{\percent} & True \\
403. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.4\) & \num{< 1e-5} & \qty{90}{\percent} & \qty{10}{\percent} & False \\
404. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.4\) & \num{< 1e-5} & \qty{80}{\percent} & \qty{10}{\percent} & True \\
405. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.0\) & \num{< 1e-5} & \qty{100}{\percent} & \qty{10}{\percent} & False \\
406. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.0\) & \num{< 1e-5} & \qty{89}{\percent} & \qty{10}{\percent} & True \\
407. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.1\) & \num{< 1e-5} & \qty{100}{\percent} & \qty{10}{\percent} & False \\
408. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.1\) & \num{< 1e-5} & \qty{89}{\percent} & \qty{10}{\percent} & True \\
409. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.5\) & \num{< 1e-5} & \qty{75}{\percent} & \qty{10}{\percent} & False \\
410. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.5\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{10}{\percent} & True \\
411. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Dataset}=\nslkdd{}\) & \num{< 1e-5} & \qty{81}{\percent} & \qty{10}{\percent} & False \\
412. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Dataset}=\nslkdd{}\) & \num{< 1e-5} & \qty{70}{\percent} & \qty{10}{\percent} & True \\
413. & \lp[\infty] & is better than &  \lp[2] & when & \(\cov{}=\textit{Enabled}\) & \num{< 1e-5} & \qty{49}{\percent} & \qty{10}{\percent} & False \\
414. & \lp[2] & is better than &  \lp[\infty] & when & \(\cov{}=\textit{Enabled}\) & \num{< 1e-5} & \qty{60}{\percent} & \qty{10}{\percent} & True \\
415. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.3\) & \num{< 1e-5} & \qty{67}{\percent} & \qty{10}{\percent} & False \\
416. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.3\) & \num{< 1e-5} & \qty{56}{\percent} & \qty{10}{\percent} & True \\
417. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.6\) & \num{1.4e-02} & \qty{54}{\percent} & \qty{10}{\percent} & False \\
418. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.6\) & \num{4.3e-05} & \qty{56}{\percent} & \qty{10}{\percent} & True \\
419. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.5\) & \num{< 1e-5} & \qty{90}{\percent} & \qty{10}{\percent} & False \\
420. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.5\) & \num{< 1e-5} & \qty{80}{\percent} & \qty{10}{\percent} & True \\
421. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\lp{}-\mathtt{target}=\lp[\infty]\) & \num{< 2.2e-308} & \qty{78}{\percent} & \qty{10}{\percent} & False \\
422. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\lp{}-\mathtt{target}=\lp[\infty]\) & \num{< 2.2e-308} & \qty{68}{\percent} & \qty{10}{\percent} & True \\
423. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Dataset}=\fmnist{}\) & \num{< 2.2e-308} & \qty{63}{\percent} & \qty{10}{\percent} & False \\
424. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Dataset}=\fmnist{}\) & \num{< 2.2e-308} & \qty{74}{\percent} & \qty{10}{\percent} & True \\
425. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Dataset}=\nslkdd{}\) & \num{< 1e-5} & \qty{53}{\percent} & \qty{10}{\percent} & False \\
426. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Dataset}=\nslkdd{}\) & \num{< 1e-5} & \qty{63}{\percent} & \qty{10}{\percent} & True \\
427. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.1\) & \num{< 1e-5} & \qty{79}{\percent} & \qty{10}{\percent} & False \\
428. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.1\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{10}{\percent} & True \\
429. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.3\) & \num{4.5e-02} & \qty{53}{\percent} & \qty{9}{\percent} & False \\
430. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.3\) & \num{< 1e-5} & \qty{56}{\percent} & \qty{9}{\percent} & True \\
431. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.2\) & \num{< 1e-5} & \qty{99}{\percent} & \qty{9}{\percent} & False \\
432. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.2\) & \num{< 1e-5} & \qty{89}{\percent} & \qty{9}{\percent} & True \\
433. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Dataset}=\phishing{}\) & \num{< 2.2e-308} & \qty{83}{\percent} & \qty{9}{\percent} & False \\
434. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Dataset}=\phishing{}\) & \num{< 2.2e-308} & \qty{93}{\percent} & \qty{9}{\percent} & True \\
435. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Dataset}=\phishing{}\) & \num{< 2.2e-308} & \qty{84}{\percent} & \qty{9}{\percent} & False \\
436. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Dataset}=\phishing{}\) & \num{< 1e-5} & \qty{74}{\percent} & \qty{9}{\percent} & True \\
437. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Dataset}=\unswnb{}\) & \num{< 1e-5} & \qty{68}{\percent} & \qty{9}{\percent} & False \\
438. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Dataset}=\unswnb{}\) & \num{< 1e-5} & \qty{58}{\percent} & \qty{9}{\percent} & True \\
439. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.0\) & \num{< 1e-5} & \qty{75}{\percent} & \qty{9}{\percent} & False \\
440. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.0\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{9}{\percent} & True \\
441. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.2\) & \num{7.8e-02} & \qty{53}{\percent} & \qty{9}{\percent} & False \\
442. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.2\) & \num{< 1e-5} & \qty{56}{\percent} & \qty{9}{\percent} & True \\
443. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.3\) & \num{< 1e-5} & \qty{83}{\percent} & \qty{9}{\percent} & False \\
444. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.3\) & \num{< 1e-5} & \qty{74}{\percent} & \qty{9}{\percent} & True \\
445. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.4\) & \num{< 1e-5} & \qty{84}{\percent} & \qty{9}{\percent} & False \\
446. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.4\) & \num{< 1e-5} & \qty{74}{\percent} & \qty{9}{\percent} & True \\
447. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.5\) & \num{< 1e-5} & \qty{86}{\percent} & \qty{9}{\percent} & False \\
448. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.5\) & \num{< 1e-5} & \qty{76}{\percent} & \qty{9}{\percent} & True \\
449. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.7\) & \num{9.8e-03} & \qty{54}{\percent} & \qty{9}{\percent} & False \\
450. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.7\) & \num{7.3e-05} & \qty{55}{\percent} & \qty{9}{\percent} & True \\
451. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.6\) & \num{< 1e-5} & \qty{90}{\percent} & \qty{9}{\percent} & False \\
452. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.6\) & \num{< 1e-5} & \qty{80}{\percent} & \qty{9}{\percent} & True \\
453. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+2.0\) & \num{< 1e-5} & \qty{91}{\percent} & \qty{9}{\percent} & False \\
454. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+2.0\) & \num{< 1e-5} & \qty{81}{\percent} & \qty{9}{\percent} & True \\
455. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.4\) & \num{< 1e-5} & \qty{75}{\percent} & \qty{9}{\percent} & False \\
456. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.4\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{9}{\percent} & True \\
457. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.9\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{9}{\percent} & False \\
458. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.9\) & \num{< 1e-5} & \qty{55}{\percent} & \qty{9}{\percent} & True \\
459. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\cov{}=\textit{Disabled}\) & \num{< 1e-5} & \qty{56}{\percent} & \qty{9}{\percent} & False \\
460. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\cov{}=\textit{Disabled}\) & \num{< 1e-5} & \qty{53}{\percent} & \qty{9}{\percent} & True \\
461. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Loss}=\identitylossfull{}\) & \num{< 2.2e-308} & \qty{67}{\percent} & \qty{9}{\percent} & False \\
462. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Loss}=\identitylossfull{}\) & \num{< 2.2e-308} & \qty{58}{\percent} & \qty{9}{\percent} & True \\
463. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.0\) & \num{< 1e-5} & \qty{84}{\percent} & \qty{9}{\percent} & False \\
464. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.0\) & \num{< 1e-5} & \qty{74}{\percent} & \qty{9}{\percent} & True \\
465. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.2\) & \num{< 1e-5} & \qty{64}{\percent} & \qty{9}{\percent} & False \\
466. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.2\) & \num{< 1e-5} & \qty{73}{\percent} & \qty{9}{\percent} & True \\
467. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.7\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{9}{\percent} & False \\
468. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.7\) & \num{< 1e-5} & \qty{55}{\percent} & \qty{9}{\percent} & True \\
469. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.8\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{9}{\percent} & False \\
470. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.8\) & \num{< 1e-5} & \qty{55}{\percent} & \qty{9}{\percent} & True \\
471. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.9\) & \num{6.8e-04} & \qty{55}{\percent} & \qty{9}{\percent} & False \\
472. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.9\) & \num{3.9e-04} & \qty{65}{\percent} & \qty{9}{\percent} & True \\
473. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.1\) & \num{2.3e-03} & \qty{56}{\percent} & \qty{9}{\percent} & False \\
474. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.1\) & \num{7.1e-04} & \qty{53}{\percent} & \qty{9}{\percent} & True \\
475. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.3\) & \num{< 1e-5} & \qty{64}{\percent} & \qty{9}{\percent} & False \\
476. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.3\) & \num{< 1e-5} & \qty{55}{\percent} & \qty{9}{\percent} & True \\
477. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.9\) & \num{< 1e-5} & \qty{91}{\percent} & \qty{9}{\percent} & False \\
478. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.9\) & \num{< 1e-5} & \qty{81}{\percent} & \qty{9}{\percent} & True \\
479. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.1\) & \num{< 1e-5} & \qty{70}{\percent} & \qty{9}{\percent} & False \\
480. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.1\) & \num{5.6e-04} & \qty{60}{\percent} & \qty{9}{\percent} & True \\
481. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.2\) & \num{< 1e-5} & \qty{62}{\percent} & \qty{9}{\percent} & False \\
482. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.2\) & \num{< 1e-5} & \qty{52}{\percent} & \qty{9}{\percent} & True \\
483. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.6\) & \num{8.0e-03} & \qty{55}{\percent} & \qty{9}{\percent} & False \\
484. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.6\) & \num{1.2e-03} & \qty{65}{\percent} & \qty{9}{\percent} & True \\
485. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Loss}=\cwlossfull{}\) & \num{< 1e-5} & \qty{66}{\percent} & \qty{9}{\percent} & False \\
486. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Loss}=\cwlossfull{}\) & \num{< 2.2e-308} & \qty{76}{\percent} & \qty{9}{\percent} & True \\
487. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.4\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{9}{\percent} & False \\
488. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.4\) & \num{< 1e-5} & \qty{56}{\percent} & \qty{9}{\percent} & True \\
489. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.2\) & \num{< 1e-5} & \qty{93}{\percent} & \qty{9}{\percent} & False \\
490. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.2\) & \num{< 1e-5} & \qty{84}{\percent} & \qty{9}{\percent} & True \\
491. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.2\) & \num{< 1e-5} & \qty{64}{\percent} & \qty{9}{\percent} & False \\
492. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.2\) & \num{< 1e-5} & \qty{55}{\percent} & \qty{9}{\percent} & True \\
493. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\rr{}=\textit{Enabled}\) & \num{< 1e-5} & \qty{56}{\percent} & \qty{9}{\percent} & False \\
494. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\rr{}=\textit{Enabled}\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{9}{\percent} & True \\
495. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.8\) & \num{5.9e-03} & \qty{54}{\percent} & \qty{9}{\percent} & False \\
496. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.8\) & \num{1.5e-04} & \qty{54}{\percent} & \qty{9}{\percent} & True \\
497. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.5\) & \num{2.2e-02} & \qty{53}{\percent} & \qty{9}{\percent} & False \\
498. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.5\) & \num{2.6e-05} & \qty{56}{\percent} & \qty{9}{\percent} & True \\
499. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.2\) & \num{< 1e-5} & \qty{76}{\percent} & \qty{9}{\percent} & False \\
500. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.2\) & \num{< 1e-5} & \qty{67}{\percent} & \qty{9}{\percent} & True \\
501. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.5\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{9}{\percent} & False \\
502. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.5\) & \num{< 1e-5} & \qty{56}{\percent} & \qty{9}{\percent} & True \\
503. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.6\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{9}{\percent} & False \\
504. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.6\) & \num{< 1e-5} & \qty{56}{\percent} & \qty{9}{\percent} & True \\
505. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.0\) & \num{< 1e-5} & \qty{64}{\percent} & \qty{9}{\percent} & False \\
506. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.0\) & \num{< 1e-5} & \qty{55}{\percent} & \qty{9}{\percent} & True \\
507. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.4\) & \num{< 1e-5} & \qty{64}{\percent} & \qty{9}{\percent} & False \\
508. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.4\) & \num{< 1e-5} & \qty{55}{\percent} & \qty{9}{\percent} & True \\
509. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\lp{}-\mathtt{target}=\lp[2]\) & \num{4.0e-04} & \qty{57}{\percent} & \qty{8}{\percent} & False \\
510. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\lp{}-\mathtt{target}=\lp[2]\) & \num{< 1e-5} & \qty{66}{\percent} & \qty{8}{\percent} & True \\
511. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\lp{}-\mathtt{target}=\lp[2]\) & \num{< 1e-5} & \qty{68}{\percent} & \qty{8}{\percent} & False \\
512. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\lp{}-\mathtt{target}=\lp[2]\) & \num{< 1e-5} & \qty{59}{\percent} & \qty{8}{\percent} & True \\
513. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.1\) & \num{< 1e-5} & \qty{63}{\percent} & \qty{8}{\percent} & False \\
514. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.1\) & \num{3.2e-03} & \qty{54}{\percent} & \qty{8}{\percent} & True \\
515. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.4\) & \num{3.4e-02} & \qty{52}{\percent} & \qty{8}{\percent} & False \\
516. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.4\) & \num{1.0e-05} & \qty{56}{\percent} & \qty{8}{\percent} & True \\
517. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.0\) & \num{1.4e-04} & \qty{55}{\percent} & \qty{8}{\percent} & False \\
518. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.0\) & \num{4.3e-04} & \qty{64}{\percent} & \qty{8}{\percent} & True \\
519. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.1\) & \num{< 1e-5} & \qty{64}{\percent} & \qty{8}{\percent} & False \\
520. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.1\) & \num{< 1e-5} & \qty{55}{\percent} & \qty{8}{\percent} & True \\
521. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.3\) & \num{9.4e-04} & \qty{56}{\percent} & \qty{8}{\percent} & False \\
522. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.3\) & \num{1.6e-03} & \qty{52}{\percent} & \qty{8}{\percent} & True \\
523. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.4\) & \num{6.5e-04} & \qty{56}{\percent} & \qty{8}{\percent} & False \\
524. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.4\) & \num{2.1e-03} & \qty{52}{\percent} & \qty{8}{\percent} & True \\
525. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.5\) & \num{4.9e-04} & \qty{55}{\percent} & \qty{8}{\percent} & False \\
526. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.5\) & \num{2.6e-03} & \qty{53}{\percent} & \qty{8}{\percent} & True \\
527. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.6\) & \num{3.6e-04} & \qty{55}{\percent} & \qty{8}{\percent} & False \\
528. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.6\) & \num{3.0e-03} & \qty{53}{\percent} & \qty{8}{\percent} & True \\
529. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.7\) & \num{2.9e-04} & \qty{55}{\percent} & \qty{8}{\percent} & False \\
530. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.7\) & \num{3.4e-03} & \qty{53}{\percent} & \qty{8}{\percent} & True \\
531. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.8\) & \num{1.8e-04} & \qty{55}{\percent} & \qty{8}{\percent} & False \\
532. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.8\) & \num{3.9e-03} & \qty{53}{\percent} & \qty{8}{\percent} & True \\
533. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+2.0\) & \num{8.3e-05} & \qty{55}{\percent} & \qty{8}{\percent} & False \\
534. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+2.0\) & \num{5.1e-03} & \qty{53}{\percent} & \qty{8}{\percent} & True \\
535. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.7\) & \num{< 1e-5} & \qty{90}{\percent} & \qty{8}{\percent} & False \\
536. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.7\) & \num{< 1e-5} & \qty{81}{\percent} & \qty{8}{\percent} & True \\
537. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.8\) & \num{< 1e-5} & \qty{90}{\percent} & \qty{8}{\percent} & False \\
538. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.8\) & \num{< 1e-5} & \qty{81}{\percent} & \qty{8}{\percent} & True \\
539. & \adam{} & is better than &  \sgd{} & when & \(\lp{}-\mathtt{target}=\lp[0]\) & \num{< 2.2e-308} & \qty{98}{\percent} & \qty{8}{\percent} & False \\
540. & \adam{} & is better than &  \sgd{} & when & \(\lp{}-\mathtt{target}=\lp[0]\) & \num{< 2.2e-308} & \qty{89}{\percent} & \qty{8}{\percent} & True \\
541. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.5\) & \num{< 1e-5} & \qty{64}{\percent} & \qty{8}{\percent} & False \\
542. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.5\) & \num{< 1e-5} & \qty{55}{\percent} & \qty{8}{\percent} & True \\
543. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.6\) & \num{< 1e-5} & \qty{64}{\percent} & \qty{8}{\percent} & False \\
544. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.6\) & \num{< 1e-5} & \qty{55}{\percent} & \qty{8}{\percent} & True \\
545. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.7\) & \num{< 1e-5} & \qty{64}{\percent} & \qty{8}{\percent} & False \\
546. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.7\) & \num{< 1e-5} & \qty{55}{\percent} & \qty{8}{\percent} & True \\
547. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.4\) & \num{< 1e-5} & \qty{62}{\percent} & \qty{8}{\percent} & False \\
548. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.4\) & \num{< 1e-5} & \qty{54}{\percent} & \qty{8}{\percent} & True \\
549. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Solver}=\sgd{}\) & \num{< 1e-5} & \qty{61}{\percent} & \qty{8}{\percent} & False \\
550. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Solver}=\sgd{}\) & \num{< 2.2e-308} & \qty{69}{\percent} & \qty{8}{\percent} & True \\
551. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+2.0\) & \num{< 1e-5} & \qty{77}{\percent} & \qty{8}{\percent} & False \\
552. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+2.0\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{8}{\percent} & True \\
553. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.4\) & \num{8.7e-03} & \qty{56}{\percent} & \qty{8}{\percent} & False \\
554. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.4\) & \num{3.2e-01} & \qty{48}{\percent} & \qty{8}{\percent} & True \\
555. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.9\) & \num{4.3e-03} & \qty{54}{\percent} & \qty{8}{\percent} & False \\
556. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.9\) & \num{2.6e-04} & \qty{53}{\percent} & \qty{8}{\percent} & True \\
557. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.0\) & \num{3.4e-03} & \qty{55}{\percent} & \qty{8}{\percent} & False \\
558. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.0\) & \num{4.9e-04} & \qty{53}{\percent} & \qty{8}{\percent} & True \\
559. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.3\) & \num{< 1e-5} & \qty{99}{\percent} & \qty{8}{\percent} & False \\
560. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.3\) & \num{< 1e-5} & \qty{90}{\percent} & \qty{8}{\percent} & True \\
561. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.3\) & \num{< 1e-5} & \qty{75}{\percent} & \qty{8}{\percent} & False \\
562. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.3\) & \num{< 1e-5} & \qty{67}{\percent} & \qty{8}{\percent} & True \\
563. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.2\) & \num{6.3e-03} & \qty{52}{\percent} & \qty{8}{\percent} & False \\
564. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.2\) & \num{< 1e-5} & \qty{61}{\percent} & \qty{8}{\percent} & True \\
565. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\rr{}=\textit{Enabled}\) & \num{< 1e-5} & \qty{54}{\percent} & \qty{8}{\percent} & False \\
566. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\rr{}=\textit{Enabled}\) & \num{< 1e-5} & \qty{54}{\percent} & \qty{8}{\percent} & True \\
567. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\lp{}-\mathtt{target}=\lp[0]\) & \num{< 2.2e-308} & \qty{70}{\percent} & \qty{8}{\percent} & False \\
568. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\lp{}-\mathtt{target}=\lp[0]\) & \num{< 1e-5} & \qty{62}{\percent} & \qty{8}{\percent} & True \\
569. & \lp[\infty] & is better than &  \lp[2] & when & \(\cov{}=\textit{Disabled}\) & \num{< 2.2e-308} & \qty{65}{\percent} & \qty{8}{\percent} & False \\
570. & \lp[\infty] & is better than &  \lp[2] & when & \(\cov{}=\textit{Disabled}\) & \num{< 1e-5} & \qty{57}{\percent} & \qty{8}{\percent} & True \\
571. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Solver}=\adam{}\) & \num{< 1e-5} & \qty{51}{\percent} & \qty{8}{\percent} & False \\
572. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Solver}=\adam{}\) & \num{< 1e-5} & \qty{59}{\percent} & \qty{8}{\percent} & True \\
573. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\lp{}-\mathtt{target}=\lp[0]\) & \num{< 1e-5} & \qty{58}{\percent} & \qty{8}{\percent} & False \\
574. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\lp{}-\mathtt{target}=\lp[0]\) & \num{1.8e-01} & \qty{49}{\percent} & \qty{8}{\percent} & True \\
575. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Dataset}=\unswnb{}\) & \num{< 1e-5} & \qty{73}{\percent} & \qty{8}{\percent} & False \\
576. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Dataset}=\unswnb{}\) & \num{< 2.2e-308} & \qty{81}{\percent} & \qty{8}{\percent} & True \\
577. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Dataset}=\phishing{}\) & \num{< 1e-5} & \qty{59}{\percent} & \qty{8}{\percent} & False \\
578. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Dataset}=\phishing{}\) & \num{< 1e-5} & \qty{51}{\percent} & \qty{8}{\percent} & True \\
579. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.1\) & \num{< 1e-5} & \qty{77}{\percent} & \qty{8}{\percent} & False \\
580. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.1\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{8}{\percent} & True \\
581. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.8\) & \num{< 1e-5} & \qty{77}{\percent} & \qty{8}{\percent} & False \\
582. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.8\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{8}{\percent} & True \\
583. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.9\) & \num{< 1e-5} & \qty{77}{\percent} & \qty{8}{\percent} & False \\
584. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.9\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{8}{\percent} & True \\
585. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.3\) & \num{7.2e-03} & \qty{56}{\percent} & \qty{8}{\percent} & False \\
586. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.3\) & \num{3.8e-01} & \qty{48}{\percent} & \qty{8}{\percent} & True \\
587. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.7\) & \num{1.8e-02} & \qty{57}{\percent} & \qty{8}{\percent} & False \\
588. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.7\) & \num{1.9e-01} & \qty{49}{\percent} & \qty{8}{\percent} & True \\
589. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.2\) & \num{1.5e-03} & \qty{55}{\percent} & \qty{8}{\percent} & False \\
590. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.2\) & \num{1.0e-03} & \qty{53}{\percent} & \qty{8}{\percent} & True \\
591. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.8\) & \num{< 1e-5} & \qty{64}{\percent} & \qty{8}{\percent} & False \\
592. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.8\) & \num{< 1e-5} & \qty{55}{\percent} & \qty{8}{\percent} & True \\
593. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.0\) & \num{< 1e-5} & \qty{76}{\percent} & \qty{8}{\percent} & False \\
594. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.0\) & \num{< 1e-5} & \qty{68}{\percent} & \qty{8}{\percent} & True \\
595. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Loss}=\crossentropyfull{}\) & \num{2.7e-05} & \qty{52}{\percent} & \qty{8}{\percent} & False \\
596. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Loss}=\crossentropyfull{}\) & \num{2.7e-01} & \qty{44}{\percent} & \qty{8}{\percent} & True \\
597. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\rr{}=\textit{Disabled}\) & \num{< 1e-5} & \qty{56}{\percent} & \qty{8}{\percent} & False \\
598. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\rr{}=\textit{Disabled}\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{8}{\percent} & True \\
599. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[2]+2.0\) & \num{< 1e-5} & \qty{64}{\percent} & \qty{8}{\percent} & False \\
600. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[2]+2.0\) & \num{< 1e-5} & \qty{56}{\percent} & \qty{8}{\percent} & True \\
601. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.3\) & \num{< 1e-5} & \qty{62}{\percent} & \qty{8}{\percent} & False \\
602. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.3\) & \num{< 1e-5} & \qty{54}{\percent} & \qty{8}{\percent} & True \\
603. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\lp{}-\mathtt{target}=\lp[2]\) & \num{< 1e-5} & \qty{52}{\percent} & \qty{8}{\percent} & False \\
604. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\lp{}-\mathtt{target}=\lp[2]\) & \num{< 1e-5} & \qty{60}{\percent} & \qty{8}{\percent} & True \\
605. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Solver}=\adam{}\) & \num{< 2.2e-308} & \qty{74}{\percent} & \qty{8}{\percent} & False \\
606. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Solver}=\adam{}\) & \num{< 2.2e-308} & \qty{66}{\percent} & \qty{8}{\percent} & True \\
607. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.2\) & \num{< 1e-5} & \qty{77}{\percent} & \qty{8}{\percent} & False \\
608. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.2\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{8}{\percent} & True \\
609. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.3\) & \num{< 1e-5} & \qty{77}{\percent} & \qty{8}{\percent} & False \\
610. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.3\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{8}{\percent} & True \\
611. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.4\) & \num{< 1e-5} & \qty{77}{\percent} & \qty{8}{\percent} & False \\
612. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.4\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{8}{\percent} & True \\
613. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.6\) & \num{< 1e-5} & \qty{77}{\percent} & \qty{8}{\percent} & False \\
614. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.6\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{8}{\percent} & True \\
615. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.7\) & \num{< 1e-5} & \qty{77}{\percent} & \qty{8}{\percent} & False \\
616. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.7\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{8}{\percent} & True \\
617. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.9\) & \num{1.3e-04} & \qty{55}{\percent} & \qty{8}{\percent} & False \\
618. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.9\) & \num{4.4e-03} & \qty{53}{\percent} & \qty{8}{\percent} & True \\
619. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.7\) & \num{3.6e-03} & \qty{56}{\percent} & \qty{8}{\percent} & False \\
620. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.7\) & \num{1.3e-03} & \qty{65}{\percent} & \qty{8}{\percent} & True \\
621. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+2.0\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{8}{\percent} & False \\
622. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+2.0\) & \num{< 1e-5} & \qty{73}{\percent} & \qty{8}{\percent} & True \\
623. & \cwlossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.0\) & \num{4.0e-01} & \qty{50}{\percent} & \qty{8}{\percent} & False \\
624. & \cwlossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.0\) & \num{8.9e-01} & \qty{58}{\percent} & \qty{8}{\percent} & True \\
625. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.3\) & \num{< 1e-5} & \qty{61}{\percent} & \qty{8}{\percent} & False \\
626. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.3\) & \num{< 1e-5} & \qty{53}{\percent} & \qty{8}{\percent} & True \\
627. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.1\) & \num{< 1e-5} & \qty{76}{\percent} & \qty{8}{\percent} & False \\
628. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.1\) & \num{< 1e-5} & \qty{68}{\percent} & \qty{8}{\percent} & True \\
629. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.6\) & \num{1.4e-02} & \qty{56}{\percent} & \qty{8}{\percent} & False \\
630. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.6\) & \num{2.2e-01} & \qty{48}{\percent} & \qty{8}{\percent} & True \\
631. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.9\) & \num{< 1e-5} & \qty{64}{\percent} & \qty{7}{\percent} & False \\
632. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.9\) & \num{< 1e-5} & \qty{56}{\percent} & \qty{7}{\percent} & True \\
633. & \lp[\infty] & is better than &  \lp[0] & when & \(\cov{}=\textit{Disabled}\) & \num{< 1e-5} & \qty{60}{\percent} & \qty{7}{\percent} & False \\
634. & \lp[\infty] & is better than &  \lp[0] & when & \(\cov{}=\textit{Disabled}\) & \num{< 2.2e-308} & \qty{68}{\percent} & \qty{7}{\percent} & True \\
635. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Saliency Map}=\jsmasmapfull{}\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{7}{\percent} & False \\
636. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Saliency Map}=\jsmasmapfull{}\) & \num{< 2.2e-308} & \qty{77}{\percent} & \qty{7}{\percent} & True \\
637. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.0\) & \num{< 1e-5} & \qty{76}{\percent} & \qty{7}{\percent} & False \\
638. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.0\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{7}{\percent} & True \\
639. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.1\) & \num{3.6e-05} & \qty{57}{\percent} & \qty{7}{\percent} & False \\
640. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.1\) & \num{5.0e-04} & \qty{65}{\percent} & \qty{7}{\percent} & True \\
641. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.0\) & \num{2.3e-01} & \qty{49}{\percent} & \qty{7}{\percent} & False \\
642. & \cwlossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.0\) & \num{3.9e-01} & \qty{58}{\percent} & \qty{7}{\percent} & True \\
643. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.0\) & \num{8.5e-04} & \qty{55}{\percent} & \qty{7}{\percent} & False \\
644. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.0\) & \num{< 1e-5} & \qty{63}{\percent} & \qty{7}{\percent} & True \\
645. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.0\) & \num{3.7e-03} & \qty{55}{\percent} & \qty{7}{\percent} & False \\
646. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.0\) & \num{7.5e-02} & \qty{48}{\percent} & \qty{7}{\percent} & True \\
647. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.2\) & \num{< 1e-5} & \qty{63}{\percent} & \qty{7}{\percent} & False \\
648. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.2\) & \num{1.4e-04} & \qty{56}{\percent} & \qty{7}{\percent} & True \\
649. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.5\) & \num{1.1e-02} & \qty{56}{\percent} & \qty{7}{\percent} & False \\
650. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.5\) & \num{2.6e-01} & \qty{48}{\percent} & \qty{7}{\percent} & True \\
651. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.3\) & \num{< 1e-5} & \qty{74}{\percent} & \qty{7}{\percent} & False \\
652. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.3\) & \num{< 1e-5} & \qty{82}{\percent} & \qty{7}{\percent} & True \\
653. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.0\) & \num{< 1e-5} & \qty{92}{\percent} & \qty{7}{\percent} & False \\
654. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.0\) & \num{< 1e-5} & \qty{84}{\percent} & \qty{7}{\percent} & True \\
655. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.9\) & \num{< 1e-5} & \qty{61}{\percent} & \qty{7}{\percent} & False \\
656. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.9\) & \num{< 1e-5} & \qty{53}{\percent} & \qty{7}{\percent} & True \\
657. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.0\) & \num{< 1e-5} & \qty{61}{\percent} & \qty{7}{\percent} & False \\
658. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.0\) & \num{< 1e-5} & \qty{54}{\percent} & \qty{7}{\percent} & True \\
659. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+2.0\) & \num{1.7e-01} & \qty{53}{\percent} & \qty{7}{\percent} & False \\
660. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+2.0\) & \num{5.2e-04} & \qty{54}{\percent} & \qty{7}{\percent} & True \\
661. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+2.0\) & \num{< 1e-5} & \qty{62}{\percent} & \qty{7}{\percent} & False \\
662. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+2.0\) & \num{1.9e-05} & \qty{55}{\percent} & \qty{7}{\percent} & True \\
663. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Dataset}=\unswnb{}\) & \num{< 1e-5} & \qty{64}{\percent} & \qty{7}{\percent} & False \\
664. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Dataset}=\unswnb{}\) & \num{< 1e-5} & \qty{72}{\percent} & \qty{7}{\percent} & True \\
665. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\lp{}-\mathtt{target}=\lp[\infty]\) & \num{< 2.2e-308} & \qty{73}{\percent} & \qty{7}{\percent} & False \\
666. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\lp{}-\mathtt{target}=\lp[\infty]\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{7}{\percent} & True \\
667. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Solver}=\adam{}\) & \num{< 1e-5} & \qty{56}{\percent} & \qty{7}{\percent} & False \\
668. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Solver}=\adam{}\) & \num{< 1e-5} & \qty{51}{\percent} & \qty{7}{\percent} & True \\
669. & \jsmasmapfull{} & is better than &  \identitysmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.0\) & \num{< 1e-5} & \qty{72}{\percent} & \qty{7}{\percent} & False \\
670. & \jsmasmapfull{} & is better than &  \identitysmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.0\) & \num{2.7e-05} & \qty{65}{\percent} & \qty{7}{\percent} & True \\
671. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.8\) & \num{< 1e-5} & \qty{76}{\percent} & \qty{7}{\percent} & False \\
672. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.8\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{7}{\percent} & True \\
673. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.9\) & \num{< 1e-5} & \qty{76}{\percent} & \qty{7}{\percent} & False \\
674. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.9\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{7}{\percent} & True \\
675. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.5\) & \num{< 1e-5} & \qty{76}{\percent} & \qty{7}{\percent} & False \\
676. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.5\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{7}{\percent} & True \\
677. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.3\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{7}{\percent} & False \\
678. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.3\) & \num{< 1e-5} & \qty{57}{\percent} & \qty{7}{\percent} & True \\
679. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.4\) & \num{< 1e-5} & \qty{75}{\percent} & \qty{7}{\percent} & False \\
680. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.4\) & \num{< 1e-5} & \qty{82}{\percent} & \qty{7}{\percent} & True \\
681. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.8\) & \num{1.8e-03} & \qty{57}{\percent} & \qty{7}{\percent} & False \\
682. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.8\) & \num{1.3e-03} & \qty{64}{\percent} & \qty{7}{\percent} & True \\
683. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.9\) & \num{< 1e-5} & \qty{72}{\percent} & \qty{7}{\percent} & False \\
684. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.9\) & \num{< 1e-5} & \qty{80}{\percent} & \qty{7}{\percent} & True \\
685. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.0\) & \num{< 1e-5} & \qty{73}{\percent} & \qty{7}{\percent} & False \\
686. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.0\) & \num{< 1e-5} & \qty{80}{\percent} & \qty{7}{\percent} & True \\
687. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.2\) & \num{< 1e-5} & \qty{74}{\percent} & \qty{7}{\percent} & False \\
688. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.2\) & \num{< 1e-5} & \qty{81}{\percent} & \qty{7}{\percent} & True \\
689. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.2\) & \num{< 1e-5} & \qty{61}{\percent} & \qty{7}{\percent} & False \\
690. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.2\) & \num{< 1e-5} & \qty{54}{\percent} & \qty{7}{\percent} & True \\
691. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\lp{}-\mathtt{target}=\lp[\infty]\) & \num{< 1e-5} & \qty{52}{\percent} & \qty{7}{\percent} & False \\
692. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\lp{}-\mathtt{target}=\lp[\infty]\) & \num{< 1e-5} & \qty{60}{\percent} & \qty{7}{\percent} & True \\
693. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Dataset}=\unswnb{}\) & \num{< 1e-5} & \qty{70}{\percent} & \qty{7}{\percent} & False \\
694. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Dataset}=\unswnb{}\) & \num{< 2.2e-308} & \qty{78}{\percent} & \qty{7}{\percent} & True \\
695. & \lp[2] & is better than &  \lp[0] & when & \(\rr{}=\textit{Disabled}\) & \num{< 1e-5} & \qty{64}{\percent} & \qty{7}{\percent} & False \\
696. & \lp[2] & is better than &  \lp[0] & when & \(\rr{}=\textit{Disabled}\) & \num{< 2.2e-308} & \qty{71}{\percent} & \qty{7}{\percent} & True \\
697. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Loss}=\identitylossfull{}\) & \num{< 1e-5} & \qty{68}{\percent} & \qty{7}{\percent} & False \\
698. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Loss}=\identitylossfull{}\) & \num{< 2.2e-308} & \qty{75}{\percent} & \qty{7}{\percent} & True \\
699. & \lp[\infty] & is better than &  \lp[2] & when & \(\rr{}=\textit{Enabled}\) & \num{< 1e-5} & \qty{57}{\percent} & \qty{7}{\percent} & False \\
700. & \lp[\infty] & is better than &  \lp[2] & when & \(\rr{}=\textit{Enabled}\) & \num{< 1e-5} & \qty{50}{\percent} & \qty{7}{\percent} & True \\
701. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Dataset}=\fmnist{}\) & \num{< 1e-5} & \qty{57}{\percent} & \qty{7}{\percent} & False \\
702. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Dataset}=\fmnist{}\) & \num{< 1e-5} & \qty{64}{\percent} & \qty{7}{\percent} & True \\
703. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Dataset}=\phishing{}\) & \num{7.3e-03} & \qty{51}{\percent} & \qty{7}{\percent} & False \\
704. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Dataset}=\phishing{}\) & \num{< 1e-5} & \qty{55}{\percent} & \qty{7}{\percent} & True \\
705. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.9\) & \num{8.2e-04} & \qty{57}{\percent} & \qty{7}{\percent} & False \\
706. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.9\) & \num{1.3e-03} & \qty{64}{\percent} & \qty{7}{\percent} & True \\
707. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.4\) & \num{5.6e-02} & \qty{51}{\percent} & \qty{7}{\percent} & False \\
708. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.4\) & \num{< 1e-5} & \qty{59}{\percent} & \qty{7}{\percent} & True \\
709. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.4\) & \num{< 1e-5} & \qty{99}{\percent} & \qty{7}{\percent} & False \\
710. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.4\) & \num{< 1e-5} & \qty{91}{\percent} & \qty{7}{\percent} & True \\
711. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.6\) & \num{< 1e-5} & \qty{60}{\percent} & \qty{7}{\percent} & False \\
712. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.6\) & \num{< 1e-5} & \qty{53}{\percent} & \qty{7}{\percent} & True \\
713. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.9\) & \num{< 1e-5} & \qty{76}{\percent} & \qty{7}{\percent} & False \\
714. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.9\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{7}{\percent} & True \\
715. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.3\) & \num{< 1e-5} & \qty{78}{\percent} & \qty{7}{\percent} & False \\
716. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.3\) & \num{< 1e-5} & \qty{86}{\percent} & \qty{7}{\percent} & True \\
717. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.6\) & \num{4.7e-01} & \qty{52}{\percent} & \qty{7}{\percent} & False \\
718. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.6\) & \num{2.1e-04} & \qty{55}{\percent} & \qty{7}{\percent} & True \\
719. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.8\) & \num{3.1e-01} & \qty{52}{\percent} & \qty{7}{\percent} & False \\
720. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.8\) & \num{3.8e-04} & \qty{54}{\percent} & \qty{7}{\percent} & True \\
721. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.9\) & \num{2.1e-01} & \qty{52}{\percent} & \qty{7}{\percent} & False \\
722. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.9\) & \num{4.5e-04} & \qty{54}{\percent} & \qty{7}{\percent} & True \\
723. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.9\) & \num{< 1e-5} & \qty{61}{\percent} & \qty{7}{\percent} & False \\
724. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.9\) & \num{1.8e-05} & \qty{54}{\percent} & \qty{7}{\percent} & True \\
725. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.3\) & \num{< 1e-5} & \qty{66}{\percent} & \qty{7}{\percent} & False \\
726. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.3\) & \num{< 1e-5} & \qty{74}{\percent} & \qty{7}{\percent} & True \\
727. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.7\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{7}{\percent} & False \\
728. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.7\) & \num{< 1e-5} & \qty{72}{\percent} & \qty{7}{\percent} & True \\
729. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.9\) & \num{< 1e-5} & \qty{66}{\percent} & \qty{7}{\percent} & False \\
730. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.9\) & \num{< 1e-5} & \qty{73}{\percent} & \qty{7}{\percent} & True \\
731. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Dataset}=\fmnist{}\) & \num{< 2.2e-308} & \qty{97}{\percent} & \qty{7}{\percent} & False \\
732. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Dataset}=\fmnist{}\) & \num{< 2.2e-308} & \qty{90}{\percent} & \qty{7}{\percent} & True \\
733. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.1\) & \num{3.9e-03} & \qty{62}{\percent} & \qty{6}{\percent} & False \\
734. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.1\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{6}{\percent} & True \\
735. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.7\) & \num{< 1e-5} & \qty{76}{\percent} & \qty{6}{\percent} & False \\
736. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.7\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{6}{\percent} & True \\
737. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.8\) & \num{< 1e-5} & \qty{72}{\percent} & \qty{6}{\percent} & False \\
738. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.8\) & \num{< 1e-5} & \qty{79}{\percent} & \qty{6}{\percent} & True \\
739. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.1\) & \num{< 1e-5} & \qty{74}{\percent} & \qty{6}{\percent} & False \\
740. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.1\) & \num{< 1e-5} & \qty{81}{\percent} & \qty{6}{\percent} & True \\
741. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.5\) & \num{< 1e-5} & \qty{75}{\percent} & \qty{6}{\percent} & False \\
742. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.5\) & \num{< 1e-5} & \qty{82}{\percent} & \qty{6}{\percent} & True \\
743. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.1\) & \num{9.3e-02} & \qty{58}{\percent} & \qty{6}{\percent} & False \\
744. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.1\) & \num{1.6e-02} & \qty{51}{\percent} & \qty{6}{\percent} & True \\
745. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.3\) & \num{1.8e-02} & \qty{52}{\percent} & \qty{6}{\percent} & False \\
746. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.3\) & \num{< 1e-5} & \qty{59}{\percent} & \qty{6}{\percent} & True \\
747. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.4\) & \num{< 1e-5} & \qty{60}{\percent} & \qty{6}{\percent} & False \\
748. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.4\) & \num{< 1e-5} & \qty{53}{\percent} & \qty{6}{\percent} & True \\
749. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.1\) & \num{< 1e-5} & \qty{61}{\percent} & \qty{6}{\percent} & False \\
750. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.1\) & \num{< 1e-5} & \qty{54}{\percent} & \qty{6}{\percent} & True \\
751. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.5\) & \num{5.6e-01} & \qty{51}{\percent} & \qty{6}{\percent} & False \\
752. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.5\) & \num{1.4e-04} & \qty{55}{\percent} & \qty{6}{\percent} & True \\
753. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.6\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{6}{\percent} & False \\
754. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.6\) & \num{< 1e-5} & \qty{72}{\percent} & \qty{6}{\percent} & True \\
755. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.7\) & \num{4.1e-01} & \qty{52}{\percent} & \qty{6}{\percent} & False \\
756. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.7\) & \num{3.0e-04} & \qty{54}{\percent} & \qty{6}{\percent} & True \\
757. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Solver}=\adam{}\) & \num{< 2.2e-308} & \qty{70}{\percent} & \qty{6}{\percent} & False \\
758. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Solver}=\adam{}\) & \num{< 1e-5} & \qty{63}{\percent} & \qty{6}{\percent} & True \\
759. & \adam{} & is better than &  \sgd{} & when & \(\cov{}=\textit{Disabled}\) & \num{< 2.2e-308} & \qty{73}{\percent} & \qty{6}{\percent} & False \\
760. & \adam{} & is better than &  \sgd{} & when & \(\cov{}=\textit{Disabled}\) & \num{< 2.2e-308} & \qty{66}{\percent} & \qty{6}{\percent} & True \\
761. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.1\) & \num{4.6e-04} & \qty{55}{\percent} & \qty{6}{\percent} & False \\
762. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.1\) & \num{< 1e-5} & \qty{61}{\percent} & \qty{6}{\percent} & True \\
763. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.5\) & \num{< 1e-5} & \qty{60}{\percent} & \qty{6}{\percent} & False \\
764. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.5\) & \num{< 1e-5} & \qty{53}{\percent} & \qty{6}{\percent} & True \\
765. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.7\) & \num{3.1e-01} & \qty{50}{\percent} & \qty{6}{\percent} & False \\
766. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.7\) & \num{< 1e-5} & \qty{57}{\percent} & \qty{6}{\percent} & True \\
767. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.8\) & \num{< 1e-5} & \qty{60}{\percent} & \qty{6}{\percent} & False \\
768. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.8\) & \num{< 1e-5} & \qty{53}{\percent} & \qty{6}{\percent} & True \\
769. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.1\) & \num{< 1e-5} & \qty{73}{\percent} & \qty{6}{\percent} & False \\
770. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.1\) & \num{< 1e-5} & \qty{66}{\percent} & \qty{6}{\percent} & True \\
771. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.2\) & \num{< 1e-5} & \qty{73}{\percent} & \qty{6}{\percent} & False \\
772. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.2\) & \num{< 1e-5} & \qty{66}{\percent} & \qty{6}{\percent} & True \\
773. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.4\) & \num{< 1e-5} & \qty{74}{\percent} & \qty{6}{\percent} & False \\
774. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.4\) & \num{< 1e-5} & \qty{67}{\percent} & \qty{6}{\percent} & True \\
775. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.6\) & \num{< 1e-5} & \qty{75}{\percent} & \qty{6}{\percent} & False \\
776. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.6\) & \num{< 1e-5} & \qty{68}{\percent} & \qty{6}{\percent} & True \\
777. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.8\) & \num{3.4e-02} & \qty{56}{\percent} & \qty{6}{\percent} & False \\
778. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.8\) & \num{1.6e-01} & \qty{49}{\percent} & \qty{6}{\percent} & True \\
779. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.2\) & \num{< 1e-5} & \qty{58}{\percent} & \qty{6}{\percent} & False \\
780. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.2\) & \num{5.3e-04} & \qty{65}{\percent} & \qty{6}{\percent} & True \\
781. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.3\) & \num{< 1e-5} & \qty{58}{\percent} & \qty{6}{\percent} & False \\
782. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.3\) & \num{6.4e-04} & \qty{65}{\percent} & \qty{6}{\percent} & True \\
783. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.6\) & \num{< 1e-5} & \qty{76}{\percent} & \qty{6}{\percent} & False \\
784. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.6\) & \num{< 1e-5} & \qty{82}{\percent} & \qty{6}{\percent} & True \\
785. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.1\) & \num{< 1e-5} & \qty{61}{\percent} & \qty{6}{\percent} & False \\
786. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.1\) & \num{< 1e-5} & \qty{54}{\percent} & \qty{6}{\percent} & True \\
787. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.5\) & \num{1.3e-01} & \qty{51}{\percent} & \qty{6}{\percent} & False \\
788. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.5\) & \num{< 1e-5} & \qty{58}{\percent} & \qty{6}{\percent} & True \\
789. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.6\) & \num{2.1e-01} & \qty{50}{\percent} & \qty{6}{\percent} & False \\
790. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.6\) & \num{< 1e-5} & \qty{57}{\percent} & \qty{6}{\percent} & True \\
791. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.7\) & \num{< 1e-5} & \qty{60}{\percent} & \qty{6}{\percent} & False \\
792. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.7\) & \num{< 1e-5} & \qty{54}{\percent} & \qty{6}{\percent} & True \\
793. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.8\) & \num{3.6e-01} & \qty{50}{\percent} & \qty{6}{\percent} & False \\
794. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.8\) & \num{< 1e-5} & \qty{56}{\percent} & \qty{6}{\percent} & True \\
795. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.8\) & \num{< 1e-5} & \qty{77}{\percent} & \qty{6}{\percent} & False \\
796. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.8\) & \num{< 1e-5} & \qty{70}{\percent} & \qty{6}{\percent} & True \\
797. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.0\) & \num{7.1e-01} & \qty{49}{\percent} & \qty{6}{\percent} & False \\
798. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.0\) & \num{< 1e-5} & \qty{56}{\percent} & \qty{6}{\percent} & True \\
799. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.1\) & \num{9.4e-01} & \qty{49}{\percent} & \qty{6}{\percent} & False \\
800. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.1\) & \num{2.1e-05} & \qty{55}{\percent} & \qty{6}{\percent} & True \\
801. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.1\) & \num{< 1e-5} & \qty{75}{\percent} & \qty{6}{\percent} & False \\
802. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.1\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{6}{\percent} & True \\
803. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.2\) & \num{< 1e-5} & \qty{75}{\percent} & \qty{6}{\percent} & False \\
804. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.2\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{6}{\percent} & True \\
805. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.3\) & \num{< 1e-5} & \qty{75}{\percent} & \qty{6}{\percent} & False \\
806. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.3\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{6}{\percent} & True \\
807. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.8\) & \num{< 1e-5} & \qty{66}{\percent} & \qty{6}{\percent} & False \\
808. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.8\) & \num{< 1e-5} & \qty{72}{\percent} & \qty{6}{\percent} & True \\
809. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.8\) & \num{< 1e-5} & \qty{61}{\percent} & \qty{6}{\percent} & False \\
810. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.8\) & \num{1.5e-05} & \qty{55}{\percent} & \qty{6}{\percent} & True \\
811. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\lp{}-\mathtt{target}=\lp[\infty]\) & \num{< 1e-5} & \qty{59}{\percent} & \qty{6}{\percent} & False \\
812. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\lp{}-\mathtt{target}=\lp[\infty]\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{6}{\percent} & True \\
813. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Loss}=\cwlossfull{}\) & \num{< 1e-5} & \qty{53}{\percent} & \qty{6}{\percent} & False \\
814. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Loss}=\cwlossfull{}\) & \num{< 1e-5} & \qty{46}{\percent} & \qty{6}{\percent} & True \\
815. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.0\) & \num{< 1e-5} & \qty{75}{\percent} & \qty{6}{\percent} & False \\
816. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.0\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{6}{\percent} & True \\
817. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Saliency Map}=\dfsmapfull{}\) & \num{< 2.2e-308} & \qty{64}{\percent} & \qty{6}{\percent} & False \\
818. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Saliency Map}=\dfsmapfull{}\) & \num{< 1e-5} & \qty{58}{\percent} & \qty{6}{\percent} & True \\
819. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.9\) & \num{< 1e-5} & \qty{80}{\percent} & \qty{6}{\percent} & False \\
820. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.9\) & \num{< 1e-5} & \qty{86}{\percent} & \qty{6}{\percent} & True \\
821. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+2.0\) & \num{< 1e-5} & \qty{80}{\percent} & \qty{6}{\percent} & False \\
822. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+2.0\) & \num{< 1e-5} & \qty{86}{\percent} & \qty{6}{\percent} & True \\
823. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.5\) & \num{< 1e-5} & \qty{75}{\percent} & \qty{6}{\percent} & False \\
824. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.5\) & \num{< 1e-5} & \qty{68}{\percent} & \qty{6}{\percent} & True \\
825. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.2\) & \num{7.4e-03} & \qty{55}{\percent} & \qty{6}{\percent} & False \\
826. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.2\) & \num{4.7e-01} & \qty{48}{\percent} & \qty{6}{\percent} & True \\
827. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.7\) & \num{< 1e-5} & \qty{71}{\percent} & \qty{6}{\percent} & False \\
828. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.7\) & \num{< 1e-5} & \qty{78}{\percent} & \qty{6}{\percent} & True \\
829. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.0\) & \num{1.6e-05} & \qty{59}{\percent} & \qty{6}{\percent} & False \\
830. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.0\) & \num{< 1e-5} & \qty{66}{\percent} & \qty{6}{\percent} & True \\
831. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.7\) & \num{< 1e-5} & \qty{77}{\percent} & \qty{6}{\percent} & False \\
832. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.7\) & \num{< 1e-5} & \qty{71}{\percent} & \qty{6}{\percent} & True \\
833. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.0\) & \num{< 1e-5} & \qty{63}{\percent} & \qty{6}{\percent} & False \\
834. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.0\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{6}{\percent} & True \\
835. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.1\) & \num{< 1e-5} & \qty{63}{\percent} & \qty{6}{\percent} & False \\
836. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.1\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{6}{\percent} & True \\
837. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.2\) & \num{< 1e-5} & \qty{78}{\percent} & \qty{6}{\percent} & False \\
838. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.2\) & \num{< 1e-5} & \qty{85}{\percent} & \qty{6}{\percent} & True \\
839. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.4\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{6}{\percent} & False \\
840. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.4\) & \num{< 1e-5} & \qty{71}{\percent} & \qty{6}{\percent} & True \\
841. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.4\) & \num{6.8e-01} & \qty{51}{\percent} & \qty{6}{\percent} & False \\
842. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.4\) & \num{9.9e-05} & \qty{55}{\percent} & \qty{6}{\percent} & True \\
843. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.4\) & \num{< 1e-5} & \qty{61}{\percent} & \qty{6}{\percent} & False \\
844. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.4\) & \num{< 1e-5} & \qty{55}{\percent} & \qty{6}{\percent} & True \\
845. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.5\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{6}{\percent} & False \\
846. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.5\) & \num{< 1e-5} & \qty{71}{\percent} & \qty{6}{\percent} & True \\
847. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.5\) & \num{< 1e-5} & \qty{61}{\percent} & \qty{6}{\percent} & False \\
848. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.5\) & \num{< 1e-5} & \qty{55}{\percent} & \qty{6}{\percent} & True \\
849. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.6\) & \num{< 1e-5} & \qty{61}{\percent} & \qty{6}{\percent} & False \\
850. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.6\) & \num{1.0e-05} & \qty{55}{\percent} & \qty{6}{\percent} & True \\
851. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.7\) & \num{< 1e-5} & \qty{61}{\percent} & \qty{6}{\percent} & False \\
852. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.7\) & \num{1.2e-05} & \qty{55}{\percent} & \qty{6}{\percent} & True \\
853. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.8\) & \num{< 1e-5} & \qty{79}{\percent} & \qty{6}{\percent} & False \\
854. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.8\) & \num{< 1e-5} & \qty{86}{\percent} & \qty{6}{\percent} & True \\
855. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+2.0\) & \num{3.9e-04} & \qty{58}{\percent} & \qty{6}{\percent} & False \\
856. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+2.0\) & \num{1.4e-03} & \qty{65}{\percent} & \qty{6}{\percent} & True \\
857. & \lp[\infty] & is better than &  \lp[0] & when & \(\cov{}=\textit{Enabled}\) & \num{< 2.2e-308} & \qty{98}{\percent} & \qty{6}{\percent} & False \\
858. & \lp[\infty] & is better than &  \lp[0] & when & \(\cov{}=\textit{Enabled}\) & \num{< 2.2e-308} & \qty{91}{\percent} & \qty{6}{\percent} & True \\
859. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.4\) & \num{< 1e-5} & \qty{75}{\percent} & \qty{6}{\percent} & False \\
860. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.4\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{6}{\percent} & True \\
861. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.5\) & \num{< 1e-5} & \qty{75}{\percent} & \qty{6}{\percent} & False \\
862. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.5\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{6}{\percent} & True \\
863. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Dataset}=\mnist{}\) & \num{< 2.2e-308} & \qty{99}{\percent} & \qty{6}{\percent} & False \\
864. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Dataset}=\mnist{}\) & \num{< 2.2e-308} & \qty{93}{\percent} & \qty{6}{\percent} & True \\
865. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Dataset}=\phishing{}\) & \num{< 1e-5} & \qty{80}{\percent} & \qty{6}{\percent} & False \\
866. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Dataset}=\phishing{}\) & \num{< 1e-5} & \qty{74}{\percent} & \qty{6}{\percent} & True \\
867. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.6\) & \num{< 1e-5} & \qty{60}{\percent} & \qty{6}{\percent} & False \\
868. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.6\) & \num{< 1e-5} & \qty{66}{\percent} & \qty{6}{\percent} & True \\
869. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+2.0\) & \num{1.5e-04} & \qty{59}{\percent} & \qty{6}{\percent} & False \\
870. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+2.0\) & \num{5.2e-01} & \qty{46}{\percent} & \qty{6}{\percent} & True \\
871. & \jsmasmapfull{} & is better than &  \identitysmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.1\) & \num{3.2e-03} & \qty{51}{\percent} & \qty{6}{\percent} & False \\
872. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.1\) & \num{9.3e-01} & \qty{55}{\percent} & \qty{6}{\percent} & True \\
873. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.7\) & \num{< 1e-5} & \qty{60}{\percent} & \qty{6}{\percent} & False \\
874. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.7\) & \num{< 1e-5} & \qty{66}{\percent} & \qty{6}{\percent} & True \\
875. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.2\) & \num{< 1e-5} & \qty{61}{\percent} & \qty{6}{\percent} & False \\
876. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.2\) & \num{< 1e-5} & \qty{55}{\percent} & \qty{6}{\percent} & True \\
877. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.3\) & \num{< 1e-5} & \qty{61}{\percent} & \qty{6}{\percent} & False \\
878. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.3\) & \num{< 1e-5} & \qty{55}{\percent} & \qty{6}{\percent} & True \\
879. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.7\) & \num{< 1e-5} & \qty{80}{\percent} & \qty{6}{\percent} & False \\
880. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.7\) & \num{< 1e-5} & \qty{86}{\percent} & \qty{6}{\percent} & True \\
881. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Loss}=\cwlossfull{}\) & \num{< 2.2e-308} & \qty{63}{\percent} & \qty{6}{\percent} & False \\
882. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Loss}=\cwlossfull{}\) & \num{< 2.2e-308} & \qty{69}{\percent} & \qty{6}{\percent} & True \\
883. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.7\) & \num{< 1e-5} & \qty{60}{\percent} & \qty{5}{\percent} & False \\
884. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.7\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{5}{\percent} & True \\
885. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.6\) & \num{< 1e-5} & \qty{75}{\percent} & \qty{5}{\percent} & False \\
886. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.6\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{5}{\percent} & True \\
887. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.7\) & \num{< 1e-5} & \qty{75}{\percent} & \qty{5}{\percent} & False \\
888. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.7\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{5}{\percent} & True \\
889. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.8\) & \num{< 1e-5} & \qty{75}{\percent} & \qty{5}{\percent} & False \\
890. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.8\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{5}{\percent} & True \\
891. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.9\) & \num{< 1e-5} & \qty{75}{\percent} & \qty{5}{\percent} & False \\
892. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.9\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{5}{\percent} & True \\
893. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+2.0\) & \num{< 1e-5} & \qty{74}{\percent} & \qty{5}{\percent} & False \\
894. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+2.0\) & \num{< 1e-5} & \qty{68}{\percent} & \qty{5}{\percent} & True \\
895. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Loss}=\crossentropyfull{}\) & \num{< 2.2e-308} & \qty{70}{\percent} & \qty{5}{\percent} & False \\
896. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Loss}=\crossentropyfull{}\) & \num{< 2.2e-308} & \qty{64}{\percent} & \qty{5}{\percent} & True \\
897. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.1\) & \num{< 1e-5} & \qty{72}{\percent} & \qty{5}{\percent} & False \\
898. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.1\) & \num{5.3e-05} & \qty{66}{\percent} & \qty{5}{\percent} & True \\
899. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.2\) & \num{< 1e-5} & \qty{76}{\percent} & \qty{5}{\percent} & False \\
900. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.2\) & \num{< 1e-5} & \qty{71}{\percent} & \qty{5}{\percent} & True \\
901. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.9\) & \num{1.1e-04} & \qty{59}{\percent} & \qty{5}{\percent} & False \\
902. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.9\) & \num{5.5e-01} & \qty{46}{\percent} & \qty{5}{\percent} & True \\
903. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.5\) & \num{< 1e-5} & \qty{70}{\percent} & \qty{5}{\percent} & False \\
904. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.5\) & \num{< 1e-5} & \qty{76}{\percent} & \qty{5}{\percent} & True \\
905. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.5\) & \num{< 1e-5} & \qty{60}{\percent} & \qty{5}{\percent} & False \\
906. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.5\) & \num{7.8e-04} & \qty{65}{\percent} & \qty{5}{\percent} & True \\
907. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.7\) & \num{< 1e-5} & \qty{76}{\percent} & \qty{5}{\percent} & False \\
908. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.7\) & \num{< 1e-5} & \qty{82}{\percent} & \qty{5}{\percent} & True \\
909. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.2\) & \num{< 1e-5} & \qty{63}{\percent} & \qty{5}{\percent} & False \\
910. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.2\) & \num{< 1e-5} & \qty{68}{\percent} & \qty{5}{\percent} & True \\
911. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.9\) & \num{< 1e-5} & \qty{62}{\percent} & \qty{5}{\percent} & False \\
912. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.9\) & \num{< 1e-5} & \qty{68}{\percent} & \qty{5}{\percent} & True \\
913. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.4\) & \num{< 1e-5} & \qty{80}{\percent} & \qty{5}{\percent} & False \\
914. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.4\) & \num{< 1e-5} & \qty{86}{\percent} & \qty{5}{\percent} & True \\
915. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.5\) & \num{< 1e-5} & \qty{80}{\percent} & \qty{5}{\percent} & False \\
916. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.5\) & \num{< 1e-5} & \qty{86}{\percent} & \qty{5}{\percent} & True \\
917. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+2.0\) & \num{< 1e-5} & \qty{75}{\percent} & \qty{5}{\percent} & False \\
918. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+2.0\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{5}{\percent} & True \\
919. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.3\) & \num{< 1e-5} & \qty{73}{\percent} & \qty{5}{\percent} & False \\
920. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.3\) & \num{< 1e-5} & \qty{67}{\percent} & \qty{5}{\percent} & True \\
921. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.2\) & \num{9.1e-01} & \qty{51}{\percent} & \qty{5}{\percent} & False \\
922. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.2\) & \num{5.5e-05} & \qty{54}{\percent} & \qty{5}{\percent} & True \\
923. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.3\) & \num{8.0e-01} & \qty{50}{\percent} & \qty{5}{\percent} & False \\
924. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.3\) & \num{7.7e-05} & \qty{55}{\percent} & \qty{5}{\percent} & True \\
925. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.5\) & \num{< 1e-5} & \qty{60}{\percent} & \qty{5}{\percent} & False \\
926. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.5\) & \num{< 1e-5} & \qty{66}{\percent} & \qty{5}{\percent} & True \\
927. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Solver}=\sgd{}\) & \num{< 1e-5} & \qty{58}{\percent} & \qty{5}{\percent} & False \\
928. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Solver}=\sgd{}\) & \num{< 1e-5} & \qty{53}{\percent} & \qty{5}{\percent} & True \\
929. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\lp{}-\mathtt{target}=\lp[2]\) & \num{< 2.2e-308} & \qty{85}{\percent} & \qty{5}{\percent} & False \\
930. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\lp{}-\mathtt{target}=\lp[2]\) & \num{< 2.2e-308} & \qty{80}{\percent} & \qty{5}{\percent} & True \\
931. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.1\) & \num{< 1e-5} & \qty{76}{\percent} & \qty{5}{\percent} & False \\
932. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.1\) & \num{< 1e-5} & \qty{71}{\percent} & \qty{5}{\percent} & True \\
933. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.2\) & \num{< 1e-5} & \qty{60}{\percent} & \qty{5}{\percent} & False \\
934. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.2\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{5}{\percent} & True \\
935. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.3\) & \num{< 1e-5} & \qty{60}{\percent} & \qty{5}{\percent} & False \\
936. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.3\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{5}{\percent} & True \\
937. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+2.0\) & \num{< 1e-5} & \qty{77}{\percent} & \qty{5}{\percent} & False \\
938. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+2.0\) & \num{< 1e-5} & \qty{71}{\percent} & \qty{5}{\percent} & True \\
939. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.3\) & \num{< 1e-5} & \qty{93}{\percent} & \qty{5}{\percent} & False \\
940. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.3\) & \num{< 1e-5} & \qty{87}{\percent} & \qty{5}{\percent} & True \\
941. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.4\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{5}{\percent} & False \\
942. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.4\) & \num{< 1e-5} & \qty{75}{\percent} & \qty{5}{\percent} & True \\
943. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.6\) & \num{< 1e-5} & \qty{71}{\percent} & \qty{5}{\percent} & False \\
944. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+0.6\) & \num{< 1e-5} & \qty{76}{\percent} & \qty{5}{\percent} & True \\
945. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.4\) & \num{< 1e-5} & \qty{59}{\percent} & \qty{5}{\percent} & False \\
946. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.4\) & \num{7.2e-04} & \qty{65}{\percent} & \qty{5}{\percent} & True \\
947. & \cwlossfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.1\) & \num{1.6e-01} & \qty{46}{\percent} & \qty{5}{\percent} & False \\
948. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.1\) & \num{8.4e-01} & \qty{48}{\percent} & \qty{5}{\percent} & True \\
949. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.4\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{5}{\percent} & False \\
950. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.4\) & \num{< 1e-5} & \qty{70}{\percent} & \qty{5}{\percent} & True \\
951. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.5\) & \num{< 1e-5} & \qty{62}{\percent} & \qty{5}{\percent} & False \\
952. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.5\) & \num{< 1e-5} & \qty{57}{\percent} & \qty{5}{\percent} & True \\
953. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.2\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{5}{\percent} & False \\
954. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.2\) & \num{< 1e-5} & \qty{70}{\percent} & \qty{5}{\percent} & True \\
955. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.9\) & \num{< 1e-5} & \qty{76}{\percent} & \qty{5}{\percent} & False \\
956. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.9\) & \num{< 1e-5} & \qty{70}{\percent} & \qty{5}{\percent} & True \\
957. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.0\) & \num{< 1e-5} & \qty{76}{\percent} & \qty{5}{\percent} & False \\
958. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.0\) & \num{< 1e-5} & \qty{70}{\percent} & \qty{5}{\percent} & True \\
959. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Solver}=\sgd{}\) & \num{< 1e-5} & \qty{54}{\percent} & \qty{5}{\percent} & False \\
960. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Solver}=\sgd{}\) & \num{< 1e-5} & \qty{59}{\percent} & \qty{5}{\percent} & True \\
961. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Saliency Map}=\dfsmapfull{}\) & \num{< 1e-5} & \qty{59}{\percent} & \qty{5}{\percent} & False \\
962. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Saliency Map}=\dfsmapfull{}\) & \num{< 1e-5} & \qty{54}{\percent} & \qty{5}{\percent} & True \\
963. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.1\) & \num{< 1e-5} & \qty{61}{\percent} & \qty{5}{\percent} & False \\
964. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.1\) & \num{< 1e-5} & \qty{66}{\percent} & \qty{5}{\percent} & True \\
965. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.8\) & \num{< 1e-5} & \qty{60}{\percent} & \qty{5}{\percent} & False \\
966. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.8\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{5}{\percent} & True \\
967. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.1\) & \num{< 1e-5} & \qty{60}{\percent} & \qty{5}{\percent} & False \\
968. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.1\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{5}{\percent} & True \\
969. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\rr{}=\textit{Disabled}\) & \num{< 2.2e-308} & \qty{69}{\percent} & \qty{5}{\percent} & False \\
970. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\rr{}=\textit{Disabled}\) & \num{< 1e-5} & \qty{63}{\percent} & \qty{5}{\percent} & True \\
971. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Dataset}=\nslkdd{}\) & \num{< 2.2e-308} & \qty{76}{\percent} & \qty{5}{\percent} & False \\
972. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Dataset}=\nslkdd{}\) & \num{< 1e-5} & \qty{70}{\percent} & \qty{5}{\percent} & True \\
973. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.3\) & \num{< 1e-5} & \qty{76}{\percent} & \qty{5}{\percent} & False \\
974. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.3\) & \num{< 1e-5} & \qty{71}{\percent} & \qty{5}{\percent} & True \\
975. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.6\) & \num{< 1e-5} & \qty{77}{\percent} & \qty{5}{\percent} & False \\
976. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.6\) & \num{< 1e-5} & \qty{71}{\percent} & \qty{5}{\percent} & True \\
977. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.8\) & \num{< 1e-5} & \qty{77}{\percent} & \qty{5}{\percent} & False \\
978. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.8\) & \num{< 1e-5} & \qty{71}{\percent} & \qty{5}{\percent} & True \\
979. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.9\) & \num{< 1e-5} & \qty{77}{\percent} & \qty{5}{\percent} & False \\
980. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.9\) & \num{< 1e-5} & \qty{71}{\percent} & \qty{5}{\percent} & True \\
981. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.6\) & \num{< 1e-5} & \qty{60}{\percent} & \qty{5}{\percent} & False \\
982. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.6\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{5}{\percent} & True \\
983. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.3\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{5}{\percent} & False \\
984. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.3\) & \num{< 1e-5} & \qty{70}{\percent} & \qty{5}{\percent} & True \\
985. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.9\) & \num{< 1e-5} & \qty{74}{\percent} & \qty{5}{\percent} & False \\
986. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.9\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{5}{\percent} & True \\
987. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.8\) & \num{< 1e-5} & \qty{75}{\percent} & \qty{5}{\percent} & False \\
988. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.8\) & \num{< 1e-5} & \qty{70}{\percent} & \qty{5}{\percent} & True \\
989. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.6\) & \num{4.5e-05} & \qty{60}{\percent} & \qty{5}{\percent} & False \\
990. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.6\) & \num{7.0e-01} & \qty{45}{\percent} & \qty{5}{\percent} & True \\
991. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.1\) & \num{7.3e-03} & \qty{54}{\percent} & \qty{5}{\percent} & False \\
992. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.1\) & \num{6.0e-01} & \qty{49}{\percent} & \qty{5}{\percent} & True \\
993. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.2\) & \num{< 1e-5} & \qty{72}{\percent} & \qty{5}{\percent} & False \\
994. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.2\) & \num{< 1e-5} & \qty{67}{\percent} & \qty{5}{\percent} & True \\
995. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.3\) & \num{< 1e-5} & \qty{64}{\percent} & \qty{5}{\percent} & False \\
996. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.3\) & \num{< 1e-5} & \qty{70}{\percent} & \qty{5}{\percent} & True \\
997. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.6\) & \num{< 1e-5} & \qty{98}{\percent} & \qty{5}{\percent} & False \\
998. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.6\) & \num{< 1e-5} & \qty{93}{\percent} & \qty{5}{\percent} & True \\
999. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.9\) & \num{4.4e-01} & \qty{50}{\percent} & \qty{5}{\percent} & False \\
1000. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.9\) & \num{< 1e-5} & \qty{56}{\percent} & \qty{5}{\percent} & True \\
1001. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.6\) & \num{< 1e-5} & \qty{80}{\percent} & \qty{5}{\percent} & False \\
1002. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.6\) & \num{< 1e-5} & \qty{85}{\percent} & \qty{5}{\percent} & True \\
1003. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.4\) & \num{< 1e-5} & \qty{60}{\percent} & \qty{5}{\percent} & False \\
1004. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.4\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{5}{\percent} & True \\
1005. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.6\) & \num{< 1e-5} & \qty{63}{\percent} & \qty{5}{\percent} & False \\
1006. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.6\) & \num{< 1e-5} & \qty{57}{\percent} & \qty{5}{\percent} & True \\
1007. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.9\) & \num{< 1e-5} & \qty{75}{\percent} & \qty{5}{\percent} & False \\
1008. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.9\) & \num{< 1e-5} & \qty{70}{\percent} & \qty{5}{\percent} & True \\
1009. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\lp{}-\mathtt{target}=\lp[2]\) & \num{< 1e-5} & \qty{58}{\percent} & \qty{5}{\percent} & False \\
1010. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\lp{}-\mathtt{target}=\lp[2]\) & \num{< 1e-5} & \qty{53}{\percent} & \qty{5}{\percent} & True \\
1011. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Dataset}=\fmnist{}\) & \num{< 1e-5} & \qty{51}{\percent} & \qty{5}{\percent} & False \\
1012. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Dataset}=\fmnist{}\) & \num{7.0e-03} & \qty{56}{\percent} & \qty{5}{\percent} & True \\
1013. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Saliency Map}=\dfsmapfull{}\) & \num{< 1e-5} & \qty{66}{\percent} & \qty{5}{\percent} & False \\
1014. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Saliency Map}=\dfsmapfull{}\) & \num{< 2.2e-308} & \qty{71}{\percent} & \qty{5}{\percent} & True \\
1015. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Loss}=\identitylossfull{}\) & \num{< 1e-5} & \qty{54}{\percent} & \qty{5}{\percent} & False \\
1016. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Loss}=\identitylossfull{}\) & \num{< 1e-5} & \qty{49}{\percent} & \qty{5}{\percent} & True \\
1017. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.1\) & \num{< 1e-5} & \qty{71}{\percent} & \qty{5}{\percent} & False \\
1018. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.1\) & \num{< 1e-5} & \qty{66}{\percent} & \qty{5}{\percent} & True \\
1019. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.0\) & \num{< 1e-5} & \qty{60}{\percent} & \qty{5}{\percent} & False \\
1020. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.0\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{5}{\percent} & True \\
1021. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.4\) & \num{< 1e-5} & \qty{76}{\percent} & \qty{5}{\percent} & False \\
1022. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.4\) & \num{< 1e-5} & \qty{71}{\percent} & \qty{5}{\percent} & True \\
1023. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.1\) & \num{< 1e-5} & \qty{92}{\percent} & \qty{5}{\percent} & False \\
1024. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.1\) & \num{< 1e-5} & \qty{87}{\percent} & \qty{5}{\percent} & True \\
1025. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.8\) & \num{< 1e-5} & \qty{62}{\percent} & \qty{5}{\percent} & False \\
1026. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.8\) & \num{< 1e-5} & \qty{67}{\percent} & \qty{5}{\percent} & True \\
1027. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.5\) & \num{< 1e-5} & \qty{93}{\percent} & \qty{5}{\percent} & False \\
1028. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.5\) & \num{< 1e-5} & \qty{88}{\percent} & \qty{5}{\percent} & True \\
1029. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.8\) & \num{< 1e-5} & \qty{74}{\percent} & \qty{5}{\percent} & False \\
1030. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.8\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{5}{\percent} & True \\
1031. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.2\) & \num{< 1e-5} & \qty{61}{\percent} & \qty{4}{\percent} & False \\
1032. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.2\) & \num{< 1e-5} & \qty{66}{\percent} & \qty{4}{\percent} & True \\
1033. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.7\) & \num{< 1e-5} & \qty{75}{\percent} & \qty{4}{\percent} & False \\
1034. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.7\) & \num{< 1e-5} & \qty{70}{\percent} & \qty{4}{\percent} & True \\
1035. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.9\) & \num{< 1e-5} & \qty{60}{\percent} & \qty{4}{\percent} & False \\
1036. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.9\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{4}{\percent} & True \\
1037. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.7\) & \num{6.5e-05} & \qty{59}{\percent} & \qty{4}{\percent} & False \\
1038. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.7\) & \num{6.5e-01} & \qty{45}{\percent} & \qty{4}{\percent} & True \\
1039. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.8\) & \num{8.9e-05} & \qty{59}{\percent} & \qty{4}{\percent} & False \\
1040. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.8\) & \num{6.0e-01} & \qty{45}{\percent} & \qty{4}{\percent} & True \\
1041. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.6\) & \num{< 1e-5} & \qty{61}{\percent} & \qty{4}{\percent} & False \\
1042. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.6\) & \num{8.4e-04} & \qty{66}{\percent} & \qty{4}{\percent} & True \\
1043. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.5\) & \num{< 1e-5} & \qty{98}{\percent} & \qty{4}{\percent} & False \\
1044. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.5\) & \num{< 1e-5} & \qty{93}{\percent} & \qty{4}{\percent} & True \\
1045. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.6\) & \num{< 1e-5} & \qty{67}{\percent} & \qty{4}{\percent} & False \\
1046. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.6\) & \num{< 1e-5} & \qty{72}{\percent} & \qty{4}{\percent} & True \\
1047. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\lp{}-\mathtt{target}=\lp[\infty]\) & \num{< 1e-5} & \qty{59}{\percent} & \qty{4}{\percent} & False \\
1048. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\lp{}-\mathtt{target}=\lp[\infty]\) & \num{< 1e-5} & \qty{54}{\percent} & \qty{4}{\percent} & True \\
1049. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Dataset}=\nslkdd{}\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{4}{\percent} & False \\
1050. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Dataset}=\nslkdd{}\) & \num{< 1e-5} & \qty{70}{\percent} & \qty{4}{\percent} & True \\
1051. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Saliency Map}=\identitysmapfull{}\) & \num{< 1e-5} & \qty{56}{\percent} & \qty{4}{\percent} & False \\
1052. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Saliency Map}=\identitysmapfull{}\) & \num{< 1e-5} & \qty{51}{\percent} & \qty{4}{\percent} & True \\
1053. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\lp{}-\mathtt{target}=\lp[0]\) & \num{< 1e-5} & \qty{62}{\percent} & \qty{4}{\percent} & False \\
1054. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\lp{}-\mathtt{target}=\lp[0]\) & \num{< 1e-5} & \qty{67}{\percent} & \qty{4}{\percent} & True \\
1055. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Loss}=\cwlossfull{}\) & \num{< 1e-5} & \qty{56}{\percent} & \qty{4}{\percent} & False \\
1056. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Loss}=\cwlossfull{}\) & \num{< 1e-5} & \qty{52}{\percent} & \qty{4}{\percent} & True \\
1057. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Dataset}=\phishing{}\) & \num{< 2.2e-308} & \qty{92}{\percent} & \qty{4}{\percent} & False \\
1058. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Dataset}=\phishing{}\) & \num{< 2.2e-308} & \qty{87}{\percent} & \qty{4}{\percent} & True \\
1059. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Saliency Map}=\identitysmapfull{}\) & \num{< 2.2e-308} & \qty{93}{\percent} & \qty{4}{\percent} & False \\
1060. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Saliency Map}=\identitysmapfull{}\) & \num{< 2.2e-308} & \qty{89}{\percent} & \qty{4}{\percent} & True \\
1061. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.3\) & \num{< 1e-5} & \qty{61}{\percent} & \qty{4}{\percent} & False \\
1062. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.3\) & \num{< 1e-5} & \qty{66}{\percent} & \qty{4}{\percent} & True \\
1063. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.5\) & \num{< 1e-5} & \qty{60}{\percent} & \qty{4}{\percent} & False \\
1064. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.5\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{4}{\percent} & True \\
1065. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.4\) & \num{< 1e-5} & \qty{93}{\percent} & \qty{4}{\percent} & False \\
1066. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.4\) & \num{< 1e-5} & \qty{88}{\percent} & \qty{4}{\percent} & True \\
1067. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.0\) & \num{< 1e-5} & \qty{73}{\percent} & \qty{4}{\percent} & False \\
1068. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.0\) & \num{< 1e-5} & \qty{68}{\percent} & \qty{4}{\percent} & True \\
1069. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.8\) & \num{< 1e-5} & \qty{75}{\percent} & \qty{4}{\percent} & False \\
1070. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.8\) & \num{< 1e-5} & \qty{71}{\percent} & \qty{4}{\percent} & True \\
1071. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.6\) & \num{< 1e-5} & \qty{94}{\percent} & \qty{4}{\percent} & False \\
1072. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.6\) & \num{< 1e-5} & \qty{89}{\percent} & \qty{4}{\percent} & True \\
1073. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.7\) & \num{< 1e-5} & \qty{94}{\percent} & \qty{4}{\percent} & False \\
1074. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.7\) & \num{< 1e-5} & \qty{89}{\percent} & \qty{4}{\percent} & True \\
1075. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.9\) & \num{< 1e-5} & \qty{94}{\percent} & \qty{4}{\percent} & False \\
1076. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.9\) & \num{< 1e-5} & \qty{90}{\percent} & \qty{4}{\percent} & True \\
1077. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+2.0\) & \num{< 1e-5} & \qty{94}{\percent} & \qty{4}{\percent} & False \\
1078. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+2.0\) & \num{< 1e-5} & \qty{90}{\percent} & \qty{4}{\percent} & True \\
1079. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Dataset}=\unswnb{}\) & \num{< 1e-5} & \qty{70}{\percent} & \qty{4}{\percent} & False \\
1080. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Dataset}=\unswnb{}\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{4}{\percent} & True \\
1081. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.2\) & \num{1.5e-02} & \qty{63}{\percent} & \qty{4}{\percent} & False \\
1082. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.2\) & \num{1.4e-04} & \qty{67}{\percent} & \qty{4}{\percent} & True \\
1083. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.7\) & \num{< 1e-5} & \qty{76}{\percent} & \qty{4}{\percent} & False \\
1084. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.7\) & \num{< 1e-5} & \qty{72}{\percent} & \qty{4}{\percent} & True \\
1085. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.8\) & \num{< 1e-5} & \qty{78}{\percent} & \qty{4}{\percent} & False \\
1086. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.8\) & \num{< 1e-5} & \qty{82}{\percent} & \qty{4}{\percent} & True \\
1087. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.5\) & \num{< 1e-5} & \qty{66}{\percent} & \qty{4}{\percent} & False \\
1088. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.5\) & \num{< 1e-5} & \qty{71}{\percent} & \qty{4}{\percent} & True \\
1089. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.3\) & \num{< 1e-5} & \qty{72}{\percent} & \qty{4}{\percent} & False \\
1090. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.3\) & \num{< 1e-5} & \qty{68}{\percent} & \qty{4}{\percent} & True \\
1091. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.7\) & \num{< 1e-5} & \qty{61}{\percent} & \qty{4}{\percent} & False \\
1092. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.7\) & \num{9.1e-04} & \qty{66}{\percent} & \qty{4}{\percent} & True \\
1093. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.4\) & \num{< 1e-5} & \qty{93}{\percent} & \qty{4}{\percent} & False \\
1094. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.4\) & \num{< 1e-5} & \qty{88}{\percent} & \qty{4}{\percent} & True \\
1095. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.6\) & \num{< 1e-5} & \qty{60}{\percent} & \qty{4}{\percent} & False \\
1096. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.6\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{4}{\percent} & True \\
1097. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.3\) & \num{< 1e-5} & \qty{92}{\percent} & \qty{4}{\percent} & False \\
1098. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.3\) & \num{< 1e-5} & \qty{88}{\percent} & \qty{4}{\percent} & True \\
1099. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.4\) & \num{< 1e-5} & \qty{92}{\percent} & \qty{4}{\percent} & False \\
1100. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.4\) & \num{< 1e-5} & \qty{88}{\percent} & \qty{4}{\percent} & True \\
1101. & \adam{} & is better than &  \sgd{} & when & \(\rr{}=\textit{Enabled}\) & \num{< 2.2e-308} & \qty{69}{\percent} & \qty{4}{\percent} & False \\
1102. & \adam{} & is better than &  \sgd{} & when & \(\rr{}=\textit{Enabled}\) & \num{< 2.2e-308} & \qty{65}{\percent} & \qty{4}{\percent} & True \\
1103. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\cov{}=\textit{Enabled}\) & \num{< 2.2e-308} & \qty{70}{\percent} & \qty{4}{\percent} & False \\
1104. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\cov{}=\textit{Enabled}\) & \num{< 2.2e-308} & \qty{65}{\percent} & \qty{4}{\percent} & True \\
1105. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.5\) & \num{< 1e-5} & \qty{76}{\percent} & \qty{4}{\percent} & False \\
1106. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.5\) & \num{< 1e-5} & \qty{72}{\percent} & \qty{4}{\percent} & True \\
1107. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.2\) & \num{< 1e-5} & \qty{92}{\percent} & \qty{4}{\percent} & False \\
1108. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.2\) & \num{< 1e-5} & \qty{88}{\percent} & \qty{4}{\percent} & True \\
1109. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.5\) & \num{< 1e-5} & \qty{92}{\percent} & \qty{4}{\percent} & False \\
1110. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.5\) & \num{< 1e-5} & \qty{88}{\percent} & \qty{4}{\percent} & True \\
1111. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.8\) & \num{< 1e-5} & \qty{94}{\percent} & \qty{4}{\percent} & False \\
1112. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.8\) & \num{< 1e-5} & \qty{89}{\percent} & \qty{4}{\percent} & True \\
1113. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.9\) & \num{< 1e-5} & \qty{60}{\percent} & \qty{4}{\percent} & False \\
1114. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.9\) & \num{6.4e-01} & \qty{55}{\percent} & \qty{4}{\percent} & True \\
1115. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.0\) & \num{< 1e-5} & \qty{60}{\percent} & \qty{4}{\percent} & False \\
1116. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.0\) & \num{7.8e-01} & \qty{55}{\percent} & \qty{4}{\percent} & True \\
1117. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.1\) & \num{< 1e-5} & \qty{60}{\percent} & \qty{4}{\percent} & False \\
1118. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.1\) & \num{9.0e-01} & \qty{55}{\percent} & \qty{4}{\percent} & True \\
1119. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.5\) & \num{3.1e-05} & \qty{59}{\percent} & \qty{4}{\percent} & False \\
1120. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.5\) & \num{7.6e-01} & \qty{44}{\percent} & \qty{4}{\percent} & True \\
1121. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.7\) & \num{< 1e-5} & \qty{61}{\percent} & \qty{4}{\percent} & False \\
1122. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.7\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{4}{\percent} & True \\
1123. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.8\) & \num{< 1e-5} & \qty{61}{\percent} & \qty{4}{\percent} & False \\
1124. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.8\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{4}{\percent} & True \\
1125. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[0]+2.0\) & \num{< 1e-5} & \qty{61}{\percent} & \qty{4}{\percent} & False \\
1126. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[0]+2.0\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{4}{\percent} & True \\
1127. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.4\) & \num{< 1e-5} & \qty{66}{\percent} & \qty{4}{\percent} & False \\
1128. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.4\) & \num{< 1e-5} & \qty{62}{\percent} & \qty{4}{\percent} & True \\
1129. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.5\) & \num{< 1e-5} & \qty{93}{\percent} & \qty{4}{\percent} & False \\
1130. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.5\) & \num{< 1e-5} & \qty{89}{\percent} & \qty{4}{\percent} & True \\
1131. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.9\) & \num{5.2e-02} & \qty{54}{\percent} & \qty{4}{\percent} & False \\
1132. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.9\) & \num{1.3e-01} & \qty{50}{\percent} & \qty{4}{\percent} & True \\
1133. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.6\) & \num{< 1e-5} & \qty{76}{\percent} & \qty{4}{\percent} & False \\
1134. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.6\) & \num{< 1e-5} & \qty{71}{\percent} & \qty{4}{\percent} & True \\
1135. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.7\) & \num{< 1e-5} & \qty{75}{\percent} & \qty{4}{\percent} & False \\
1136. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.7\) & \num{< 1e-5} & \qty{71}{\percent} & \qty{4}{\percent} & True \\
1137. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.7\) & \num{< 1e-5} & \qty{98}{\percent} & \qty{4}{\percent} & False \\
1138. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.7\) & \num{< 1e-5} & \qty{94}{\percent} & \qty{4}{\percent} & True \\
1139. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.8\) & \num{< 1e-5} & \qty{63}{\percent} & \qty{4}{\percent} & False \\
1140. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.8\) & \num{< 1e-5} & \qty{59}{\percent} & \qty{4}{\percent} & True \\
1141. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.8\) & \num{< 1e-5} & \qty{98}{\percent} & \qty{4}{\percent} & False \\
1142. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.8\) & \num{< 1e-5} & \qty{94}{\percent} & \qty{4}{\percent} & True \\
1143. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.9\) & \num{< 1e-5} & \qty{98}{\percent} & \qty{4}{\percent} & False \\
1144. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.9\) & \num{< 1e-5} & \qty{94}{\percent} & \qty{4}{\percent} & True \\
1145. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.1\) & \num{< 1e-5} & \qty{78}{\percent} & \qty{4}{\percent} & False \\
1146. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.1\) & \num{< 1e-5} & \qty{83}{\percent} & \qty{4}{\percent} & True \\
1147. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.4\) & \num{< 1e-5} & \qty{61}{\percent} & \qty{4}{\percent} & False \\
1148. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.4\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{4}{\percent} & True \\
1149. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.5\) & \num{< 1e-5} & \qty{76}{\percent} & \qty{4}{\percent} & False \\
1150. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.5\) & \num{< 1e-5} & \qty{72}{\percent} & \qty{4}{\percent} & True \\
1151. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.9\) & \num{< 1e-5} & \qty{61}{\percent} & \qty{4}{\percent} & False \\
1152. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.9\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{4}{\percent} & True \\
1153. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.9\) & \num{< 1e-5} & \qty{64}{\percent} & \qty{4}{\percent} & False \\
1154. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.9\) & \num{< 1e-5} & \qty{60}{\percent} & \qty{4}{\percent} & True \\
1155. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Saliency Map}=\jsmasmapfull{}\) & \num{< 1e-5} & \qty{54}{\percent} & \qty{4}{\percent} & False \\
1156. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Saliency Map}=\jsmasmapfull{}\) & \num{< 1e-5} & \qty{58}{\percent} & \qty{4}{\percent} & True \\
1157. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.6\) & \num{< 1e-5} & \qty{74}{\percent} & \qty{4}{\percent} & False \\
1158. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.6\) & \num{< 1e-5} & \qty{70}{\percent} & \qty{4}{\percent} & True \\
1159. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.5\) & \num{< 1e-5} & \qty{60}{\percent} & \qty{4}{\percent} & False \\
1160. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.5\) & \num{< 1e-5} & \qty{64}{\percent} & \qty{4}{\percent} & True \\
1161. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.8\) & \num{1.1e-04} & \qty{64}{\percent} & \qty{4}{\percent} & False \\
1162. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.8\) & \num{< 1e-5} & \qty{60}{\percent} & \qty{4}{\percent} & True \\
1163. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.2\) & \num{< 1e-5} & \qty{72}{\percent} & \qty{4}{\percent} & False \\
1164. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.2\) & \num{< 1e-5} & \qty{68}{\percent} & \qty{4}{\percent} & True \\
1165. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.4\) & \num{< 1e-5} & \qty{72}{\percent} & \qty{4}{\percent} & False \\
1166. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.4\) & \num{< 1e-5} & \qty{68}{\percent} & \qty{4}{\percent} & True \\
1167. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.2\) & \num{< 1e-5} & \qty{60}{\percent} & \qty{4}{\percent} & False \\
1168. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.2\) & \num{9.9e-01} & \qty{44}{\percent} & \qty{4}{\percent} & True \\
1169. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.4\) & \num{2.2e-05} & \qty{59}{\percent} & \qty{4}{\percent} & False \\
1170. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.4\) & \num{8.4e-01} & \qty{44}{\percent} & \qty{4}{\percent} & True \\
1171. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.8\) & \num{< 1e-5} & \qty{62}{\percent} & \qty{4}{\percent} & False \\
1172. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.8\) & \num{9.3e-04} & \qty{66}{\percent} & \qty{4}{\percent} & True \\
1173. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Saliency Map}=\dfsmapfull{}\) & \num{< 1e-5} & \qty{61}{\percent} & \qty{4}{\percent} & False \\
1174. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Saliency Map}=\dfsmapfull{}\) & \num{< 1e-5} & \qty{57}{\percent} & \qty{4}{\percent} & True \\
1175. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.0\) & \num{< 1e-5} & \qty{64}{\percent} & \qty{4}{\percent} & False \\
1176. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.0\) & \num{< 1e-5} & \qty{60}{\percent} & \qty{4}{\percent} & True \\
1177. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.1\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{4}{\percent} & False \\
1178. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.1\) & \num{< 1e-5} & \qty{60}{\percent} & \qty{4}{\percent} & True \\
1179. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Saliency Map}=\jsmasmapfull{}\) & \num{< 1e-5} & \qty{51}{\percent} & \qty{4}{\percent} & False \\
1180. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Saliency Map}=\jsmasmapfull{}\) & \num{< 1e-5} & \qty{56}{\percent} & \qty{4}{\percent} & True \\
1181. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Saliency Map}=\dfsmapfull{}\) & \num{< 2.2e-308} & \qty{96}{\percent} & \qty{3}{\percent} & False \\
1182. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Saliency Map}=\dfsmapfull{}\) & \num{< 2.2e-308} & \qty{93}{\percent} & \qty{3}{\percent} & True \\
1183. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.1\) & \num{9.2e-02} & \qty{54}{\percent} & \qty{3}{\percent} & False \\
1184. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.1\) & \num{9.6e-02} & \qty{50}{\percent} & \qty{3}{\percent} & True \\
1185. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.6\) & \num{< 1e-5} & \qty{92}{\percent} & \qty{3}{\percent} & False \\
1186. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.6\) & \num{< 1e-5} & \qty{88}{\percent} & \qty{3}{\percent} & True \\
1187. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.7\) & \num{< 1e-5} & \qty{62}{\percent} & \qty{3}{\percent} & False \\
1188. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.7\) & \num{< 1e-5} & \qty{59}{\percent} & \qty{3}{\percent} & True \\
1189. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.5\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{3}{\percent} & False \\
1190. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.5\) & \num{< 1e-5} & \qty{61}{\percent} & \qty{3}{\percent} & True \\
1191. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.8\) & \num{< 1e-5} & \qty{59}{\percent} & \qty{3}{\percent} & False \\
1192. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.8\) & \num{4.8e-01} & \qty{55}{\percent} & \qty{3}{\percent} & True \\
1193. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.3\) & \num{1.4e-05} & \qty{59}{\percent} & \qty{3}{\percent} & False \\
1194. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.3\) & \num{9.2e-01} & \qty{44}{\percent} & \qty{3}{\percent} & True \\
1195. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.0\) & \num{7.6e-02} & \qty{53}{\percent} & \qty{3}{\percent} & False \\
1196. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.0\) & \num{1.1e-01} & \qty{50}{\percent} & \qty{3}{\percent} & True \\
1197. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.9\) & \num{< 1e-5} & \qty{62}{\percent} & \qty{3}{\percent} & False \\
1198. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.9\) & \num{9.6e-04} & \qty{66}{\percent} & \qty{3}{\percent} & True \\
1199. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.9\) & \num{< 1e-5} & \qty{78}{\percent} & \qty{3}{\percent} & False \\
1200. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+1.9\) & \num{< 1e-5} & \qty{82}{\percent} & \qty{3}{\percent} & True \\
1201. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.3\) & \num{< 1e-5} & \qty{75}{\percent} & \qty{3}{\percent} & False \\
1202. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.3\) & \num{< 1e-5} & \qty{72}{\percent} & \qty{3}{\percent} & True \\
1203. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.4\) & \num{< 1e-5} & \qty{76}{\percent} & \qty{3}{\percent} & False \\
1204. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.4\) & \num{< 1e-5} & \qty{72}{\percent} & \qty{3}{\percent} & True \\
1205. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.7\) & \num{< 1e-5} & \qty{68}{\percent} & \qty{3}{\percent} & False \\
1206. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.7\) & \num{< 1e-5} & \qty{72}{\percent} & \qty{3}{\percent} & True \\
1207. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.0\) & \num{< 1e-5} & \qty{98}{\percent} & \qty{3}{\percent} & False \\
1208. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.0\) & \num{< 1e-5} & \qty{94}{\percent} & \qty{3}{\percent} & True \\
1209. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.1\) & \num{< 1e-5} & \qty{93}{\percent} & \qty{3}{\percent} & False \\
1210. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.1\) & \num{< 1e-5} & \qty{89}{\percent} & \qty{3}{\percent} & True \\
1211. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.1\) & \num{< 1e-5} & \qty{98}{\percent} & \qty{3}{\percent} & False \\
1212. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.1\) & \num{< 1e-5} & \qty{94}{\percent} & \qty{3}{\percent} & True \\
1213. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.2\) & \num{< 1e-5} & \qty{93}{\percent} & \qty{3}{\percent} & False \\
1214. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.2\) & \num{< 1e-5} & \qty{89}{\percent} & \qty{3}{\percent} & True \\
1215. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.2\) & \num{< 1e-5} & \qty{98}{\percent} & \qty{3}{\percent} & False \\
1216. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.2\) & \num{< 1e-5} & \qty{94}{\percent} & \qty{3}{\percent} & True \\
1217. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.3\) & \num{< 1e-5} & \qty{93}{\percent} & \qty{3}{\percent} & False \\
1218. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.3\) & \num{< 1e-5} & \qty{89}{\percent} & \qty{3}{\percent} & True \\
1219. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.3\) & \num{< 1e-5} & \qty{98}{\percent} & \qty{3}{\percent} & False \\
1220. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.3\) & \num{< 1e-5} & \qty{94}{\percent} & \qty{3}{\percent} & True \\
1221. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.4\) & \num{< 1e-5} & \qty{98}{\percent} & \qty{3}{\percent} & False \\
1222. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.4\) & \num{< 1e-5} & \qty{94}{\percent} & \qty{3}{\percent} & True \\
1223. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.7\) & \num{< 1e-5} & \qty{73}{\percent} & \qty{3}{\percent} & False \\
1224. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.7\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{3}{\percent} & True \\
1225. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Loss}=\crossentropyfull{}\) & \num{< 1e-5} & \qty{59}{\percent} & \qty{3}{\percent} & False \\
1226. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Loss}=\crossentropyfull{}\) & \num{< 1e-5} & \qty{55}{\percent} & \qty{3}{\percent} & True \\
1227. & \lp[\infty] & is better than &  \lp[0] & when & \(\rr{}=\textit{Enabled}\) & \num{< 2.2e-308} & \qty{80}{\percent} & \qty{3}{\percent} & False \\
1228. & \lp[\infty] & is better than &  \lp[0] & when & \(\rr{}=\textit{Enabled}\) & \num{< 2.2e-308} & \qty{84}{\percent} & \qty{3}{\percent} & True \\
1229. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.2\) & \num{< 1e-5} & \qty{64}{\percent} & \qty{3}{\percent} & False \\
1230. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.2\) & \num{< 1e-5} & \qty{60}{\percent} & \qty{3}{\percent} & True \\
1231. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.3\) & \num{< 1e-5} & \qty{64}{\percent} & \qty{3}{\percent} & False \\
1232. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.3\) & \num{< 1e-5} & \qty{61}{\percent} & \qty{3}{\percent} & True \\
1233. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.4\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{3}{\percent} & False \\
1234. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.4\) & \num{< 1e-5} & \qty{61}{\percent} & \qty{3}{\percent} & True \\
1235. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.6\) & \num{< 1e-5} & \qty{93}{\percent} & \qty{3}{\percent} & False \\
1236. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.6\) & \num{< 1e-5} & \qty{90}{\percent} & \qty{3}{\percent} & True \\
1237. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.8\) & \num{< 1e-5} & \qty{93}{\percent} & \qty{3}{\percent} & False \\
1238. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.8\) & \num{< 1e-5} & \qty{90}{\percent} & \qty{3}{\percent} & True \\
1239. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.0\) & \num{< 1e-5} & \qty{78}{\percent} & \qty{3}{\percent} & False \\
1240. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.0\) & \num{< 1e-5} & \qty{81}{\percent} & \qty{3}{\percent} & True \\
1241. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.5\) & \num{< 1e-5} & \qty{98}{\percent} & \qty{3}{\percent} & False \\
1242. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.5\) & \num{< 1e-5} & \qty{95}{\percent} & \qty{3}{\percent} & True \\
1243. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.2\) & \num{2.3e-02} & \qty{63}{\percent} & \qty{3}{\percent} & False \\
1244. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.2\) & \num{2.1e-01} & \qty{60}{\percent} & \qty{3}{\percent} & True \\
1245. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.5\) & \num{< 1e-5} & \qty{73}{\percent} & \qty{3}{\percent} & False \\
1246. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.5\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{3}{\percent} & True \\
1247. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.6\) & \num{< 1e-5} & \qty{76}{\percent} & \qty{3}{\percent} & False \\
1248. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.6\) & \num{< 1e-5} & \qty{73}{\percent} & \qty{3}{\percent} & True \\
1249. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.9\) & \num{1.9e-05} & \qty{65}{\percent} & \qty{3}{\percent} & False \\
1250. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.9\) & \num{< 1e-5} & \qty{61}{\percent} & \qty{3}{\percent} & True \\
1251. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.6\) & \num{< 1e-5} & \qty{73}{\percent} & \qty{3}{\percent} & False \\
1252. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.6\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{3}{\percent} & True \\
1253. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Loss}=\crossentropyfull{}\) & \num{< 2.2e-308} & \qty{95}{\percent} & \qty{3}{\percent} & False \\
1254. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Loss}=\crossentropyfull{}\) & \num{< 2.2e-308} & \qty{91}{\percent} & \qty{3}{\percent} & True \\
1255. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.0\) & \num{< 1e-5} & \qty{55}{\percent} & \qty{3}{\percent} & False \\
1256. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.0\) & \num{6.1e-03} & \qty{52}{\percent} & \qty{3}{\percent} & True \\
1257. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Loss}=\identitylossfull{}\) & \num{< 2.2e-308} & \qty{95}{\percent} & \qty{3}{\percent} & False \\
1258. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Loss}=\identitylossfull{}\) & \num{< 2.2e-308} & \qty{91}{\percent} & \qty{3}{\percent} & True \\
1259. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\rr{}=\textit{Enabled}\) & \num{< 1e-5} & \qty{53}{\percent} & \qty{3}{\percent} & False \\
1260. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\rr{}=\textit{Enabled}\) & \num{< 1e-5} & \qty{50}{\percent} & \qty{3}{\percent} & True \\
1261. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.1\) & \num{9.0e-02} & \qty{63}{\percent} & \qty{3}{\percent} & False \\
1262. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.1\) & \num{4.4e-01} & \qty{60}{\percent} & \qty{3}{\percent} & True \\
1263. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+2.0\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{3}{\percent} & False \\
1264. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+2.0\) & \num{4.0e-04} & \qty{66}{\percent} & \qty{3}{\percent} & True \\
1265. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+2.0\) & \num{< 1e-5} & \qty{79}{\percent} & \qty{3}{\percent} & False \\
1266. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[2]+2.0\) & \num{< 1e-5} & \qty{83}{\percent} & \qty{3}{\percent} & True \\
1267. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.3\) & \num{< 1e-5} & \qty{73}{\percent} & \qty{3}{\percent} & False \\
1268. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.3\) & \num{< 1e-5} & \qty{70}{\percent} & \qty{3}{\percent} & True \\
1269. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.4\) & \num{3.2e-05} & \qty{60}{\percent} & \qty{3}{\percent} & False \\
1270. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.4\) & \num{< 1e-5} & \qty{63}{\percent} & \qty{3}{\percent} & True \\
1271. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.7\) & \num{7.1e-04} & \qty{63}{\percent} & \qty{3}{\percent} & False \\
1272. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.7\) & \num{< 1e-5} & \qty{60}{\percent} & \qty{3}{\percent} & True \\
1273. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.6\) & \num{< 1e-5} & \qty{98}{\percent} & \qty{3}{\percent} & False \\
1274. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.6\) & \num{< 1e-5} & \qty{95}{\percent} & \qty{3}{\percent} & True \\
1275. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.7\) & \num{< 1e-5} & \qty{98}{\percent} & \qty{3}{\percent} & False \\
1276. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.7\) & \num{< 1e-5} & \qty{95}{\percent} & \qty{3}{\percent} & True \\
1277. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.8\) & \num{< 1e-5} & \qty{98}{\percent} & \qty{3}{\percent} & False \\
1278. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.8\) & \num{< 1e-5} & \qty{95}{\percent} & \qty{3}{\percent} & True \\
1279. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\rr{}=\textit{Disabled}\) & \num{< 2.2e-308} & \qty{95}{\percent} & \qty{3}{\percent} & False \\
1280. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\rr{}=\textit{Disabled}\) & \num{< 2.2e-308} & \qty{92}{\percent} & \qty{3}{\percent} & True \\
1281. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\cov{}=\textit{Disabled}\) & \num{< 1e-5} & \qty{51}{\percent} & \qty{3}{\percent} & False \\
1282. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\cov{}=\textit{Disabled}\) & \num{< 1e-5} & \qty{47}{\percent} & \qty{3}{\percent} & True \\
1283. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\cov{}=\textit{Disabled}\) & \num{< 1e-5} & \qty{66}{\percent} & \qty{3}{\percent} & False \\
1284. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\cov{}=\textit{Disabled}\) & \num{< 1e-5} & \qty{63}{\percent} & \qty{3}{\percent} & True \\
1285. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.7\) & \num{< 1e-5} & \qty{93}{\percent} & \qty{3}{\percent} & False \\
1286. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.7\) & \num{< 1e-5} & \qty{90}{\percent} & \qty{3}{\percent} & True \\
1287. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.7\) & \num{< 1e-5} & \qty{92}{\percent} & \qty{3}{\percent} & False \\
1288. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.7\) & \num{< 1e-5} & \qty{89}{\percent} & \qty{3}{\percent} & True \\
1289. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.8\) & \num{< 1e-5} & \qty{92}{\percent} & \qty{3}{\percent} & False \\
1290. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.8\) & \num{< 1e-5} & \qty{89}{\percent} & \qty{3}{\percent} & True \\
1291. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Solver}=\sgd{}\) & \num{< 2.2e-308} & \qty{90}{\percent} & \qty{3}{\percent} & False \\
1292. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Solver}=\sgd{}\) & \num{< 2.2e-308} & \qty{87}{\percent} & \qty{3}{\percent} & True \\
1293. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Dataset}=\fmnist{}\) & \num{< 1e-5} & \qty{60}{\percent} & \qty{3}{\percent} & False \\
1294. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Dataset}=\fmnist{}\) & \num{< 1e-5} & \qty{63}{\percent} & \qty{3}{\percent} & True \\
1295. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.0\) & \num{1.4e-01} & \qty{44}{\percent} & \qty{3}{\percent} & False \\
1296. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.0\) & \num{2.0e-01} & \qty{47}{\percent} & \qty{3}{\percent} & True \\
1297. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.8\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{3}{\percent} & False \\
1298. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.8\) & \num{3.1e-04} & \qty{66}{\percent} & \qty{3}{\percent} & True \\
1299. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.9\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{3}{\percent} & False \\
1300. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.9\) & \num{3.7e-04} & \qty{66}{\percent} & \qty{3}{\percent} & True \\
1301. & \jsmasmapfull{} & is better than &  \identitysmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.2\) & \num{3.2e-01} & \qty{46}{\percent} & \qty{3}{\percent} & False \\
1302. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.2\) & \num{4.3e-01} & \qty{56}{\percent} & \qty{3}{\percent} & True \\
1303. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.2\) & \num{1.1e-01} & \qty{54}{\percent} & \qty{3}{\percent} & False \\
1304. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.2\) & \num{7.7e-02} & \qty{51}{\percent} & \qty{3}{\percent} & True \\
1305. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.3\) & \num{1.3e-01} & \qty{53}{\percent} & \qty{3}{\percent} & False \\
1306. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.3\) & \num{6.3e-02} & \qty{50}{\percent} & \qty{3}{\percent} & True \\
1307. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.5\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{3}{\percent} & False \\
1308. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.5\) & \num{< 1e-5} & \qty{72}{\percent} & \qty{3}{\percent} & True \\
1309. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.6\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{3}{\percent} & False \\
1310. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.6\) & \num{< 1e-5} & \qty{72}{\percent} & \qty{3}{\percent} & True \\
1311. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.7\) & \num{< 1e-5} & \qty{70}{\percent} & \qty{3}{\percent} & False \\
1312. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.7\) & \num{< 1e-5} & \qty{73}{\percent} & \qty{3}{\percent} & True \\
1313. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.8\) & \num{< 1e-5} & \qty{70}{\percent} & \qty{3}{\percent} & False \\
1314. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.8\) & \num{< 1e-5} & \qty{73}{\percent} & \qty{3}{\percent} & True \\
1315. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.4\) & \num{< 1e-5} & \qty{77}{\percent} & \qty{3}{\percent} & False \\
1316. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.4\) & \num{< 1e-5} & \qty{74}{\percent} & \qty{3}{\percent} & True \\
1317. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.5\) & \num{< 1e-5} & \qty{77}{\percent} & \qty{3}{\percent} & False \\
1318. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.5\) & \num{< 1e-5} & \qty{74}{\percent} & \qty{3}{\percent} & True \\
1319. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.9\) & \num{< 1e-5} & \qty{78}{\percent} & \qty{3}{\percent} & False \\
1320. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.9\) & \num{< 1e-5} & \qty{81}{\percent} & \qty{3}{\percent} & True \\
1321. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.0\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{3}{\percent} & False \\
1322. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.0\) & \num{< 1e-5} & \qty{62}{\percent} & \qty{3}{\percent} & True \\
1323. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.1\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{3}{\percent} & False \\
1324. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.1\) & \num{< 1e-5} & \qty{62}{\percent} & \qty{3}{\percent} & True \\
1325. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.9\) & \num{< 1e-5} & \qty{93}{\percent} & \qty{2}{\percent} & False \\
1326. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.9\) & \num{< 1e-5} & \qty{90}{\percent} & \qty{2}{\percent} & True \\
1327. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.9\) & \num{< 1e-5} & \qty{92}{\percent} & \qty{2}{\percent} & False \\
1328. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.9\) & \num{< 1e-5} & \qty{90}{\percent} & \qty{2}{\percent} & True \\
1329. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.0\) & \num{< 1e-5} & \qty{92}{\percent} & \qty{2}{\percent} & False \\
1330. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.0\) & \num{< 1e-5} & \qty{90}{\percent} & \qty{2}{\percent} & True \\
1331. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Loss}=\identitylossfull{}\) & \num{< 2.2e-308} & \qty{80}{\percent} & \qty{2}{\percent} & False \\
1332. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Loss}=\identitylossfull{}\) & \num{< 2.2e-308} & \qty{83}{\percent} & \qty{2}{\percent} & True \\
1333. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Solver}=\sgd{}\) & \num{< 1e-5} & \qty{56}{\percent} & \qty{2}{\percent} & False \\
1334. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Solver}=\sgd{}\) & \num{< 1e-5} & \qty{58}{\percent} & \qty{2}{\percent} & True \\
1335. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\lp{}-\mathtt{target}=\lp[2]\) & \num{< 1e-5} & \qty{63}{\percent} & \qty{2}{\percent} & False \\
1336. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\lp{}-\mathtt{target}=\lp[2]\) & \num{< 1e-5} & \qty{66}{\percent} & \qty{2}{\percent} & True \\
1337. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\rr{}=\textit{Disabled}\) & \num{< 1e-5} & \qty{61}{\percent} & \qty{2}{\percent} & False \\
1338. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\rr{}=\textit{Disabled}\) & \num{< 1e-5} & \qty{64}{\percent} & \qty{2}{\percent} & True \\
1339. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Solver}=\adam{}\) & \num{< 2.2e-308} & \qty{99}{\percent} & \qty{2}{\percent} & False \\
1340. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Solver}=\adam{}\) & \num{< 2.2e-308} & \qty{96}{\percent} & \qty{2}{\percent} & True \\
1341. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.2\) & \num{< 1e-5} & \qty{71}{\percent} & \qty{2}{\percent} & False \\
1342. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.2\) & \num{1.9e-05} & \qty{68}{\percent} & \qty{2}{\percent} & True \\
1343. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.3\) & \num{2.6e-02} & \qty{62}{\percent} & \qty{2}{\percent} & False \\
1344. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.3\) & \num{9.7e-04} & \qty{65}{\percent} & \qty{2}{\percent} & True \\
1345. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.5\) & \num{3.9e-04} & \qty{64}{\percent} & \qty{2}{\percent} & False \\
1346. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.5\) & \num{1.8e-02} & \qty{61}{\percent} & \qty{2}{\percent} & True \\
1347. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.7\) & \num{< 1e-5} & \qty{68}{\percent} & \qty{2}{\percent} & False \\
1348. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.7\) & \num{2.6e-04} & \qty{66}{\percent} & \qty{2}{\percent} & True \\
1349. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.0\) & \num{< 1e-5} & \qty{67}{\percent} & \qty{2}{\percent} & False \\
1350. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.0\) & \num{< 1e-5} & \qty{70}{\percent} & \qty{2}{\percent} & True \\
1351. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.5\) & \num{1.4e-01} & \qty{53}{\percent} & \qty{2}{\percent} & False \\
1352. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.5\) & \num{4.8e-02} & \qty{50}{\percent} & \qty{2}{\percent} & True \\
1353. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.9\) & \num{< 1e-5} & \qty{70}{\percent} & \qty{2}{\percent} & False \\
1354. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.9\) & \num{< 1e-5} & \qty{73}{\percent} & \qty{2}{\percent} & True \\
1355. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+2.0\) & \num{< 1e-5} & \qty{63}{\percent} & \qty{2}{\percent} & False \\
1356. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+2.0\) & \num{1.0e-03} & \qty{66}{\percent} & \qty{2}{\percent} & True \\
1357. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.0\) & \num{< 1e-5} & \qty{63}{\percent} & \qty{2}{\percent} & False \\
1358. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.0\) & \num{< 1e-5} & \qty{61}{\percent} & \qty{2}{\percent} & True \\
1359. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.2\) & \num{< 1e-5} & \qty{75}{\percent} & \qty{2}{\percent} & False \\
1360. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.2\) & \num{< 1e-5} & \qty{72}{\percent} & \qty{2}{\percent} & True \\
1361. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.4\) & \num{< 1e-5} & \qty{72}{\percent} & \qty{2}{\percent} & False \\
1362. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.4\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{2}{\percent} & True \\
1363. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.5\) & \num{< 1e-5} & \qty{72}{\percent} & \qty{2}{\percent} & False \\
1364. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.5\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{2}{\percent} & True \\
1365. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.6\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{2}{\percent} & False \\
1366. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.6\) & \num{< 1e-5} & \qty{62}{\percent} & \qty{2}{\percent} & True \\
1367. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.9\) & \num{< 1e-5} & \qty{98}{\percent} & \qty{2}{\percent} & False \\
1368. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.9\) & \num{< 1e-5} & \qty{95}{\percent} & \qty{2}{\percent} & True \\
1369. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+2.0\) & \num{< 1e-5} & \qty{98}{\percent} & \qty{2}{\percent} & False \\
1370. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+2.0\) & \num{< 1e-5} & \qty{95}{\percent} & \qty{2}{\percent} & True \\
1371. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.9\) & \num{< 1e-5} & \qty{67}{\percent} & \qty{2}{\percent} & False \\
1372. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.9\) & \num{< 1e-5} & \qty{70}{\percent} & \qty{2}{\percent} & True \\
1373. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Solver}=\adam{}\) & \num{< 2.2e-308} & \qty{75}{\percent} & \qty{2}{\percent} & False \\
1374. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Solver}=\adam{}\) & \num{< 2.2e-308} & \qty{78}{\percent} & \qty{2}{\percent} & True \\
1375. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\rr{}=\textit{Enabled}\) & \num{< 2.2e-308} & \qty{94}{\percent} & \qty{2}{\percent} & False \\
1376. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\rr{}=\textit{Enabled}\) & \num{< 2.2e-308} & \qty{91}{\percent} & \qty{2}{\percent} & True \\
1377. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.0\) & \num{< 1e-5} & \qty{92}{\percent} & \qty{2}{\percent} & False \\
1378. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.0\) & \num{< 1e-5} & \qty{90}{\percent} & \qty{2}{\percent} & True \\
1379. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Loss}=\identitylossfull{}\) & \num{< 1e-5} & \qty{54}{\percent} & \qty{2}{\percent} & False \\
1380. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Loss}=\identitylossfull{}\) & \num{< 1e-5} & \qty{56}{\percent} & \qty{2}{\percent} & True \\
1381. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\lp{}-\mathtt{target}=\lp[\infty]\) & \num{< 1e-5} & \qty{56}{\percent} & \qty{2}{\percent} & False \\
1382. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\lp{}-\mathtt{target}=\lp[\infty]\) & \num{2.8e-03} & \qty{54}{\percent} & \qty{2}{\percent} & True \\
1383. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.3\) & \num{5.8e-03} & \qty{63}{\percent} & \qty{2}{\percent} & False \\
1384. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.3\) & \num{8.9e-02} & \qty{60}{\percent} & \qty{2}{\percent} & True \\
1385. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.7\) & \num{< 1e-5} & \qty{66}{\percent} & \qty{2}{\percent} & False \\
1386. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.7\) & \num{< 1e-5} & \qty{68}{\percent} & \qty{2}{\percent} & True \\
1387. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.8\) & \num{< 1e-5} & \qty{66}{\percent} & \qty{2}{\percent} & False \\
1388. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.8\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{2}{\percent} & True \\
1389. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.2\) & \num{< 1e-5} & \qty{68}{\percent} & \qty{2}{\percent} & False \\
1390. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.2\) & \num{< 1e-5} & \qty{71}{\percent} & \qty{2}{\percent} & True \\
1391. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+2.0\) & \num{< 1e-5} & \qty{71}{\percent} & \qty{2}{\percent} & False \\
1392. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+2.0\) & \num{< 1e-5} & \qty{73}{\percent} & \qty{2}{\percent} & True \\
1393. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.5\) & \num{< 1e-5} & \qty{77}{\percent} & \qty{2}{\percent} & False \\
1394. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.5\) & \num{< 1e-5} & \qty{75}{\percent} & \qty{2}{\percent} & True \\
1395. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.8\) & \num{< 1e-5} & \qty{70}{\percent} & \qty{2}{\percent} & False \\
1396. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.8\) & \num{< 1e-5} & \qty{72}{\percent} & \qty{2}{\percent} & True \\
1397. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.2\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{2}{\percent} & False \\
1398. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.2\) & \num{< 1e-5} & \qty{63}{\percent} & \qty{2}{\percent} & True \\
1399. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.2\) & \num{< 1e-5} & \qty{72}{\percent} & \qty{2}{\percent} & False \\
1400. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.2\) & \num{< 1e-5} & \qty{70}{\percent} & \qty{2}{\percent} & True \\
1401. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.4\) & \num{1.4e-03} & \qty{63}{\percent} & \qty{2}{\percent} & False \\
1402. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.4\) & \num{4.0e-02} & \qty{61}{\percent} & \qty{2}{\percent} & True \\
1403. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.4\) & \num{< 1e-5} & \qty{75}{\percent} & \qty{2}{\percent} & False \\
1404. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.4\) & \num{< 1e-5} & \qty{73}{\percent} & \qty{2}{\percent} & True \\
1405. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.8\) & \num{< 1e-5} & \qty{77}{\percent} & \qty{2}{\percent} & False \\
1406. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.8\) & \num{< 1e-5} & \qty{80}{\percent} & \qty{2}{\percent} & True \\
1407. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\lp{}-\mathtt{target}=\lp[\infty]\) & \num{< 2.2e-308} & \qty{99}{\percent} & \qty{2}{\percent} & False \\
1408. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\lp{}-\mathtt{target}=\lp[\infty]\) & \num{< 2.2e-308} & \qty{96}{\percent} & \qty{2}{\percent} & True \\
1409. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.7\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{2}{\percent} & False \\
1410. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.7\) & \num{< 1e-5} & \qty{62}{\percent} & \qty{2}{\percent} & True \\
1411. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\rr{}=\textit{Enabled}\) & \num{< 1e-5} & \qty{67}{\percent} & \qty{2}{\percent} & False \\
1412. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\rr{}=\textit{Enabled}\) & \num{< 2.2e-308} & \qty{65}{\percent} & \qty{2}{\percent} & True \\
1413. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Saliency Map}=\identitysmapfull{}\) & \num{< 2.2e-308} & \qty{74}{\percent} & \qty{2}{\percent} & False \\
1414. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Saliency Map}=\identitysmapfull{}\) & \num{< 2.2e-308} & \qty{77}{\percent} & \qty{2}{\percent} & True \\
1415. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\cov{}=\textit{Enabled}\) & \num{< 1e-5} & \qty{53}{\percent} & \qty{2}{\percent} & False \\
1416. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\cov{}=\textit{Enabled}\) & \num{< 1e-5} & \qty{51}{\percent} & \qty{2}{\percent} & True \\
1417. & \lp[\infty] & is better than &  \lp[0] & when & \(\rr{}=\textit{Disabled}\) & \num{< 2.2e-308} & \qty{77}{\percent} & \qty{2}{\percent} & False \\
1418. & \lp[\infty] & is better than &  \lp[0] & when & \(\rr{}=\textit{Disabled}\) & \num{< 2.2e-308} & \qty{75}{\percent} & \qty{2}{\percent} & True \\
1419. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.2\) & \num{< 1e-5} & \qty{57}{\percent} & \qty{2}{\percent} & False \\
1420. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.2\) & \num{1.1e-02} & \qty{59}{\percent} & \qty{2}{\percent} & True \\
1421. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.5\) & \num{< 1e-5} & \qty{68}{\percent} & \qty{2}{\percent} & False \\
1422. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.5\) & \num{2.0e-04} & \qty{66}{\percent} & \qty{2}{\percent} & True \\
1423. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.6\) & \num{< 1e-5} & \qty{68}{\percent} & \qty{2}{\percent} & False \\
1424. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.6\) & \num{2.3e-04} & \qty{66}{\percent} & \qty{2}{\percent} & True \\
1425. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.1\) & \num{< 1e-5} & \qty{56}{\percent} & \qty{2}{\percent} & False \\
1426. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.1\) & \num{< 1e-5} & \qty{54}{\percent} & \qty{2}{\percent} & True \\
1427. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.4\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{2}{\percent} & False \\
1428. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.4\) & \num{< 1e-5} & \qty{71}{\percent} & \qty{2}{\percent} & True \\
1429. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.4\) & \num{1.3e-01} & \qty{53}{\percent} & \qty{2}{\percent} & False \\
1430. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.4\) & \num{5.5e-02} & \qty{50}{\percent} & \qty{2}{\percent} & True \\
1431. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.6\) & \num{1.5e-01} & \qty{53}{\percent} & \qty{2}{\percent} & False \\
1432. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.6\) & \num{4.0e-02} & \qty{51}{\percent} & \qty{2}{\percent} & True \\
1433. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.7\) & \num{1.5e-01} & \qty{53}{\percent} & \qty{2}{\percent} & False \\
1434. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.7\) & \num{3.4e-02} & \qty{51}{\percent} & \qty{2}{\percent} & True \\
1435. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.8\) & \num{1.6e-01} & \qty{53}{\percent} & \qty{2}{\percent} & False \\
1436. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.8\) & \num{3.0e-02} & \qty{51}{\percent} & \qty{2}{\percent} & True \\
1437. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.2\) & \num{3.6e-03} & \qty{58}{\percent} & \qty{2}{\percent} & False \\
1438. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.2\) & \num{5.6e-05} & \qty{56}{\percent} & \qty{2}{\percent} & True \\
1439. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.2\) & \num{< 1e-5} & \qty{78}{\percent} & \qty{2}{\percent} & False \\
1440. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.2\) & \num{< 1e-5} & \qty{75}{\percent} & \qty{2}{\percent} & True \\
1441. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.3\) & \num{< 1e-5} & \qty{77}{\percent} & \qty{2}{\percent} & False \\
1442. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.3\) & \num{< 1e-5} & \qty{75}{\percent} & \qty{2}{\percent} & True \\
1443. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.6\) & \num{5.0e-03} & \qty{61}{\percent} & \qty{2}{\percent} & False \\
1444. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.6\) & \num{< 1e-5} & \qty{59}{\percent} & \qty{2}{\percent} & True \\
1445. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.3\) & \num{< 1e-5} & \qty{72}{\percent} & \qty{2}{\percent} & False \\
1446. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.3\) & \num{< 1e-5} & \qty{70}{\percent} & \qty{2}{\percent} & True \\
1447. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.8\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{2}{\percent} & False \\
1448. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.8\) & \num{< 1e-5} & \qty{63}{\percent} & \qty{2}{\percent} & True \\
1449. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.1\) & \num{< 1e-5} & \qty{92}{\percent} & \qty{2}{\percent} & False \\
1450. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.1\) & \num{< 1e-5} & \qty{90}{\percent} & \qty{2}{\percent} & True \\
1451. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Dataset}=\phishing{}\) & \num{< 1e-5} & \qty{75}{\percent} & \qty{2}{\percent} & False \\
1452. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Dataset}=\phishing{}\) & \num{< 1e-5} & \qty{73}{\percent} & \qty{2}{\percent} & True \\
1453. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\lp{}-\mathtt{target}=\lp[0]\) & \num{< 2.2e-308} & \qty{67}{\percent} & \qty{2}{\percent} & False \\
1454. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\lp{}-\mathtt{target}=\lp[0]\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{2}{\percent} & True \\
1455. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\rr{}=\textit{Disabled}\) & \num{3.0e-02} & \qty{50}{\percent} & \qty{2}{\percent} & False \\
1456. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\rr{}=\textit{Disabled}\) & \num{< 1e-5} & \qty{48}{\percent} & \qty{2}{\percent} & True \\
1457. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\rr{}=\textit{Enabled}\) & \num{< 1e-5} & \qty{67}{\percent} & \qty{2}{\percent} & False \\
1458. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\rr{}=\textit{Enabled}\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{2}{\percent} & True \\
1459. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\cov{}=\textit{Disabled}\) & \num{< 1e-5} & \qty{64}{\percent} & \qty{2}{\percent} & False \\
1460. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\cov{}=\textit{Disabled}\) & \num{< 2.2e-308} & \qty{66}{\percent} & \qty{2}{\percent} & True \\
1461. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Dataset}=\nslkdd{}\) & \num{< 1e-5} & \qty{68}{\percent} & \qty{2}{\percent} & False \\
1462. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Dataset}=\nslkdd{}\) & \num{< 1e-5} & \qty{70}{\percent} & \qty{2}{\percent} & True \\
1463. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\lp{}-\mathtt{target}=\lp[0]\) & \num{< 1e-5} & \qty{67}{\percent} & \qty{2}{\percent} & False \\
1464. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\lp{}-\mathtt{target}=\lp[0]\) & \num{< 2.2e-308} & \qty{69}{\percent} & \qty{2}{\percent} & True \\
1465. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.0\) & \num{< 1e-5} & \qty{97}{\percent} & \qty{2}{\percent} & False \\
1466. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.0\) & \num{< 1e-5} & \qty{100}{\percent} & \qty{2}{\percent} & True \\
1467. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.8\) & \num{< 1e-5} & \qty{98}{\percent} & \qty{2}{\percent} & False \\
1468. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.8\) & \num{< 1e-5} & \qty{96}{\percent} & \qty{2}{\percent} & True \\
1469. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.9\) & \num{< 1e-5} & \qty{98}{\percent} & \qty{2}{\percent} & False \\
1470. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.9\) & \num{< 1e-5} & \qty{96}{\percent} & \qty{2}{\percent} & True \\
1471. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+2.0\) & \num{< 1e-5} & \qty{98}{\percent} & \qty{2}{\percent} & False \\
1472. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+2.0\) & \num{< 1e-5} & \qty{96}{\percent} & \qty{2}{\percent} & True \\
1473. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.6\) & \num{< 1e-5} & \qty{62}{\percent} & \qty{2}{\percent} & False \\
1474. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.6\) & \num{< 1e-5} & \qty{60}{\percent} & \qty{2}{\percent} & True \\
1475. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\cov{}=\textit{Disabled}\) & \num{4.0e-01} & \qty{55}{\percent} & \qty{1}{\percent} & False \\
1476. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\cov{}=\textit{Disabled}\) & \num{1.9e-03} & \qty{57}{\percent} & \qty{1}{\percent} & True \\
1477. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.0\) & \num{< 1e-5} & \qty{57}{\percent} & \qty{1}{\percent} & False \\
1478. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.0\) & \num{< 1e-5} & \qty{59}{\percent} & \qty{1}{\percent} & True \\
1479. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.4\) & \num{3.6e-02} & \qty{62}{\percent} & \qty{1}{\percent} & False \\
1480. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.4\) & \num{3.6e-03} & \qty{64}{\percent} & \qty{1}{\percent} & True \\
1481. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.5\) & \num{< 1e-5} & \qty{59}{\percent} & \qty{1}{\percent} & False \\
1482. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.5\) & \num{1.5e-01} & \qty{57}{\percent} & \qty{1}{\percent} & True \\
1483. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.6\) & \num{< 1e-5} & \qty{59}{\percent} & \qty{1}{\percent} & False \\
1484. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.6\) & \num{2.3e-01} & \qty{57}{\percent} & \qty{1}{\percent} & True \\
1485. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.3\) & \num{9.8e-02} & \qty{59}{\percent} & \qty{1}{\percent} & False \\
1486. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.3\) & \num{6.2e-02} & \qty{57}{\percent} & \qty{1}{\percent} & True \\
1487. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.0\) & \num{3.7e-01} & \qty{55}{\percent} & \qty{1}{\percent} & False \\
1488. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.0\) & \num{2.1e-04} & \qty{53}{\percent} & \qty{1}{\percent} & True \\
1489. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.0\) & \num{5.4e-03} & \qty{56}{\percent} & \qty{1}{\percent} & False \\
1490. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.0\) & \num{7.9e-01} & \qty{54}{\percent} & \qty{1}{\percent} & True \\
1491. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.6\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{1}{\percent} & False \\
1492. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.6\) & \num{< 1e-5} & \qty{67}{\percent} & \qty{1}{\percent} & True \\
1493. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.1\) & \num{< 1e-5} & \qty{68}{\percent} & \qty{1}{\percent} & False \\
1494. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.1\) & \num{< 1e-5} & \qty{70}{\percent} & \qty{1}{\percent} & True \\
1495. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.9\) & \num{1.7e-01} & \qty{53}{\percent} & \qty{1}{\percent} & False \\
1496. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.9\) & \num{2.6e-02} & \qty{51}{\percent} & \qty{1}{\percent} & True \\
1497. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+2.0\) & \num{1.7e-01} & \qty{53}{\percent} & \qty{1}{\percent} & False \\
1498. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+2.0\) & \num{2.4e-02} & \qty{51}{\percent} & \qty{1}{\percent} & True \\
1499. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.3\) & \num{2.9e-04} & \qty{59}{\percent} & \qty{1}{\percent} & False \\
1500. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.3\) & \num{< 1e-5} & \qty{61}{\percent} & \qty{1}{\percent} & True \\
1501. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.7\) & \num{< 1e-5} & \qty{77}{\percent} & \qty{1}{\percent} & False \\
1502. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.7\) & \num{< 1e-5} & \qty{79}{\percent} & \qty{1}{\percent} & True \\
1503. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.3\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{1}{\percent} & False \\
1504. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.3\) & \num{< 1e-5} & \qty{63}{\percent} & \qty{1}{\percent} & True \\
1505. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.5\) & \num{< 1e-5} & \qty{66}{\percent} & \qty{1}{\percent} & False \\
1506. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.5\) & \num{< 1e-5} & \qty{64}{\percent} & \qty{1}{\percent} & True \\
1507. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\cov{}=\textit{Enabled}\) & \num{< 2.2e-308} & \qty{69}{\percent} & \qty{1}{\percent} & False \\
1508. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\cov{}=\textit{Enabled}\) & \num{< 1e-5} & \qty{71}{\percent} & \qty{1}{\percent} & True \\
1509. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Saliency Map}=\jsmasmapfull{}\) & \num{< 2.2e-308} & \qty{73}{\percent} & \qty{1}{\percent} & False \\
1510. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Saliency Map}=\jsmasmapfull{}\) & \num{< 2.2e-308} & \qty{71}{\percent} & \qty{1}{\percent} & True \\
1511. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Loss}=\cwlossfull{}\) & \num{< 2.2e-308} & \qty{94}{\percent} & \qty{1}{\percent} & False \\
1512. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Loss}=\cwlossfull{}\) & \num{< 2.2e-308} & \qty{92}{\percent} & \qty{1}{\percent} & True \\
1513. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.7\) & \num{< 1e-5} & \qty{98}{\percent} & \qty{1}{\percent} & False \\
1514. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.7\) & \num{< 1e-5} & \qty{97}{\percent} & \qty{1}{\percent} & True \\
1515. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.5\) & \num{< 1e-5} & \qty{61}{\percent} & \qty{1}{\percent} & False \\
1516. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.5\) & \num{< 1e-5} & \qty{59}{\percent} & \qty{1}{\percent} & True \\
1517. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.0\) & \num{< 1e-5} & \qty{85}{\percent} & \qty{1}{\percent} & False \\
1518. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.0\) & \num{< 1e-5} & \qty{87}{\percent} & \qty{1}{\percent} & True \\
1519. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Dataset}=\fmnist{}\) & \num{< 1e-5} & \qty{54}{\percent} & \qty{1}{\percent} & False \\
1520. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Dataset}=\fmnist{}\) & \num{< 1e-5} & \qty{52}{\percent} & \qty{1}{\percent} & True \\
1521. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Solver}=\sgd{}\) & \num{< 2.2e-308} & \qty{81}{\percent} & \qty{1}{\percent} & False \\
1522. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Solver}=\sgd{}\) & \num{< 2.2e-308} & \qty{82}{\percent} & \qty{1}{\percent} & True \\
1523. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Dataset}=\phishing{}\) & \num{< 2.2e-308} & \qty{90}{\percent} & \qty{1}{\percent} & False \\
1524. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Dataset}=\phishing{}\) & \num{< 2.2e-308} & \qty{89}{\percent} & \qty{1}{\percent} & True \\
1525. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.7\) & \num{< 1e-5} & \qty{58}{\percent} & \qty{1}{\percent} & False \\
1526. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.7\) & \num{3.3e-01} & \qty{57}{\percent} & \qty{1}{\percent} & True \\
1527. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.8\) & \num{< 1e-5} & \qty{64}{\percent} & \qty{1}{\percent} & False \\
1528. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.8\) & \num{3.2e-03} & \qty{63}{\percent} & \qty{1}{\percent} & True \\
1529. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.0\) & \num{< 1e-5} & \qty{64}{\percent} & \qty{1}{\percent} & False \\
1530. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.0\) & \num{1.4e-03} & \qty{62}{\percent} & \qty{1}{\percent} & True \\
1531. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.4\) & \num{< 1e-5} & \qty{68}{\percent} & \qty{1}{\percent} & False \\
1532. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.4\) & \num{1.7e-04} & \qty{66}{\percent} & \qty{1}{\percent} & True \\
1533. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.4\) & \num{9.5e-02} & \qty{58}{\percent} & \qty{1}{\percent} & False \\
1534. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.4\) & \num{6.7e-02} & \qty{57}{\percent} & \qty{1}{\percent} & True \\
1535. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.5\) & \num{8.8e-02} & \qty{58}{\percent} & \qty{1}{\percent} & False \\
1536. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.5\) & \num{7.0e-02} & \qty{56}{\percent} & \qty{1}{\percent} & True \\
1537. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.6\) & \num{< 1e-5} & \qty{98}{\percent} & \qty{1}{\percent} & False \\
1538. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.6\) & \num{< 1e-5} & \qty{97}{\percent} & \qty{1}{\percent} & True \\
1539. & \identitylossfull{} & is better than &  \crossentropyfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.0\) & \num{5.0e-01} & \qty{39}{\percent} & \qty{1}{\percent} & False \\
1540. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.0\) & \num{5.5e-01} & \qty{58}{\percent} & \qty{1}{\percent} & True \\
1541. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.1\) & \num{1.1e-01} & \qty{60}{\percent} & \qty{1}{\percent} & False \\
1542. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.1\) & \num{4.6e-02} & \qty{58}{\percent} & \qty{1}{\percent} & True \\
1543. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.1\) & \num{< 1e-5} & \qty{74}{\percent} & \qty{1}{\percent} & False \\
1544. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.1\) & \num{< 1e-5} & \qty{72}{\percent} & \qty{1}{\percent} & True \\
1545. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.1\) & \num{< 1e-5} & \qty{78}{\percent} & \qty{1}{\percent} & False \\
1546. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.1\) & \num{< 1e-5} & \qty{76}{\percent} & \qty{1}{\percent} & True \\
1547. & \cwlossfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.2\) & \num{7.9e-01} & \qty{45}{\percent} & \qty{1}{\percent} & False \\
1548. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.2\) & \num{8.2e-02} & \qty{52}{\percent} & \qty{1}{\percent} & True \\
1549. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.5\) & \num{2.9e-02} & \qty{60}{\percent} & \qty{1}{\percent} & False \\
1550. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.5\) & \num{4.6e-05} & \qty{58}{\percent} & \qty{1}{\percent} & True \\
1551. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+2.0\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{1}{\percent} & False \\
1552. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+2.0\) & \num{< 1e-5} & \qty{63}{\percent} & \qty{1}{\percent} & True \\
1553. & \adam{} & is better than &  \sgd{} & when & \(\rr{}=\textit{Disabled}\) & \num{< 2.2e-308} & \qty{64}{\percent} & \qty{1}{\percent} & False \\
1554. & \adam{} & is better than &  \sgd{} & when & \(\rr{}=\textit{Disabled}\) & \num{< 2.2e-308} & \qty{62}{\percent} & \qty{1}{\percent} & True \\
1555. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Solver}=\adam{}\) & \num{< 1e-5} & \qty{54}{\percent} & \qty{1}{\percent} & False \\
1556. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Solver}=\adam{}\) & \num{< 1e-5} & \qty{56}{\percent} & \qty{1}{\percent} & True \\
1557. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\cov{}=\textit{Enabled}\) & \num{< 2.2e-308} & \qty{71}{\percent} & \qty{1}{\percent} & False \\
1558. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\cov{}=\textit{Enabled}\) & \num{< 2.2e-308} & \qty{69}{\percent} & \qty{1}{\percent} & True \\
1559. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.2\) & \num{< 1e-5} & \qty{92}{\percent} & \qty{1}{\percent} & False \\
1560. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.2\) & \num{< 1e-5} & \qty{90}{\percent} & \qty{1}{\percent} & True \\
1561. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.9\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{1}{\percent} & False \\
1562. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.9\) & \num{< 1e-5} & \qty{63}{\percent} & \qty{1}{\percent} & True \\
1563. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.1\) & \num{< 1e-5} & \qty{57}{\percent} & \qty{1}{\percent} & False \\
1564. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.1\) & \num{4.0e-03} & \qty{58}{\percent} & \qty{1}{\percent} & True \\
1565. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.3\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{1}{\percent} & False \\
1566. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.3\) & \num{< 1e-5} & \qty{71}{\percent} & \qty{1}{\percent} & True \\
1567. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.8\) & \num{< 1e-5} & \qty{67}{\percent} & \qty{1}{\percent} & False \\
1568. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.8\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{1}{\percent} & True \\
1569. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.3\) & \num{< 1e-5} & \qty{70}{\percent} & \qty{1}{\percent} & False \\
1570. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.3\) & \num{2.0e-05} & \qty{68}{\percent} & \qty{1}{\percent} & True \\
1571. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.5\) & \num{4.7e-02} & \qty{62}{\percent} & \qty{1}{\percent} & False \\
1572. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.5\) & \num{9.7e-03} & \qty{63}{\percent} & \qty{1}{\percent} & True \\
1573. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.0\) & \num{1.1e-01} & \qty{60}{\percent} & \qty{1}{\percent} & False \\
1574. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.0\) & \num{4.0e-02} & \qty{58}{\percent} & \qty{1}{\percent} & True \\
1575. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.2\) & \num{1.0e-01} & \qty{59}{\percent} & \qty{1}{\percent} & False \\
1576. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.2\) & \num{5.5e-02} & \qty{58}{\percent} & \qty{1}{\percent} & True \\
1577. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.6\) & \num{8.3e-02} & \qty{57}{\percent} & \qty{1}{\percent} & False \\
1578. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.6\) & \num{7.6e-02} & \qty{56}{\percent} & \qty{1}{\percent} & True \\
1579. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.5\) & \num{< 1e-5} & \qty{64}{\percent} & \qty{1}{\percent} & False \\
1580. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.5\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{1}{\percent} & True \\
1581. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.1\) & \num{< 1e-5} & \qty{71}{\percent} & \qty{1}{\percent} & False \\
1582. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.1\) & \num{< 1e-5} & \qty{70}{\percent} & \qty{1}{\percent} & True \\
1583. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.4\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{1}{\percent} & False \\
1584. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.4\) & \num{< 1e-5} & \qty{64}{\percent} & \qty{1}{\percent} & True \\
1585. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.6\) & \num{< 1e-5} & \qty{66}{\percent} & \qty{1}{\percent} & False \\
1586. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.6\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{1}{\percent} & True \\
1587. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.7\) & \num{< 1e-5} & \qty{66}{\percent} & \qty{1}{\percent} & False \\
1588. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.7\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{1}{\percent} & True \\
1589. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\cov{}=\textit{Enabled}\) & \num{< 2.2e-308} & \qty{73}{\percent} & \qty{1}{\percent} & False \\
1590. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\cov{}=\textit{Enabled}\) & \num{< 1e-5} & \qty{71}{\percent} & \qty{1}{\percent} & True \\
1591. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.9\) & \num{< 1e-5} & \qty{54}{\percent} & \qty{1}{\percent} & False \\
1592. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.9\) & \num{< 1e-5} & \qty{55}{\percent} & \qty{1}{\percent} & True \\
1593. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.5\) & \num{< 1e-5} & \qty{98}{\percent} & \qty{1}{\percent} & False \\
1594. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.5\) & \num{< 1e-5} & \qty{97}{\percent} & \qty{1}{\percent} & True \\
1595. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.4\) & \num{< 1e-5} & \qty{60}{\percent} & \qty{1}{\percent} & False \\
1596. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.4\) & \num{< 1e-5} & \qty{59}{\percent} & \qty{1}{\percent} & True \\
1597. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Loss}=\cwlossfull{}\) & \num{< 2.2e-308} & \qty{78}{\percent} & \qty{1}{\percent} & False \\
1598. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Loss}=\cwlossfull{}\) & \num{< 2.2e-308} & \qty{77}{\percent} & \qty{1}{\percent} & True \\
1599. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Dataset}=\mnist{}\) & \num{< 1e-5} & \qty{54}{\percent} & \qty{1}{\percent} & False \\
1600. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Dataset}=\mnist{}\) & \num{< 1e-5} & \qty{55}{\percent} & \qty{1}{\percent} & True \\
1601. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.1\) & \num{< 1e-5} & \qty{98}{\percent} & \qty{1}{\percent} & False \\
1602. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.1\) & \num{< 1e-5} & \qty{99}{\percent} & \qty{1}{\percent} & True \\
1603. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.6\) & \num{1.1e-04} & \qty{64}{\percent} & \qty{1}{\percent} & False \\
1604. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.6\) & \num{9.4e-03} & \qty{63}{\percent} & \qty{1}{\percent} & True \\
1605. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.1\) & \num{< 1e-5} & \qty{68}{\percent} & \qty{1}{\percent} & False \\
1606. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.1\) & \num{1.0e-04} & \qty{66}{\percent} & \qty{1}{\percent} & True \\
1607. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.1\) & \num{< 1e-5} & \qty{64}{\percent} & \qty{1}{\percent} & False \\
1608. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.1\) & \num{1.0e-03} & \qty{63}{\percent} & \qty{1}{\percent} & True \\
1609. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.2\) & \num{< 1e-5} & \qty{64}{\percent} & \qty{1}{\percent} & False \\
1610. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.2\) & \num{7.0e-04} & \qty{63}{\percent} & \qty{1}{\percent} & True \\
1611. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.3\) & \num{< 1e-5} & \qty{68}{\percent} & \qty{1}{\percent} & False \\
1612. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.3\) & \num{1.4e-04} & \qty{66}{\percent} & \qty{1}{\percent} & True \\
1613. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.3\) & \num{< 1e-5} & \qty{64}{\percent} & \qty{1}{\percent} & False \\
1614. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.3\) & \num{4.6e-04} & \qty{63}{\percent} & \qty{1}{\percent} & True \\
1615. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.4\) & \num{< 1e-5} & \qty{98}{\percent} & \qty{1}{\percent} & False \\
1616. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.4\) & \num{< 1e-5} & \qty{97}{\percent} & \qty{1}{\percent} & True \\
1617. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.4\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{1}{\percent} & False \\
1618. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.4\) & \num{3.2e-04} & \qty{63}{\percent} & \qty{1}{\percent} & True \\
1619. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.5\) & \num{< 1e-5} & \qty{92}{\percent} & \qty{1}{\percent} & False \\
1620. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.5\) & \num{< 1e-5} & \qty{91}{\percent} & \qty{1}{\percent} & True \\
1621. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.4\) & \num{1.3e-01} & \qty{58}{\percent} & \qty{1}{\percent} & False \\
1622. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.4\) & \num{5.4e-04} & \qty{56}{\percent} & \qty{1}{\percent} & True \\
1623. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.8\) & \num{< 1e-5} & \qty{54}{\percent} & \qty{1}{\percent} & False \\
1624. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.8\) & \num{< 1e-5} & \qty{55}{\percent} & \qty{1}{\percent} & True \\
1625. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.8\) & \num{7.2e-02} & \qty{57}{\percent} & \qty{1}{\percent} & False \\
1626. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.8\) & \num{8.8e-02} & \qty{56}{\percent} & \qty{1}{\percent} & True \\
1627. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.9\) & \num{1.4e-03} & \qty{53}{\percent} & \qty{1}{\percent} & False \\
1628. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.9\) & \num{3.4e-04} & \qty{54}{\percent} & \qty{1}{\percent} & True \\
1629. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+2.0\) & \num{2.2e-03} & \qty{53}{\percent} & \qty{1}{\percent} & False \\
1630. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+2.0\) & \num{6.2e-04} & \qty{54}{\percent} & \qty{1}{\percent} & True \\
1631. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.9\) & \num{2.0e-05} & \qty{63}{\percent} & \qty{1}{\percent} & False \\
1632. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.9\) & \num{4.1e-03} & \qty{62}{\percent} & \qty{1}{\percent} & True \\
1633. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.4\) & \num{< 1e-5} & \qty{92}{\percent} & \qty{1}{\percent} & False \\
1634. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.4\) & \num{< 1e-5} & \qty{91}{\percent} & \qty{1}{\percent} & True \\
1635. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.5\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{1}{\percent} & False \\
1636. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.5\) & \num{< 1e-5} & \qty{64}{\percent} & \qty{1}{\percent} & True \\
1637. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Dataset}=\unswnb{}\) & \num{< 1e-5} & \qty{51}{\percent} & \qty{1}{\percent} & False \\
1638. & \lp[0] & is better than &  \lp[2] & when & \(\mathtt{Dataset}=\unswnb{}\) & \num{< 1e-5} & \qty{52}{\percent} & \qty{1}{\percent} & True \\
1639. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Saliency Map}=\identitysmapfull{}\) & \num{< 2.2e-308} & \qty{62}{\percent} & \qty{0}{\percent} & False \\
1640. & \adam{} & is better than &  \sgd{} & when & \(\mathtt{Saliency Map}=\identitysmapfull{}\) & \num{< 2.2e-308} & \qty{61}{\percent} & \qty{0}{\percent} & True \\
1641. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.3\) & \num{< 1e-5} & \qty{92}{\percent} & \qty{0}{\percent} & False \\
1642. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.3\) & \num{< 1e-5} & \qty{91}{\percent} & \qty{0}{\percent} & True \\
1643. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.6\) & \num{< 1e-5} & \qty{92}{\percent} & \qty{0}{\percent} & False \\
1644. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.6\) & \num{< 1e-5} & \qty{91}{\percent} & \qty{0}{\percent} & True \\
1645. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.7\) & \num{< 1e-5} & \qty{61}{\percent} & \qty{0}{\percent} & False \\
1646. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.7\) & \num{< 1e-5} & \qty{60}{\percent} & \qty{0}{\percent} & True \\
1647. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.5\) & \num{< 1e-5} & \qty{64}{\percent} & \qty{0}{\percent} & False \\
1648. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.5\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{0}{\percent} & True \\
1649. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.8\) & \num{< 1e-5} & \qty{92}{\percent} & \qty{0}{\percent} & False \\
1650. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.8\) & \num{< 1e-5} & \qty{92}{\percent} & \qty{0}{\percent} & True \\
1651. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Solver}=\sgd{}\) & \num{< 1e-5} & \qty{66}{\percent} & \qty{0}{\percent} & False \\
1652. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Solver}=\sgd{}\) & \num{< 2.2e-308} & \qty{65}{\percent} & \qty{0}{\percent} & True \\
1653. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\rr{}=\textit{Enabled}\) & \num{< 1e-5} & \qty{67}{\percent} & \qty{0}{\percent} & False \\
1654. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\rr{}=\textit{Enabled}\) & \num{< 2.2e-308} & \qty{68}{\percent} & \qty{0}{\percent} & True \\
1655. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Loss}=\identitylossfull{}\) & \num{< 2.2e-308} & \qty{86}{\percent} & \qty{0}{\percent} & False \\
1656. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Loss}=\identitylossfull{}\) & \num{< 2.2e-308} & \qty{87}{\percent} & \qty{0}{\percent} & True \\
1657. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Solver}=\sgd{}\) & \num{< 1e-5} & \qty{66}{\percent} & \qty{0}{\percent} & False \\
1658. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Solver}=\sgd{}\) & \num{< 1e-5} & \qty{67}{\percent} & \qty{0}{\percent} & True \\
1659. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.1\) & \num{2.4e-03} & \qty{61}{\percent} & \qty{0}{\percent} & False \\
1660. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.1\) & \num{< 1e-5} & \qty{60}{\percent} & \qty{0}{\percent} & True \\
1661. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.4\) & \num{< 1e-5} & \qty{63}{\percent} & \qty{0}{\percent} & False \\
1662. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.4\) & \num{< 1e-5} & \qty{64}{\percent} & \qty{0}{\percent} & True \\
1663. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.7\) & \num{< 1e-5} & \qty{70}{\percent} & \qty{0}{\percent} & False \\
1664. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.7\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{0}{\percent} & True \\
1665. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.8\) & \num{< 1e-5} & \qty{70}{\percent} & \qty{0}{\percent} & False \\
1666. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.8\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{0}{\percent} & True \\
1667. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.9\) & \num{< 1e-5} & \qty{70}{\percent} & \qty{0}{\percent} & False \\
1668. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.9\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{0}{\percent} & True \\
1669. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+2.0\) & \num{< 1e-5} & \qty{67}{\percent} & \qty{0}{\percent} & False \\
1670. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+2.0\) & \num{< 1e-5} & \qty{66}{\percent} & \qty{0}{\percent} & True \\
1671. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.4\) & \num{< 1e-5} & \qty{70}{\percent} & \qty{0}{\percent} & False \\
1672. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.4\) & \num{2.4e-05} & \qty{69}{\percent} & \qty{0}{\percent} & True \\
1673. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.6\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{0}{\percent} & False \\
1674. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.6\) & \num{3.6e-05} & \qty{68}{\percent} & \qty{0}{\percent} & True \\
1675. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.6\) & \num{5.9e-02} & \qty{61}{\percent} & \qty{0}{\percent} & False \\
1676. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.6\) & \num{1.7e-02} & \qty{62}{\percent} & \qty{0}{\percent} & True \\
1677. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.7\) & \num{3.0e-05} & \qty{63}{\percent} & \qty{0}{\percent} & False \\
1678. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.7\) & \num{5.3e-03} & \qty{63}{\percent} & \qty{0}{\percent} & True \\
1679. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.7\) & \num{7.2e-02} & \qty{61}{\percent} & \qty{0}{\percent} & False \\
1680. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.7\) & \num{2.3e-02} & \qty{62}{\percent} & \qty{0}{\percent} & True \\
1681. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.9\) & \num{< 1e-5} & \qty{63}{\percent} & \qty{0}{\percent} & False \\
1682. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.9\) & \num{2.1e-03} & \qty{63}{\percent} & \qty{0}{\percent} & True \\
1683. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.9\) & \num{1.0e-01} & \qty{60}{\percent} & \qty{0}{\percent} & False \\
1684. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.9\) & \num{3.5e-02} & \qty{59}{\percent} & \qty{0}{\percent} & True \\
1685. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.2\) & \num{< 1e-5} & \qty{68}{\percent} & \qty{0}{\percent} & False \\
1686. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.2\) & \num{1.2e-04} & \qty{67}{\percent} & \qty{0}{\percent} & True \\
1687. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.5\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{0}{\percent} & False \\
1688. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.5\) & \num{2.4e-04} & \qty{64}{\percent} & \qty{0}{\percent} & True \\
1689. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.6\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{0}{\percent} & False \\
1690. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.6\) & \num{1.9e-04} & \qty{64}{\percent} & \qty{0}{\percent} & True \\
1691. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.7\) & \num{7.6e-02} & \qty{57}{\percent} & \qty{0}{\percent} & False \\
1692. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.7\) & \num{8.2e-02} & \qty{56}{\percent} & \qty{0}{\percent} & True \\
1693. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.9\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{0}{\percent} & False \\
1694. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.9\) & \num{1.3e-04} & \qty{64}{\percent} & \qty{0}{\percent} & True \\
1695. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.9\) & \num{6.8e-02} & \qty{57}{\percent} & \qty{0}{\percent} & False \\
1696. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+1.9\) & \num{9.5e-02} & \qty{56}{\percent} & \qty{0}{\percent} & True \\
1697. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+2.0\) & \num{6.4e-02} & \qty{57}{\percent} & \qty{0}{\percent} & False \\
1698. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+2.0\) & \num{1.0e-01} & \qty{56}{\percent} & \qty{0}{\percent} & True \\
1699. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.6\) & \num{2.9e-03} & \qty{61}{\percent} & \qty{0}{\percent} & False \\
1700. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.6\) & \num{2.0e-02} & \qty{61}{\percent} & \qty{0}{\percent} & True \\
1701. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.0\) & \num{< 1e-5} & \qty{68}{\percent} & \qty{0}{\percent} & False \\
1702. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.0\) & \num{< 1e-5} & \qty{68}{\percent} & \qty{0}{\percent} & True \\
1703. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.5\) & \num{< 1e-5} & \qty{70}{\percent} & \qty{0}{\percent} & False \\
1704. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.5\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{0}{\percent} & True \\
1705. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.6\) & \num{< 1e-5} & \qty{70}{\percent} & \qty{0}{\percent} & False \\
1706. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.6\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{0}{\percent} & True \\
1707. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.0\) & \num{< 1e-5} & \qty{77}{\percent} & \qty{0}{\percent} & False \\
1708. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.0\) & \num{< 1e-5} & \qty{76}{\percent} & \qty{0}{\percent} & True \\
1709. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.9\) & \num{< 1e-5} & \qty{71}{\percent} & \qty{0}{\percent} & False \\
1710. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.9\) & \num{< 1e-5} & \qty{71}{\percent} & \qty{0}{\percent} & True \\
1711. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\lp{}-\mathtt{target}=\lp[0]\) & \num{< 2.2e-308} & \qty{100}{\percent} & \qty{0}{\percent} & False \\
1712. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\lp{}-\mathtt{target}=\lp[0]\) & \num{< 2.2e-308} & \qty{99}{\percent} & \qty{0}{\percent} & True \\
1713. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.1\) & \num{< 1e-5} & \qty{58}{\percent} & \qty{0}{\percent} & False \\
1714. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.1\) & \num{< 1e-5} & \qty{57}{\percent} & \qty{0}{\percent} & True \\
1715. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.2\) & \num{< 1e-5} & \qty{98}{\percent} & \qty{0}{\percent} & False \\
1716. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.2\) & \num{< 1e-5} & \qty{99}{\percent} & \qty{0}{\percent} & True \\
1717. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.7\) & \num{< 1e-5} & \qty{54}{\percent} & \qty{0}{\percent} & False \\
1718. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.7\) & \num{< 1e-5} & \qty{55}{\percent} & \qty{0}{\percent} & True \\
1719. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.0\) & \num{< 1e-5} & \qty{54}{\percent} & \qty{0}{\percent} & False \\
1720. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.0\) & \num{< 1e-5} & \qty{55}{\percent} & \qty{0}{\percent} & True \\
1721. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.1\) & \num{< 1e-5} & \qty{98}{\percent} & \qty{0}{\percent} & False \\
1722. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.1\) & \num{< 1e-5} & \qty{98}{\percent} & \qty{0}{\percent} & True \\
1723. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.1\) & \num{< 1e-5} & \qty{54}{\percent} & \qty{0}{\percent} & False \\
1724. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.1\) & \num{< 1e-5} & \qty{55}{\percent} & \qty{0}{\percent} & True \\
1725. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.2\) & \num{< 1e-5} & \qty{98}{\percent} & \qty{0}{\percent} & False \\
1726. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.2\) & \num{< 1e-5} & \qty{98}{\percent} & \qty{0}{\percent} & True \\
1727. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.2\) & \num{< 1e-5} & \qty{54}{\percent} & \qty{0}{\percent} & False \\
1728. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.2\) & \num{< 1e-5} & \qty{55}{\percent} & \qty{0}{\percent} & True \\
1729. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.3\) & \num{< 1e-5} & \qty{98}{\percent} & \qty{0}{\percent} & False \\
1730. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.3\) & \num{< 1e-5} & \qty{98}{\percent} & \qty{0}{\percent} & True \\
1731. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.3\) & \num{< 1e-5} & \qty{63}{\percent} & \qty{0}{\percent} & False \\
1732. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.3\) & \num{< 1e-5} & \qty{64}{\percent} & \qty{0}{\percent} & True \\
1733. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.4\) & \num{< 1e-5} & \qty{64}{\percent} & \qty{0}{\percent} & False \\
1734. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.4\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{0}{\percent} & True \\
1735. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.7\) & \num{< 1e-5} & \qty{92}{\percent} & \qty{0}{\percent} & False \\
1736. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.7\) & \num{< 1e-5} & \qty{92}{\percent} & \qty{0}{\percent} & True \\
1737. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.9\) & \num{< 1e-5} & \qty{92}{\percent} & \qty{0}{\percent} & False \\
1738. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.9\) & \num{< 1e-5} & \qty{92}{\percent} & \qty{0}{\percent} & True \\
1739. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.8\) & \num{< 1e-5} & \qty{62}{\percent} & \qty{0}{\percent} & False \\
1740. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.8\) & \num{< 1e-5} & \qty{61}{\percent} & \qty{0}{\percent} & True \\
1741. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Loss}=\crossentropyfull{}\) & \num{< 2.2e-308} & \qty{78}{\percent} & \qty{0}{\percent} & False \\
1742. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Loss}=\crossentropyfull{}\) & \num{< 2.2e-308} & \qty{79}{\percent} & \qty{0}{\percent} & True \\
1743. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Dataset}=\mnist{}\) & \num{< 2.2e-308} & \qty{70}{\percent} & \qty{0}{\percent} & False \\
1744. & \crossentropyfull{} & is better than &  \identitylossfull{} & when & \(\mathtt{Dataset}=\mnist{}\) & \num{< 2.2e-308} & \qty{71}{\percent} & \qty{0}{\percent} & True \\
1745. & \adam{} & is better than &  \sgd{} & when & \(\cov{}=\textit{Enabled}\) & \num{< 2.2e-308} & \qty{60}{\percent} & \qty{0}{\percent} & False \\
1746. & \adam{} & is better than &  \sgd{} & when & \(\cov{}=\textit{Enabled}\) & \num{< 2.2e-308} & \qty{61}{\percent} & \qty{0}{\percent} & True \\
1747. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.3\) & \num{< 1e-5} & \qty{57}{\percent} & \qty{0}{\percent} & False \\
1748. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.3\) & \num{4.2e-02} & \qty{58}{\percent} & \qty{0}{\percent} & True \\
1749. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.8\) & \num{8.6e-02} & \qty{60}{\percent} & \qty{0}{\percent} & False \\
1750. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.8\) & \num{2.8e-02} & \qty{61}{\percent} & \qty{0}{\percent} & True \\
1751. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.3\) & \num{6.8e-01} & \qty{57}{\percent} & \qty{0}{\percent} & False \\
1752. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.3\) & \num{1.8e-01} & \qty{58}{\percent} & \qty{0}{\percent} & True \\
1753. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.9\) & \num{< 1e-5} & \qty{67}{\percent} & \qty{0}{\percent} & False \\
1754. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.9\) & \num{< 1e-5} & \qty{66}{\percent} & \qty{0}{\percent} & True \\
1755. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.5\) & \num{< 1e-5} & \qty{55}{\percent} & \qty{0}{\percent} & False \\
1756. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.5\) & \num{< 1e-5} & \qty{55}{\percent} & \qty{0}{\percent} & True \\
1757. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.5\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{0}{\percent} & False \\
1758. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.5\) & \num{2.9e-05} & \qty{69}{\percent} & \qty{0}{\percent} & True \\
1759. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.6\) & \num{< 1e-5} & \qty{54}{\percent} & \qty{0}{\percent} & False \\
1760. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.6\) & \num{< 1e-5} & \qty{55}{\percent} & \qty{0}{\percent} & True \\
1761. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.7\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{0}{\percent} & False \\
1762. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.7\) & \num{4.6e-05} & \qty{69}{\percent} & \qty{0}{\percent} & True \\
1763. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.0\) & \num{< 1e-5} & \qty{67}{\percent} & \qty{0}{\percent} & False \\
1764. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.0\) & \num{8.3e-05} & \qty{68}{\percent} & \qty{0}{\percent} & True \\
1765. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.8\) & \num{7.0e-04} & \qty{54}{\percent} & \qty{0}{\percent} & False \\
1766. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.8\) & \num{2.0e-04} & \qty{54}{\percent} & \qty{0}{\percent} & True \\
1767. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+2.0\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{0}{\percent} & False \\
1768. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+2.0\) & \num{1.2e-04} & \qty{64}{\percent} & \qty{0}{\percent} & True \\
1769. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.3\) & \num{< 1e-5} & \qty{62}{\percent} & \qty{0}{\percent} & False \\
1770. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.3\) & \num{< 1e-5} & \qty{63}{\percent} & \qty{0}{\percent} & True \\
1771. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.5\) & \num{2.2e-02} & \qty{60}{\percent} & \qty{0}{\percent} & False \\
1772. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.5\) & \num{4.1e-02} & \qty{60}{\percent} & \qty{0}{\percent} & True \\
1773. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.8\) & \num{9.3e-05} & \qty{62}{\percent} & \qty{0}{\percent} & False \\
1774. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.8\) & \num{7.1e-03} & \qty{62}{\percent} & \qty{0}{\percent} & True \\
1775. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.1\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{0}{\percent} & False \\
1776. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.1\) & \num{1.9e-03} & \qty{64}{\percent} & \qty{0}{\percent} & True \\
1777. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.7\) & \num{< 1e-5} & \qty{66}{\percent} & \qty{0}{\percent} & False \\
1778. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.7\) & \num{< 1e-5} & \qty{66}{\percent} & \qty{0}{\percent} & True \\
1779. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.7\) & \num{< 1e-5} & \qty{66}{\percent} & \qty{0}{\percent} & False \\
1780. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.7\) & \num{4.0e-04} & \qty{66}{\percent} & \qty{0}{\percent} & True \\
1781. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.8\) & \num{< 1e-5} & \qty{66}{\percent} & \qty{0}{\percent} & False \\
1782. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.8\) & \num{< 1e-5} & \qty{67}{\percent} & \qty{0}{\percent} & True \\
1783. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.8\) & \num{< 1e-5} & \qty{66}{\percent} & \qty{0}{\percent} & False \\
1784. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.8\) & \num{3.4e-04} & \qty{66}{\percent} & \qty{0}{\percent} & True \\
1785. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.9\) & \num{< 1e-5} & \qty{66}{\percent} & \qty{0}{\percent} & False \\
1786. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.9\) & \num{< 1e-5} & \qty{67}{\percent} & \qty{0}{\percent} & True \\
1787. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.3\) & \num{5.1e-01} & \qty{55}{\percent} & \qty{0}{\percent} & False \\
1788. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.3\) & \num{7.2e-03} & \qty{55}{\percent} & \qty{0}{\percent} & True \\
1789. & \lp[2] & is better than &  \lp[0] & when & \(\cov{}=\textit{Enabled}\) & \num{< 2.2e-308} & \qty{89}{\percent} & \qty{0}{\percent} & False \\
1790. & \lp[2] & is better than &  \lp[0] & when & \(\cov{}=\textit{Enabled}\) & \num{< 2.2e-308} & \qty{90}{\percent} & \qty{0}{\percent} & True \\
1791. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Dataset}=\nslkdd{}\) & \num{< 2.2e-308} & \qty{96}{\percent} & \qty{0}{\percent} & False \\
1792. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Dataset}=\nslkdd{}\) & \num{< 2.2e-308} & \qty{97}{\percent} & \qty{0}{\percent} & True \\
1793. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Dataset}=\unswnb{}\) & \num{< 2.2e-308} & \qty{90}{\percent} & \qty{0}{\percent} & False \\
1794. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Dataset}=\unswnb{}\) & \num{< 2.2e-308} & \qty{89}{\percent} & \qty{0}{\percent} & True \\
1795. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Solver}=\adam{}\) & \num{< 1e-5} & \qty{56}{\percent} & \qty{0}{\percent} & False \\
1796. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Solver}=\adam{}\) & \num{< 1e-5} & \qty{56}{\percent} & \qty{0}{\percent} & True \\
1797. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Dataset}=\mnist{}\) & \num{< 1e-5} & \qty{47}{\percent} & \qty{0}{\percent} & False \\
1798. & \lp[\infty] & is better than &  \lp[2] & when & \(\mathtt{Dataset}=\mnist{}\) & \num{< 1e-5} & \qty{47}{\percent} & \qty{0}{\percent} & True \\
1799. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.7\) & \num{< 1e-5} & \qty{98}{\percent} & \qty{0}{\percent} & False \\
1800. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.7\) & \num{< 1e-5} & \qty{98}{\percent} & \qty{0}{\percent} & True \\
1801. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.8\) & \num{< 1e-5} & \qty{98}{\percent} & \qty{0}{\percent} & False \\
1802. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.8\) & \num{< 1e-5} & \qty{98}{\percent} & \qty{0}{\percent} & True \\
1803. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.9\) & \num{< 1e-5} & \qty{98}{\percent} & \qty{0}{\percent} & False \\
1804. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.9\) & \num{< 1e-5} & \qty{98}{\percent} & \qty{0}{\percent} & True \\
1805. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.0\) & \num{< 1e-5} & \qty{98}{\percent} & \qty{0}{\percent} & False \\
1806. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.0\) & \num{< 1e-5} & \qty{98}{\percent} & \qty{0}{\percent} & True \\
1807. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.3\) & \num{1.5e-05} & \qty{54}{\percent} & \qty{0}{\percent} & False \\
1808. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.3\) & \num{< 1e-5} & \qty{55}{\percent} & \qty{0}{\percent} & True \\
1809. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.7\) & \num{3.3e-04} & \qty{54}{\percent} & \qty{0}{\percent} & False \\
1810. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.7\) & \num{1.1e-04} & \qty{54}{\percent} & \qty{0}{\percent} & True \\
1811. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.3\) & \num{< 1e-5} & \qty{59}{\percent} & \qty{0}{\percent} & False \\
1812. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.3\) & \num{< 1e-5} & \qty{59}{\percent} & \qty{0}{\percent} & True \\
1813. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.2\) & \num{< 1e-5} & \qty{64}{\percent} & \qty{0}{\percent} & False \\
1814. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.2\) & \num{< 1e-5} & \qty{63}{\percent} & \qty{0}{\percent} & True \\
1815. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+2.0\) & \num{< 1e-5} & \qty{92}{\percent} & \qty{0}{\percent} & False \\
1816. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+2.0\) & \num{< 1e-5} & \qty{92}{\percent} & \qty{0}{\percent} & True \\
1817. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+2.0\) & \num{< 1e-5} & \qty{67}{\percent} & \qty{0}{\percent} & False \\
1818. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+2.0\) & \num{< 1e-5} & \qty{67}{\percent} & \qty{0}{\percent} & True \\
1819. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Dataset}=\fmnist{}\) & \num{< 1e-5} & \qty{82}{\percent} & \qty{0}{\percent} & False \\
1820. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Dataset}=\fmnist{}\) & \num{< 2.2e-308} & \qty{83}{\percent} & \qty{0}{\percent} & True \\
1821. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Saliency Map}=\dfsmapfull{}\) & \num{< 2.2e-308} & \qty{81}{\percent} & \qty{0}{\percent} & False \\
1822. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Saliency Map}=\dfsmapfull{}\) & \num{< 2.2e-308} & \qty{82}{\percent} & \qty{0}{\percent} & True \\
1823. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Loss}=\identitylossfull{}\) & \num{< 1e-5} & \qty{59}{\percent} & \qty{0}{\percent} & False \\
1824. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Loss}=\identitylossfull{}\) & \num{< 1e-5} & \qty{59}{\percent} & \qty{0}{\percent} & True \\
1825. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\rr{}=\textit{Disabled}\) & \num{< 1e-5} & \qty{68}{\percent} & \qty{0}{\percent} & False \\
1826. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\rr{}=\textit{Disabled}\) & \num{< 2.2e-308} & \qty{67}{\percent} & \qty{0}{\percent} & True \\
1827. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Dataset}=\nslkdd{}\) & \num{< 1e-5} & \qty{58}{\percent} & \qty{0}{\percent} & False \\
1828. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Dataset}=\nslkdd{}\) & \num{< 1e-5} & \qty{59}{\percent} & \qty{0}{\percent} & True \\
1829. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.4\) & \num{< 1e-5} & \qty{58}{\percent} & \qty{0}{\percent} & False \\
1830. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.4\) & \num{8.7e-02} & \qty{57}{\percent} & \qty{0}{\percent} & True \\
1831. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.7\) & \num{< 1e-5} & \qty{66}{\percent} & \qty{0}{\percent} & False \\
1832. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.7\) & \num{< 1e-5} & \qty{67}{\percent} & \qty{0}{\percent} & True \\
1833. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.0\) & \num{< 1e-5} & \qty{62}{\percent} & \qty{0}{\percent} & False \\
1834. & \lp[2] & is better than &  \lp[\infty] & when & \(\mathtt{Threat\ Model}=\lp[0]+0.0\) & \num{< 1e-5} & \qty{62}{\percent} & \qty{0}{\percent} & True \\
1835. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.8\) & \num{< 1e-5} & \qty{68}{\percent} & \qty{0}{\percent} & False \\
1836. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.8\) & \num{5.9e-05} & \qty{68}{\percent} & \qty{0}{\percent} & True \\
1837. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.9\) & \num{< 1e-5} & \qty{68}{\percent} & \qty{0}{\percent} & False \\
1838. & \identitysmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.9\) & \num{6.9e-05} & \qty{68}{\percent} & \qty{0}{\percent} & True \\
1839. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.7\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{0}{\percent} & False \\
1840. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.7\) & \num{1.6e-04} & \qty{65}{\percent} & \qty{0}{\percent} & True \\
1841. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.4\) & \num{1.4e-01} & \qty{59}{\percent} & \qty{0}{\percent} & False \\
1842. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.4\) & \num{9.0e-02} & \qty{59}{\percent} & \qty{0}{\percent} & True \\
1843. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.6\) & \num{< 1e-5} & \qty{66}{\percent} & \qty{0}{\percent} & False \\
1844. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.6\) & \num{< 1e-5} & \qty{66}{\percent} & \qty{0}{\percent} & True \\
1845. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.8\) & \num{< 1e-5} & \qty{67}{\percent} & \qty{0}{\percent} & False \\
1846. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.8\) & \num{< 1e-5} & \qty{67}{\percent} & \qty{0}{\percent} & True \\
1847. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.0\) & \num{< 1e-5} & \qty{64}{\percent} & \qty{0}{\percent} & False \\
1848. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.0\) & \num{2.9e-03} & \qty{64}{\percent} & \qty{0}{\percent} & True \\
1849. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.2\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{0}{\percent} & False \\
1850. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.2\) & \num{1.3e-03} & \qty{65}{\percent} & \qty{0}{\percent} & True \\
1851. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.3\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{0}{\percent} & False \\
1852. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.3\) & \num{1.0e-03} & \qty{65}{\percent} & \qty{0}{\percent} & True \\
1853. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.4\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{0}{\percent} & False \\
1854. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.4\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{0}{\percent} & True \\
1855. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.4\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{0}{\percent} & False \\
1856. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.4\) & \num{8.0e-04} & \qty{66}{\percent} & \qty{0}{\percent} & True \\
1857. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.6\) & \num{< 1e-5} & \qty{66}{\percent} & \qty{0}{\percent} & False \\
1858. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.6\) & \num{4.9e-04} & \qty{66}{\percent} & \qty{0}{\percent} & True \\
1859. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.9\) & \num{< 1e-5} & \qty{66}{\percent} & \qty{0}{\percent} & False \\
1860. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.9\) & \num{2.8e-04} & \qty{66}{\percent} & \qty{0}{\percent} & True \\
1861. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+2.0\) & \num{< 1e-5} & \qty{70}{\percent} & \qty{0}{\percent} & False \\
1862. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+2.0\) & \num{< 1e-5} & \qty{70}{\percent} & \qty{0}{\percent} & True \\
1863. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.6\) & \num{< 1e-5} & \qty{78}{\percent} & \qty{0}{\percent} & False \\
1864. & \lp[2] & is better than &  \lp[0] & when & \(\mathtt{Threat\ Model}=\lp[inf]+0.6\) & \num{< 1e-5} & \qty{78}{\percent} & \qty{0}{\percent} & True \\
1865. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.0\) & \num{< 1e-5} & \qty{71}{\percent} & \qty{0}{\percent} & False \\
1866. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[inf]+1.0\) & \num{< 1e-5} & \qty{71}{\percent} & \qty{0}{\percent} & True \\
1867. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Saliency Map}=\jsmasmapfull{}\) & \num{< 2.2e-308} & \qty{81}{\percent} & \qty{0}{\percent} & False \\
1868. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Saliency Map}=\jsmasmapfull{}\) & \num{< 2.2e-308} & \qty{81}{\percent} & \qty{0}{\percent} & True \\
1869. & \jsmasmapfull{} & is better than &  \dfsmapfull{} & when & \(\mathtt{Loss}=\cwlossfull{}\) & \num{< 1e-5} & \qty{54}{\percent} & \qty{0}{\percent} & False \\
1870. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Loss}=\cwlossfull{}\) & \num{4.4e-01} & \qty{45}{\percent} & \qty{0}{\percent} & True \\
1871. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.2\) & \num{< 1e-5} & \qty{56}{\percent} & \qty{0}{\percent} & False \\
1872. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.2\) & \num{< 1e-5} & \qty{56}{\percent} & \qty{0}{\percent} & True \\
1873. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.3\) & \num{< 1e-5} & \qty{55}{\percent} & \qty{0}{\percent} & False \\
1874. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.3\) & \num{< 1e-5} & \qty{56}{\percent} & \qty{0}{\percent} & True \\
1875. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.4\) & \num{< 1e-5} & \qty{55}{\percent} & \qty{0}{\percent} & False \\
1876. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.4\) & \num{< 1e-5} & \qty{55}{\percent} & \qty{0}{\percent} & True \\
1877. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.4\) & \num{3.6e-05} & \qty{54}{\percent} & \qty{0}{\percent} & False \\
1878. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.4\) & \num{1.4e-05} & \qty{55}{\percent} & \qty{0}{\percent} & True \\
1879. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.5\) & \num{7.9e-05} & \qty{54}{\percent} & \qty{0}{\percent} & False \\
1880. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.5\) & \num{2.9e-05} & \qty{55}{\percent} & \qty{0}{\percent} & True \\
1881. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.6\) & \num{1.6e-04} & \qty{54}{\percent} & \qty{0}{\percent} & False \\
1882. & \rr{}: \textit{Disabled} & is better than &  \rr{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.6\) & \num{5.9e-05} & \qty{55}{\percent} & \qty{0}{\percent} & True \\
1883. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.2\) & \num{< 1e-5} & \qty{57}{\percent} & \qty{0}{\percent} & False \\
1884. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.2\) & \num{< 1e-5} & \qty{57}{\percent} & \qty{0}{\percent} & True \\
1885. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.0\) & \num{< 1e-5} & \qty{62}{\percent} & \qty{0}{\percent} & False \\
1886. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.0\) & \num{< 1e-5} & \qty{62}{\percent} & \qty{0}{\percent} & True \\
1887. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.1\) & \num{< 1e-5} & \qty{63}{\percent} & \qty{0}{\percent} & False \\
1888. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.1\) & \num{< 1e-5} & \qty{63}{\percent} & \qty{0}{\percent} & True \\
1889. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.6\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{0}{\percent} & False \\
1890. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.6\) & \num{< 1e-5} & \qty{66}{\percent} & \qty{0}{\percent} & True \\
1891. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Solver}=\adam{}\) & \num{< 1e-5} & \qty{62}{\percent} & \qty{0}{\percent} & False \\
1892. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Solver}=\adam{}\) & \num{< 1e-5} & \qty{61}{\percent} & \qty{0}{\percent} & True \\
1893. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.3\) & \num{< 1e-5} & \qty{98}{\percent} & \qty{0}{\percent} & False \\
1894. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.3\) & \num{< 1e-5} & \qty{99}{\percent} & \qty{0}{\percent} & True \\
1895. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Solver}=\adam{}\) & \num{< 2.2e-308} & \qty{77}{\percent} & \qty{0}{\percent} & False \\
1896. & \lp[\infty] & is better than &  \lp[0] & when & \(\mathtt{Solver}=\adam{}\) & \num{< 2.2e-308} & \qty{77}{\percent} & \qty{0}{\percent} & True \\
1897. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Saliency Map}=\jsmasmapfull{}\) & \num{< 2.2e-308} & \qty{94}{\percent} & \qty{0}{\percent} & False \\
1898. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Saliency Map}=\jsmasmapfull{}\) & \num{< 2.2e-308} & \qty{94}{\percent} & \qty{0}{\percent} & True \\
1899. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Dataset}=\fmnist{}\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{0}{\percent} & False \\
1900. & \dfsmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Dataset}=\fmnist{}\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{0}{\percent} & True \\
1901. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.4\) & \num{< 1e-5} & \qty{98}{\percent} & \qty{0}{\percent} & False \\
1902. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.4\) & \num{< 1e-5} & \qty{98}{\percent} & \qty{0}{\percent} & True \\
1903. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.5\) & \num{< 1e-5} & \qty{98}{\percent} & \qty{0}{\percent} & False \\
1904. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.5\) & \num{< 1e-5} & \qty{98}{\percent} & \qty{0}{\percent} & True \\
1905. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.6\) & \num{< 1e-5} & \qty{98}{\percent} & \qty{0}{\percent} & False \\
1906. & \cov{}: \textit{Disabled} & is better than &  \cov{}: \textit{Enabled} & when & \(\mathtt{Threat\ Model}=\lp[0]+0.6\) & \num{< 1e-5} & \qty{98}{\percent} & \qty{0}{\percent} & True \\
1907. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.8\) & \num{< 1e-5} & \qty{65}{\percent} & \qty{0}{\percent} & False \\
1908. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[0]+1.8\) & \num{1.5e-04} & \qty{65}{\percent} & \qty{0}{\percent} & True \\
1909. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.2\) & \num{6.0e-05} & \qty{61}{\percent} & \qty{0}{\percent} & False \\
1910. & \crossentropyfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.2\) & \num{< 1e-5} & \qty{61}{\percent} & \qty{0}{\percent} & True \\
1911. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.7\) & \num{4.7e-04} & \qty{61}{\percent} & \qty{0}{\percent} & False \\
1912. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.7\) & \num{1.3e-02} & \qty{61}{\percent} & \qty{0}{\percent} & True \\
1913. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.9\) & \num{< 1e-5} & \qty{68}{\percent} & \qty{0}{\percent} & False \\
1914. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.9\) & \num{< 1e-5} & \qty{68}{\percent} & \qty{0}{\percent} & True \\
1915. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.9\) & \num{< 1e-5} & \qty{62}{\percent} & \qty{0}{\percent} & False \\
1916. & \rr{}: \textit{Enabled} & is better than &  \rr{}: \textit{Disabled} & when & \(\mathtt{Threat\ Model}=\lp[2]+0.9\) & \num{< 1e-5} & \qty{62}{\percent} & \qty{0}{\percent} & True \\
1917. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.1\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{0}{\percent} & False \\
1918. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.1\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{0}{\percent} & True \\
1919. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.2\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{0}{\percent} & False \\
1920. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.2\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{0}{\percent} & True \\
1921. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.3\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{0}{\percent} & False \\
1922. & \identitylossfull{} & is better than &  \cwlossfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.3\) & \num{< 1e-5} & \qty{69}{\percent} & \qty{0}{\percent} & True \\
1923. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.5\) & \num{< 1e-5} & \qty{66}{\percent} & \qty{0}{\percent} & False \\
1924. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+1.5\) & \num{6.5e-04} & \qty{66}{\percent} & \qty{0}{\percent} & True \\
1925. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+2.0\) & \num{< 1e-5} & \qty{66}{\percent} & \qty{0}{\percent} & False \\
1926. & \identitysmapfull{} & is better than &  \jsmasmapfull{} & when & \(\mathtt{Threat\ Model}=\lp[2]+2.0\) & \num{2.3e-04} & \qty{66}{\percent} & \qty{0}{\percent} & True \\
